Concept-based Explainable Artificial Intelligence: A Survey

The field of explainable artificial intelligence emerged in response to the growing need for more transparent and reliable models. However, using raw features to provide explanations has been disputed in several works lately, advocating for more user-understandable explanations. To address this issue, a wide range of papers proposing Concept-based eXplainable Artificial Intelligence (C-XAI) methods have arisen in recent years. Nevertheless, a unified categorization and precise field definition are still missing. This paper fills the gap by offering a thorough review of C-XAI approaches. We define and identify different concepts and explanation types. We provide a taxonomy identifying nine categories and propose guidelines for selecting a suitable category based on the development context. Additionally, we report common evaluation strategies including metrics, human evaluations and dataset employed, aiming to assist the development of future methods. We believe this survey will serve researchers, practitioners, and domain experts in comprehending and advancing this innovative field.

==> Images/old/categorization_old.tex <==

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,531); %set diagram left start at 0, and has height of 531

%Rounded Rect [id:dp7274331116041264] 
\draw  [color={rgb, 255:red, 59; green, 59; blue, 59 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (345,14.34) .. controls (345,7.3) and (350.7,1.6) .. (357.74,1.6) -- (460.26,1.6) .. controls (467.3,1.6) and (473,7.3) .. (473,14.34) -- (473,52.56) .. controls (473,59.6) and (467.3,65.3) .. (460.26,65.3) -- (357.74,65.3) .. controls (350.7,65.3) and (345,59.6) .. (345,52.56) -- cycle ;

%Curve Lines [id:da9069822818900743] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (407.57,65.64) .. controls (369,95.07) and (196.34,49.45) .. (192.41,124.79) ;
\draw [shift={(192.35,127.11)}, rotate = 270.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp014536150202932419] 
\draw  [color={rgb, 255:red, 71; green, 11; blue, 125 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 12; blue, 137 }  ,fill opacity=1 ] (128.67,141.28) .. controls (128.67,134.28) and (134.34,128.6) .. (141.35,128.6) -- (245.32,128.6) .. controls (252.32,128.6) and (258,134.28) .. (258,141.28) -- (258,179.32) .. controls (258,186.32) and (252.32,192) .. (245.32,192) -- (141.35,192) .. controls (134.34,192) and (128.67,186.32) .. (128.67,179.32) -- cycle ;
%Rounded Rect [id:dp08416172009781908] 
\draw  [color={rgb, 255:red, 101; green, 0; blue, 42 }  ,draw opacity=1 ][fill={rgb, 255:red, 130; green, 0; blue, 55 }  ,fill opacity=1 ] (64.17,285.3) .. controls (64.17,278.29) and (69.85,272.6) .. (76.87,272.6) -- (146.9,272.6) .. controls (153.91,272.6) and (159.6,278.29) .. (159.6,285.3) -- (159.6,323.4) .. controls (159.6,330.41) and (153.91,336.1) .. (146.9,336.1) -- (76.87,336.1) .. controls (69.85,336.1) and (64.17,330.41) .. (64.17,323.4) -- cycle ;
%Rounded Rect [id:dp5937020336327576] 
\draw  [color={rgb, 255:red, 108; green, 16; blue, 186 }  ,draw opacity=1 ][fill={rgb, 255:red, 156; green, 13; blue, 186 }  ,fill opacity=1 ] (224.4,285.32) .. controls (224.4,278.29) and (230.09,272.6) .. (237.12,272.6) -- (306.68,272.6) .. controls (313.71,272.6) and (319.4,278.29) .. (319.4,285.32) -- (319.4,323.48) .. controls (319.4,330.51) and (313.71,336.2) .. (306.68,336.2) -- (237.12,336.2) .. controls (230.09,336.2) and (224.4,330.51) .. (224.4,323.48) -- cycle ;
%Curve Lines [id:da6433376602061189] 
\draw [color={rgb, 255:red, 71; green, 11; blue, 125 }  ,draw opacity=1 ]   (193,193.9) .. controls (193,241.12) and (114.2,189.34) .. (112.26,268.63) ;
\draw [shift={(112.23,271.07)}, rotate = 270.26] [fill={rgb, 255:red, 71; green, 11; blue, 125 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da6487079456945193] 
\draw [color={rgb, 255:red, 71; green, 11; blue, 125 }  ,draw opacity=1 ]   (193,193.9) .. controls (193,241.12) and (270.39,188.76) .. (272.32,268.99) ;
\draw [shift={(272.35,271.46)}, rotate = 269.73] [fill={rgb, 255:red, 71; green, 11; blue, 125 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da13469739807455916] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (407.57,65.64) .. controls (448.2,94.57) and (621.11,49.29) .. (624.08,124.55) ;
\draw [shift={(624.11,126.86)}, rotate = 270.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp9412948815731423] 
\draw  [color={rgb, 255:red, 0; green, 74; blue, 54 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 120; blue, 94 }  ,fill opacity=1 ] (560,141.02) .. controls (560,133.99) and (565.69,128.3) .. (572.72,128.3) -- (676.61,128.3) .. controls (683.64,128.3) and (689.33,133.99) .. (689.33,141.02) -- (689.33,179.18) .. controls (689.33,186.2) and (683.64,191.9) .. (676.61,191.9) -- (572.72,191.9) .. controls (565.69,191.9) and (560,186.2) .. (560,179.18) -- cycle ;
%Rounded Rect [id:dp4140883654195102] 
\draw  [color={rgb, 255:red, 32; green, 57; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 50; green, 84; blue, 8 }  ,fill opacity=1 ] (449.33,285.2) .. controls (449.33,278.24) and (454.97,272.6) .. (461.93,272.6) -- (533.73,272.6) .. controls (540.69,272.6) and (546.33,278.24) .. (546.33,285.2) -- (546.33,323) .. controls (546.33,329.96) and (540.69,335.6) .. (533.73,335.6) -- (461.93,335.6) .. controls (454.97,335.6) and (449.33,329.96) .. (449.33,323) -- cycle ;
%Rounded Rect [id:dp37298947698967844] 
\draw  [color={rgb, 255:red, 32; green, 57; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 85; green, 143; blue, 13 }  ,fill opacity=1 ] (322.6,446.97) .. controls (322.6,438.6) and (329.39,431.81) .. (337.77,431.81) -- (402.83,431.81) .. controls (411.21,431.81) and (418,438.6) .. (418,446.97) -- (418,492.47) .. controls (418,500.84) and (411.21,507.63) .. (402.83,507.63) -- (337.77,507.63) .. controls (329.39,507.63) and (322.6,500.84) .. (322.6,492.47) -- cycle ;
%Rounded Rect [id:dp7490310290107602] 
\draw  [color={rgb, 255:red, 32; green, 57; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 85; green, 143; blue, 13 }  ,fill opacity=1 ] (448.5,447.61) .. controls (448.5,439.22) and (455.31,432.41) .. (463.7,432.41) -- (528.3,432.41) .. controls (536.69,432.41) and (543.5,439.22) .. (543.5,447.61) -- (543.5,493.23) .. controls (543.5,501.62) and (536.69,508.43) .. (528.3,508.43) -- (463.7,508.43) .. controls (455.31,508.43) and (448.5,501.62) .. (448.5,493.23) -- cycle ;
%Curve Lines [id:da16288967986936687] 
\draw [color={rgb, 255:red, 0; green, 74; blue, 54 }  ,draw opacity=1 ]   (496.23,338.82) .. controls (496.34,415.21) and (496.06,386.5) .. (496.22,428.02) ;
\draw [shift={(496.23,430.65)}, rotate = 269.78] [fill={rgb, 255:red, 0; green, 74; blue, 54 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da4687096596486655] 
\draw [color={rgb, 255:red, 0; green, 74; blue, 54 }  ,draw opacity=1 ]   (496.23,338.82) .. controls (496.23,423.76) and (372.07,367.72) .. (368.86,427.58) ;
\draw [shift={(368.79,430.4)}, rotate = 269.52] [fill={rgb, 255:red, 0; green, 74; blue, 54 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da5756562518271202] 
\draw [color={rgb, 255:red, 0; green, 74; blue, 54 }  ,draw opacity=1 ]   (624.9,193) .. controls (624.9,239.61) and (498.68,192.07) .. (496.43,268.89) ;
\draw [shift={(496.4,271.26)}, rotate = 269.79] [fill={rgb, 255:red, 0; green, 74; blue, 54 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da10471129991374672] 
\draw [color={rgb, 255:red, 0; green, 74; blue, 54 }  ,draw opacity=1 ]   (624.9,193) .. controls (624.92,234.85) and (624.24,191.88) .. (625.37,269.34) ;
\draw [shift={(625.4,271.73)}, rotate = 269.17] [fill={rgb, 255:red, 0; green, 74; blue, 54 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da23612161999763948] 
\draw [color={rgb, 255:red, 0; green, 74; blue, 54 }  ,draw opacity=1 ]   (624.9,193) .. controls (624.9,239.61) and (749.3,190.97) .. (752.55,269.68) ;
\draw [shift={(752.61,272.1)}, rotate = 269.45] [fill={rgb, 255:red, 0; green, 74; blue, 54 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp6877486310678753] 
\draw  [color={rgb, 255:red, 32; green, 62; blue, 96 }  ,draw opacity=1 ][fill={rgb, 255:red, 49; green, 95; blue, 147 }  ,fill opacity=1 ] (578.33,285.34) .. controls (578.33,278.3) and (584.04,272.6) .. (591.07,272.6) -- (660.59,272.6) .. controls (667.63,272.6) and (673.33,278.3) .. (673.33,285.34) -- (673.33,323.56) .. controls (673.33,330.6) and (667.63,336.3) .. (660.59,336.3) -- (591.07,336.3) .. controls (584.04,336.3) and (578.33,330.6) .. (578.33,323.56) -- cycle ;
%Rounded Rect [id:dp440818976138061] 
\draw  [color={rgb, 255:red, 32; green, 62; blue, 96 }  ,draw opacity=1 ][fill={rgb, 255:red, 67; green, 129; blue, 200 }  ,fill opacity=1 ] (576.43,446.34) .. controls (576.43,437.64) and (583.48,430.6) .. (592.17,430.6) -- (657.7,430.6) .. controls (666.39,430.6) and (673.43,437.64) .. (673.43,446.34) -- (673.43,493.54) .. controls (673.43,502.23) and (666.39,509.28) .. (657.7,509.28) -- (592.17,509.28) .. controls (583.48,509.28) and (576.43,502.23) .. (576.43,493.54) -- cycle ;
%Curve Lines [id:da8665589121461441] 
\draw [color={rgb, 255:red, 29; green, 53; blue, 83 }  ,draw opacity=1 ]   (624.23,339.66) .. controls (624.07,414.84) and (624.22,384.91) .. (624.38,426.62) ;
\draw [shift={(624.39,429.26)}, rotate = 269.8] [fill={rgb, 255:red, 29; green, 53; blue, 83 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp6158138593765112] 
\draw  [color={rgb, 255:red, 32; green, 62; blue, 96 }  ,draw opacity=1 ][fill={rgb, 255:red, 67; green, 129; blue, 200 }  ,fill opacity=1 ] (704.93,448.46) .. controls (704.93,440.06) and (711.74,433.25) .. (720.14,433.25) -- (784.73,433.25) .. controls (793.13,433.25) and (799.93,440.06) .. (799.93,448.46) -- (799.93,494.07) .. controls (799.93,502.47) and (793.13,509.28) .. (784.73,509.28) -- (720.14,509.28) .. controls (711.74,509.28) and (704.93,502.47) .. (704.93,494.07) -- cycle ;
%Rounded Rect [id:dp43241390371619803] 
\draw  [color={rgb, 255:red, 79; green, 52; blue, 10 }  ,draw opacity=1 ][fill={rgb, 255:red, 160; green, 110; blue, 28 }  ,fill opacity=1 ] (704.83,285.4) .. controls (704.83,278.44) and (710.47,272.8) .. (717.43,272.8) -- (787.23,272.8) .. controls (794.19,272.8) and (799.83,278.44) .. (799.83,285.4) -- (799.83,323.2) .. controls (799.83,330.16) and (794.19,335.8) .. (787.23,335.8) -- (717.43,335.8) .. controls (710.47,335.8) and (704.83,330.16) .. (704.83,323.2) -- cycle ;
%Curve Lines [id:da6915007026339077] 
\draw [color={rgb, 255:red, 29; green, 53; blue, 83 }  ,draw opacity=1 ]   (624.23,339.66) .. controls (624.07,415.22) and (748.41,368.12) .. (752.14,428.81) ;
\draw [shift={(752.23,431.66)}, rotate = 270] [fill={rgb, 255:red, 29; green, 53; blue, 83 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da1469726563668241] 
\draw [color={rgb, 255:red, 95; green, 0; blue, 39 }  ,draw opacity=1 ]   (112,338.9) .. controls (112,386.12) and (112.66,349.36) .. (112.3,428.95) ;
\draw [shift={(112.29,431.4)}, rotate = 270.26] [fill={rgb, 255:red, 95; green, 0; blue, 39 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da7395585738425303] 
\draw [color={rgb, 255:red, 95; green, 0; blue, 39 }  ,draw opacity=1 ]   (112,338.9) .. controls (112.35,415.45) and (236.06,369.55) .. (240.67,427.67) ;
\draw [shift={(240.79,430.4)}, rotate = 269.14] [fill={rgb, 255:red, 95; green, 0; blue, 39 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp5282012160860403] 
\draw  [color={rgb, 255:red, 106; green, 9; blue, 49 }  ,draw opacity=1 ][fill={rgb, 255:red, 186; green, 13; blue, 87 }  ,fill opacity=1 ] (65,448.73) .. controls (65,440.27) and (71.86,433.42) .. (80.32,433.42) -- (145.28,433.42) .. controls (153.74,433.42) and (160.6,440.27) .. (160.6,448.73) -- (160.6,494.68) .. controls (160.6,503.14) and (153.74,510) .. (145.28,510) -- (80.32,510) .. controls (71.86,510) and (65,503.14) .. (65,494.68) -- cycle ;
%Rounded Rect [id:dp15683764057028649] 
\draw  [color={rgb, 255:red, 106; green, 9; blue, 49 }  ,draw opacity=1 ][fill={rgb, 255:red, 186; green, 13; blue, 87 }  ,fill opacity=1 ] (192.03,447.2) .. controls (192.03,438.7) and (198.92,431.81) .. (207.42,431.81) -- (272.23,431.81) .. controls (280.73,431.81) and (287.63,438.7) .. (287.63,447.2) -- (287.63,493.4) .. controls (287.63,501.9) and (280.73,508.79) .. (272.23,508.79) -- (207.42,508.79) .. controls (198.92,508.79) and (192.03,501.9) .. (192.03,493.4) -- cycle ;

% Text Node
\draw (360,16.95) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{71.58pt}\setlength\topsep{0pt}
\begin{center}
\textbf{Concept-based }\\\textbf{Explainability}
\end{center}

\end{minipage}};
% Text Node
\draw (172,84.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {No};
% Text Node
\draw (619.33,84.83) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Yes};
% Text Node
\draw (335.71,85.25) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{102.22pt}\setlength\topsep{0pt}
\begin{center}
\textit{Can I modify the model?}
\end{center}

\end{minipage}};
% Text Node
\draw (335.39,389.4) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Yes};
% Text Node
\draw (262.9,176.91) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{87.96pt}\setlength\topsep{0pt}
\begin{center}
\textit{Do I have }\\\textit{annotated concepts?}
\end{center}

\end{minipage}};
% Text Node
\draw (279.7,248.7) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {No};
% Text Node
\draw (76,248.5) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Yes};
% Text Node
\draw (509.83,245.17) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Yes};
% Text Node
\draw (632.33,244.11) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {No};
% Text Node
\draw (756.77,243) node [anchor=north west][inner sep=0.75pt]  [xslant=0] [align=left] {{\small Create them!}};
% Text Node
\draw (696.23,175.91) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{87.96pt}\setlength\topsep{0pt}
\begin{center}
\textit{Do I have }\\\textit{annotated concepts?}
\end{center}

\end{minipage}};
% Text Node
\draw (474.6,389.4) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {No};
% Text Node
\draw (374.25,345) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{60.37pt}\setlength\topsep{0pt}
\begin{center}
\textit{ On the same }\\\textit{task dataset?}
\end{center}

\end{minipage}};
% Text Node
\draw (654.73,345.3) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\textit{Which kind of }\\\textit{unsupervised concepts?}};
% Text Node
\draw (707.53,444.8) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{62.43pt}\setlength\topsep{0pt}
\begin{center}
Concept \\Basis\\(Section 5.2.2)
\end{center}

\end{minipage}};
% Text Node
\draw (451.43,445.1) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{62.43pt}\setlength\topsep{0pt}
\begin{center}
Concept\\Instillation\\(Section 5.1.2)
\end{center}

\end{minipage}};
% Text Node
\draw (72.64,286.6) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{54.77pt}\setlength\topsep{0pt}
\begin{center}
Supervised\\(Section 4.1)
\end{center}

\end{minipage}};
% Text Node
\draw (66,444.63) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{65.47pt}\setlength\topsep{0pt}
\begin{center}
Class-Concept \\Relations\\(Section 4.1.1)
\end{center}

\end{minipage}};
% Text Node
\draw (131.58,345.33) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{71.27pt}\setlength\topsep{0pt}
\begin{center}
\textit{To provide which}\\\textit{explanation? }
\end{center}

\end{minipage}};
% Text Node
\draw (194.03,445.36) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{64.47pt}\setlength\topsep{0pt}
\begin{center}
Node-Concept \\Association\\(Section 4.1.2)
\end{center}

\end{minipage}};
% Text Node
\draw (714.1,287.47) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{54.77pt}\setlength\topsep{0pt}
\begin{center}
Generative\\(Section 5.3)
\end{center}

\end{minipage}};
% Text Node
\draw (583.33,286.9) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{58.85pt}\setlength\topsep{0pt}
\begin{center}
Unsupervised\\(Section 5.2) 
\end{center}

\end{minipage}};
% Text Node
\draw (229.96,287.03) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{58.85pt}\setlength\topsep{0pt}
\begin{center}
Unsupervised\\(Section 4.2)
\end{center}

\end{minipage}};
% Text Node
\draw (458.31,286.93) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{54.77pt}\setlength\topsep{0pt}
\begin{center}
Supervised\\(Section 5.1)
\end{center}

\end{minipage}};
% Text Node
\draw (159.38,142.3) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{47.12pt}\setlength\topsep{0pt}
\begin{center}
Post-hoc \\(Section 4)
\end{center}

\end{minipage}};
% Text Node
\draw (592.13,141.63) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{47.12pt}\setlength\topsep{0pt}
\begin{center}
By-design\\(Section 5)
\end{center}

\end{minipage}};
% Text Node
\draw (325.31,445.09) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{62.43pt}\setlength\topsep{0pt}
\begin{center}
Joint \\Training\\(Section 5.1.1)
\end{center}

\end{minipage}};
% Text Node
\draw (580.14,445.17) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{62.43pt}\setlength\topsep{0pt}
\begin{center}
Prototypes-\\based\\(Section 5.2.1)
\end{center}

\end{minipage}};


\end{tikzpicture}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Tables/concept_types.tex <==




% {%
% \renewcommand{\arraystretch}{1.1}
% \begin{table}[t]
%     \centering
%     \begin{tabular}{l|l}
%         % \hline
%         Concept Type                & Definition \\
%         \hline
%         Symbolic Concept            & Human-defined attribute or abstraction \\
%         Unsupervised Concept Basis  & Cluster of similar samples\\
%         Prototypes                  & (Part-of) a training sample\\
%         Textual Concepts            & Textual representation of the main classes \\
%         % \hline
%     \end{tabular}
%     \caption{Concept Types}
%     \label{tab:conc_types}
% \end{table}
% }


% {%
% % \renewcommand{\arraystretch}{1.1}
% \begin{table}[t]
%     \centering
%     \begin{tabular}{l|ll}
%         % \hline
%         Concept Type                & Definition                                                                        & Applicability \\
%         \hline
%         Symbolic Concept            &\begin{tabular}[c]{@{}l@{}} Human-defined attribute \\or abstraction \end{tabular} & \begin{tabular}[c]{@{}l@{}}Explainable-by-design models, \\Post-hoc methods\end{tabular}\\
%         Unsupervised Concept Basis  & Cluster of similar samples              & \begin{tabular}[c]{@{}l@{}} Explainable-by-design models, \\Post-hoc Methods\end{tabular}\\
%         Prototypes                  & \begin{tabular}[c]{@{}l@{}} (Part of) a training \\ sample \end{tabular}          & Explainable-by-design models\\
%         Textual Concepts            & \begin{tabular}[c]{@{}l@{}} Textual representation \\of the main class\end{tabular} & Explainable-by-design models\\
%         % \hline
%     \end{tabular}
%     \caption{Concept Types}
%     \label{tab:conc_types}
% \end{table}
% }

==> Tables/explanation_types.tex <==
% {%
% \renewcommand{\arraystretch}{1.1}
% \begin{table}[t]
%     \centering
%     \begin{tabular}{l|l}
%         Explanation Type                & Definition \\
%         \hline
%         Class-Concept Relation    & \begin{tabular}[c]{@{}l@{}}Relation among a concept and \\ an output class of a model \end{tabular}     \\
%         Node-Concept Association & \begin{tabular}[c]{@{}l@{}}Explicit association of a concept with \\ a hidden node of the network\end{tabular} \\
%         Concept-Visualization  & \begin{tabular}[c]{@{}l@{}}Visualization of a learnt concept in terms \\ of the input features\end{tabular}   
%     \end{tabular}
%     \caption{Explanation Types}
%     \label{tab:exp_types}
% \end{table}
% }

==> Tables/table_IMG_dataset.tex <==
% \begin{comment}

% PER METTERE UNA CELLA SU DUE RIGHE BASTA METTERE QUESTO CODICE ALL'INTERNO DELLA CELLA DA MODIFICARE.
% AL POSTO DI "Concept" METTERE LA PRIMA LINEA E AL POSTO DI "Employ" METTERE LA SECONDA LINEA 
% \begin{tabular}[c]{@{}c@{}}Concept \\ Employ.\end{tabular}}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\resizebox{\textwidth}{!}{


\begin{table}[]
\centering
\caption{Datasets of Images. This table shows some of the image datasets used by the methods described. We report only those most frequently used and those in which the shape of the concepts is made explicit by the authors.}
\label{tab:IMG_datasets}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\rowcolor{Gray}
\textbf{Dataset} & \textbf{Used in}& \textbf{Size} &\textbf{Task}& \textbf{Label} & \multicolumn{1}{c}{\textbf{Concepts}} \\ \hline


MNIST~\cite{lecun1998mnist} & ~\cite{crabbe2022concept}~\cite{alvarez2018towards} ~\cite{wang2023learning}~\cite{li2018deep} &  60000& CLF & Digits & Geometrical attributes %(Loop,   Vertical/horizontal line and curvature)
\\ 
\rowcolor{Gray}
MNIST even/odd~\cite{barbiero2022entropy} & ~\cite{rigotti2022attentionbased} & 60000 & CLF & Even/odd & Digits  \\

Fashion MNIST~\cite{xiao2017fashion} & ~\cite{li2018deep} & 60000 & CLF & Clothes & Details of clothes \\
\rowcolor{Gray}
colored-MNIST~\cite{kim2019learning} &~\cite{goyal2019explaining} & 60000 & CLF & Digits & Digit's colours  \\

\makecell[l]{Caltech-UCSD\\ Birds-200 (CUB)~\cite{wah2011caltech}} & \makecell[tl]{~\cite{crabbe2022concept} ~\cite{zhang2021invertible} 
~\cite{leemann2023are}
~\cite{koh2020concept}\\
~\cite{kim2023probabilistic}
~\cite{kazhdan2020now}
~\cite{zhang2018interpretable}
~\cite{wang2023learning}\\
~\cite{chen2019looks}
~\cite{rymarczyk2021protopshare}
~\cite{rymarczyk2022interpretable}
~\cite{donnelly2022deformable}\\
~\cite{sawada2022concept}
~\cite{sarkar2022framework}
~\cite{yang2023language}
~\cite{oikarinen2023label}
~\cite{zarlenga2022concept} }& 11788 & CLF & Bird species & \makecell[l]{Visual attributes of the birds \\ %(e.g. their size, the colour of their wings,   etc.).
}\\

\rowcolor{Gray}
BRODEN ~\cite{bau2017network}& ~\cite{bau2017network}
~\cite{zhou2018interpretable}
~\cite{fong2018net2vec} & 63305 & CLF & Concepts & 1197 visual concepts. \\

CelebA~\cite{Liu_2015_ICCV} & 
~\cite{goyal2019explaining}   ~\cite{marconato2022glancenets}
~\cite{zarlenga2022concept}   ~\cite{barbiero2023interpretable} & 202599 & CLF & Person's visual attributes & Non-overlapping person visual attributes \\

\rowcolor{Gray}
\makecell[l]{OsteoArthritis \\ Initiative (OAI)~\cite{oai_website}} & ~\cite{koh2020concept} & 36369 & CLF, REG & Osteoarthritis levels & Clinical concepts (features) of osteoarthritis\\

Places365~\cite{zhou2017places} &
~\cite{zhou2015object}
~\cite{chen2020concept}
~\cite{oikarinen2023label} & 10million & CLF & Scenes & Objects landmarks\\

\rowcolor{Gray}
\makecell[tl]{Animals with Attribute\\(AwA and AwA2)~\cite{awa2_website}} & 
~\cite{yeh2020completeness}
~\cite{kim2023probabilistic}
~\cite{sarkar2022framework} & 37322 & CLF & Animals & 85 numeric attribute \\

HAM10000~\cite{tschandl2018ham10000} & ~\cite{yuksekgonul2022posthoc}
~\cite{yang2023language} & 10000 & CLF & Malignant/Benignant & \makecell[l]{Characteristics of malignant skin lesions}\\

\rowcolor{Gray}
SIIM-ISIC~\cite{isic_challenge_2020} & 
~\cite{yuksekgonul2022posthoc} & 33126 & CLF & Malignant/Benignant & \makecell[tl]{Characteristics of malignant melanoma}\\

MPI3D~\cite{gondal2019transfer} & 
~\cite{marconato2022glancenets} & >1million & CLF & Objects  & 
Object attributes and robot's sensory measurements\\

%\makecell[tl]{object\_color, object\_shape,  \\  object\_size, camera\_height,  \\ background\_color, \\ and horizontal and vertical position of the arm.}\\

\end{tabular}
}
\end{table}



==> Tables/table_MISC_dataset.tex <==
\begin{table}[]
\centering
\caption{Miscellaneous of datasets. This table includes several datasets with different types of data including graphs, time series, and tables. All the datasets are used for classification tasks.% We report only those most frequently used and those in which the shape of the concepts is made explicit by the authors.
}
\label{tab:MISC_datasets}
\resizebox{\textwidth}{!}
{
\begin{tabular}{l|l|l|l|l|l}
\rowcolor{Gray}
\textbf{Dataset} & \textbf{Data Type}& \textbf{Used in} & \textbf{Size} & \multicolumn{1}{c|}{\textbf{Label}} & \multicolumn{1}{c}{\textbf{Concepts}} \\ \hline

COMPAS~\cite{compas_analysis} & TAB &~\cite{alvarez2018towards} & >60000 & Recidivism (yes/no) & Attributes \\

\rowcolor{Gray}
V-Dem~\cite{pemstein2018v} & TAB &~\cite{barbiero2022entropy, ciravegna2023logic} & 202 &State Democracy level  & Attributes\\

MIMIC-II~\cite{saeed2011multiparameter} & TAB & ~\cite{barbiero2022entropy, ciravegna2023logic} & >40000 & Patient survival (dead/alive) & Attributes \\

\rowcolor{Gray}
\makecell[l]{MIT-BIH \\ Electrocardiogram \\ (ECG)~\cite{moody2001impact}} & \makecell[l]{TIME \\ SERIES} & ~\cite{crabbe2022concept} & 47 (187 timesteps each) & Heartbeat (normal/abnormal) & \makecell[l]{4 concepts defined \\by cardiologists. \\}%(i.e., Premature Ventricular, Supraventricular,\\ Fusion Beats and Unknown)} 
\\

MUTAG~\cite{debnath1991structure} & GRAPH & ~\cite{xuanyuan2023global} & 188 & Node labels (7 classes) & Extracted \\

\rowcolor{Gray}
Reddit-binary~\cite{kipf2016semi} & GRAPH & ~\cite{xuanyuan2023global}  & 2000 & \makecell[l]{Type of graphs \\(question/answer-based community or \\ a discussion-based community)} & Extracted \\

PROTEINS~\cite{borgwardt2005protein} & GRAPH & ~\cite{xuanyuan2023global} & >1000 & Type of protein (enzymes/not enzymes) & Extracted \\

\rowcolor{Gray}
IMBD-Binary~\cite{yanardag2015deep} &GRAPH& ~\cite{xuanyuan2023global} & 1000 & Movies & Extracted \\

\end{tabular}
}
\end{table}

==> Tables/table_TXT_dataset.tex <==
\begin{table}[]
\centering
\caption{Datasets of Texts. This table shows some of the text datasets used by the methods described. All the datasets are used for classification tasks.% We report only those most frequently used and those in which the shape of the concepts is made explicit by the authors.
}
\label{tab:TXT_datasets}
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l|l}
\rowcolor{Gray}
\textbf{Dataset} & \textbf{Used in}& \textbf{Size} & \multicolumn{1}{c|}{\textbf{Label}} & \multicolumn{1}{c}{\textbf{Concepts}} \\ \hline

CEBaB~\cite{abraham2022cebab} & ~\cite{wu2023causal} &>15000& Restaurant reviews' sentiment & Aspect-level
sentiment \\

\rowcolor{Gray}
IMBD~\cite{imdb_datasets} & ~\cite{yeh2020completeness} & 50000 & Movie reviews' sentiment (pos/neg) & Extracted\\

SST-2~\cite{socher2013recursive} & ~\cite{rajagopal2021selfexplain} & >70000 & Movie reviews' sentiment (pos/neg) & Extracted \\

\rowcolor{Gray}
SST-5~\cite{socher2013recursive} & ~\cite{rajagopal2021selfexplain} & >11000 & Movie reviews' sentiment (5 classes)  & Extracted \\

TREC-6/50~\cite{li2002learning} & ~\cite{rajagopal2021selfexplain} & >5000 & Question types (6 classes/50 classes)
 & Extracted \\

\rowcolor{Gray}
%TREC-50 & ~\cite{rajagopal2021selfexplain} & >5000 & Question. (50 classes)& Extracted from text. Non-terminal phrases of the parsing tree. \\

SUBJ~\cite{pang2005seeing} & ~\cite{rajagopal2021selfexplain} & 9000 &  Subjective/objective. &Extracted  \\
\end{tabular}
% }
\end{table}

==> Tables/table_VID_dataset.tex <==
\begin{table}[]
\centering
\caption{Datasets of Videos. This table shows some of the text datasets used by the methods described. All the datasets are used for classification tasks.% We report only those most frequently used and those in which the shape of the concepts is made explicit by the authors.
}
\label{tab:VID_datasets}
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l|l}
\rowcolor{Gray}
\textbf{Dataset} & \textbf{Used in}& \textbf{Size} & \multicolumn{1}{c|}{\textbf{Label}} & \multicolumn{1}{c}{\textbf{Concepts}} \\ \hline

Kinetics-770~\cite{carreira2019short} & ~\cite{ji2023spatial}  & 65000 & Human actions (700 classes) & Extracted \\

\rowcolor{Gray}
KTH Action~\cite{schuldt2004recognizing} & ~\cite{ji2023spatial}  & >2000 & Human actions (6 classes)  & Extracted\\

BDD-OIA~\cite{xu2020explainable} & ~\cite{sawada2022concept}  &>22000 & Human actions (4 classes) & \makecell[l]{21 concepts\\ (e.g. Traffic light is green, etc.) }\\
\end{tabular}
% }
\end{table}

==> Tables/table_by_design.tex <==
\begin{landscape}
\renewcommand{\arraystretch}{1.3}
\begin{table}[]
    \caption{Explainable By-Design Concept-based Models. We characterize the approaches based on the following dimensions. \textit{Concept employment}: joint training (Joint tr.), concept instillation (Instillation); 
    \textit{Concept type}: Symbolic Concept (Symb.), Unsupervised Concept Basis (C. Basis), Prototypes (Protot.) and Textual. \textit{Scope}: Global (GL), Local (LO).
    \textit{Explanation type} (Expl Type): Class-concept relation (C-CR), Node-concept association (N-CA), and Concept Visualization (C-Viz). 
    \textit{Data type}: Images (IMG), Tabular (TAB), Textual (TXT), Graphs (GRA).  
    Performance \textit{Loss}: yes (\vmark), no (\xmark), comparable (ON PAR).
    \textit{Task}: classification (CLF), regression (REG), clustering (CLU).
    The resources \textit{availability,  Code/Models, Data}: (\vmark), no (\xmark).
    \textit{Human evaluation } (Human eval), if a user study is conducted for evaluation purposes: (\vmark), no (\xmark).
    Type of network: CNN, GNN, Transformer-based (TRANSF), AE, VAE, LLM+CNN.
    Full category description in Section~\ref{sec:categorization}.}
    \label{tab:summary:bydesign}
% \begin{adjustbox}{angle=90}
    \centering
\scalebox{0.75}{
\begin{tabular}{l|l|llcccccccccc}
 & \textbf{Method} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Concept \\ Employment\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Concept \\ type\end{tabular}}} & \textbf{Scope} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Expl\\ Type\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Data \\ type\end{tabular}} & \textbf{Loss} & \textbf{Task} & \textbf{\begin{tabular}[c]{@{}c@{}}Code/Mod\\ Avail.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Data \\ Avail.\end{tabular}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}New\\ Metric\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Human \\ eval\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Network\\ Type\end{tabular}} \\ \hline
\multirow{7}{*}{\rotatebox{90}{Supervised}} & CBM \cite{koh2020concept} & Joint tr. & Symb. & GL & \begin{tabular}[c]{@{}l@{}}N-CA, \\ C-CR*\end{tabular} & IMG & V & CLF + REG & V & X & X & X & CNN \\
 & LEN \cite{barbiero2022entropy, ciravegna2023logic,   jain2022extending} & Joint tr. & Symb. & LO \& GL & N-CA, C-CR & TAB, IMG, TXT & V & CLF + CLU & V & X & X & V & FCN, CNN \\
 & CEM\cite{zarlenga2022concept} & Joint tr. & Symb. & GL & N-CA & TAB, IMG & X & CLF & V & X & V & X & FCN, CNN \\
 & DCR\cite{barbiero2023interpretable} & Joint tr. & Symb. & LO & N-CA (GL), C-CR (LO) & TAB, IMG, GRA & X & CLF & V & X & X & X & FCN, CNN, GNN \\
 & CT   \cite{rigotti2022attentionbased} & Joint tr. & Symb. & LO \& GL & N-CA, C-CR & IMG & X/ON PAR & CLF & V & X & X & X & TRANSF \\
 & CW  \cite{chen2020concept} & Instillation & Symb. & GL & N-CA & IMG & V & CLF & V & X & V & X & CNN \\
 & PCBMs   \cite{yuksekgonul2022posthoc} & Instillation & Symb., Textual & GL & N-CA, C-CR & IMG & V & CLF & V & X & X & X & CNN \\ \hline
\multirow{6}{*}{\rotatebox{90}{Unsupervised}} & SENN   \cite{alvarez2018towards} & - & C. Basis & LO & N-CA, C-CR & IMG & X/ON PAR & CLF & X & X & X & X & AE + CNN \\
 & GlanceNets   \cite{marconato2022glancenets} & - & C. Basis & GL & N-CA, C-CR & IMG & X & CLF & V & V * & X & X & CNN (VAE) \\
 & BotCL  \cite{wang2023learner} & - & C. Basis & LO & C-CR & IMG & X/ON PAR & CLF & V & X & X & V & AE + CNN \\
 & PrototypeDL \cite{li2018deep} & - & Protot. & GL & VCE, N-CA, C-CR & IMG & X & CLF & V & X & X & X & AE+Prot. l. \\
 & ProtoPNet \cite{chen2019looks} & - & Protot. & GL & VCE, N-CA, C-CR & IMG & V & CLF & V & X & X & X & CNN+Prototype layer \\
 & ProtoPShare   \cite{rymarczyk2021protopshare} & - & Protot. &  & C-CR, VCE &  & V &  &  &  &  & X &  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sup +\\ Unsup\end{tabular}} & CBM-AUC \cite{sawada2022concept} & - & C. Basis + Symb. & GL & C-CR, N-CA & IMG + VID & X/ON PAR & CLF & X & X & X & V & encoder + discriminator \\
 & Ante-hoc Expl. \cite{sarkar2022framework} &  & C. Basis + Symb. & LO \& GL & N-CA & IMG & V & CLF & V & X & X & X &  \\ \hline
\multirow{2}{*}{\rotatebox{90}{Generative}} & LaBO \cite{yang2023language} & - & Textual & GL & C-CI, N-CA & IMG & X/ON PAR & CLF & V & X & X & V & LLM+CNN \\
 & Label-free CBM   \cite{oikarinen2023label} & - & Textual & LO \& GL & N-CA & IMG & V & CLF & V & X & X & X & LLM+CNN \\ \hline
\end{tabular}
}
\end{table}
\end{landscape}

==> Tables/table_post_hoc.tex <==
\begin{landscape}
\renewcommand{\arraystretch}{1.3}
\begin{table}[]
    \caption{Post-hoc Concept-based Explainability methods. We characterize the approaches based on the following dimensions.
    \textit{Concept type}: Symbolic Concept (Symb.), Unsupervised Concept Basis (C. Basis), Prototypes (Protot.) and Textual. \textit{Scope}: Global (GL), Local (LO).
    \textit{Explanation type} (Expl Type): Class-concept relation (C-CR), Node-concept association (N-CA), and Concept Visualization (C-Viz). 
    \textit{Data type}: Images (IMG), Tabular (TAB), Textual (TXT), Graphs (GRA).  
    \textit{Task}: classification (CLF), regression (REG), clustering (CLU).
    The resources \textit{availability,  Code/Models, Data}: (\vmark), no (\xmark).
    \textit{Human evaluation } (Human eval), if a user study is conducted for evaluation purposes: (\vmark), no (\xmark).
    Type of network.
    Full category description in Section~\ref{sec:categorization}.}
    \label{tab:summary:posthoc}
% \begin{adjustbox}{angle=90}
    \centering
\scalebox{0.9}{
\begin{tabular}{l|l|ccccccccccc}
 & \multicolumn{1}{c|}{\textbf{Method}} & \textbf{\begin{tabular}[c]{@{}c@{}}Concept \\ Type\end{tabular}} & \textbf{Scope} & \textbf{\begin{tabular}[c]{@{}c@{}}Expl. \\ Focus\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Expl \\ type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Data \\ type\end{tabular}} & \textbf{Task} & \textbf{\begin{tabular}[c]{@{}c@{}}Code/Mod. \\ Avail.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Data \\ Avail.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}New \\ metric\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Human \\ eval\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Network \\ Type\end{tabular}} \\ \hline
\multirow{5}{*}{\rotatebox{90}{Supervised}} & T-CAV   \cite{kim2018interpretability} & Symb. & GL & class & C-CI & IMG & CLF & \vmark & \xmark & \vmark & \vmark & CNN \\
 & CAR \cite{crabbe2022concept} & Symb. & GL & class & C-CI & IMG + TS & CLF & \vmark & \xmark & \vmark & \xmark & CNN \\
 & ND   \cite{bau2017network} & Symb. & GL & unit & N-CA, C-Viz & IMG & CLF & \vmark & \vmark & \vmark & \vmark & CNN \\
 & Net2Vec \cite{fong2018net2vec} & Symb. & GL & filter & N-CA, C-Viz & IMG & CLF & \vmark & \xmark & \xmark & \vmark & CNN \\
 & IBD \cite{zhou2018interpretable} & Symb. & LO \& GL & class & C-CI, C-Viz & IMG & CLF & \vmark & \xmark & \xmark & \vmark & CNN \\ \hline
\multirow{3}{*}{\rotatebox{90}{Unsupervised}} & ACE \cite{ghorbani2019towards} & C. Basis & GL & class & C-CI, C-Viz & IMG & CLF & \vmark & \xmark & \xmark & \vmark & CNN \\
 & ICE \cite{zhang2021invertible} & C. Basis & LO \& GL & class & C-CI, C-Viz & IMG & CLF & \vmark & \xmark & \xmark & \vmark & CNN \\
% & CRP \cite{achtibat2022towards} & / & LO \& GL & unit & / & IMG + TS & CLF & \vmark & \xmark & \xmark & \xmark & CNN \\ 
  & CRAFT \cite{fel2023craft} & C. Basis & GL & class & C-CI, C-Viz & IMG & CLF & \vmark & \xmark & \vmark & \vmark &  \\ \hline
\end{tabular}
}
\end{table}
\end{landscape}

% \end{adjustbox}


==> background.tex <==

%%% WHY XAI IS NEEDED (1/2 page)
% SUCCESS OF DEEP LEARNING
\subsection{AI's Trustworthiness Problem}
In recent years, the importance of Artificial Intelligence has escalated, due to its transformative impact on various aspects of society and industry. Its impact is mostly due to the success of Deep Learning models, which have shown incredible performance in fields ranging from image recognition to natural language processing and generation~\cite{lecun2015deep}. 
% DNN PROBLEMS
However, the inherent complexity and black-box nature of Deep Neural Networks (DNN) prevent from understanding the decision-making processes behind these models. Indeed, DNNs generally comprise thousands of parameters, with recent models like GPT-3 reaching over 100 billion parameters~\cite{floridi2020gpt}. Natural language models based on this architecture (like the well-known Chat-GPT), can engage in comprehensive conversations and provide responses to various subjects. However, the provision of responses does not always guarantee their accuracy ~\cite{dale2021gpt}. More significantly, the explanations they provide for their responses often lack reliability, i.e., they do not reflect the prompted input~\cite{ye2022unreliability}. This lack of transparency and reliability raises concerns about the trustworthiness of DL models. 
% REGULATION OF AI
As a consequence, and since their first inception, AI-powered decision-making systems have faced regulatory constraints and limitations~\cite{goodman2017european, maccarthy2020examination}. This holds particularly true in critical domains that significantly affect users, such as, for example, healthcare, loan approvals,  and autonomous vehicles. Further and more stringent regulations are expected to come soon, particularly within the EU. Notably, the EU Commission has just proposed comprehensive legislation, the EU AI Act. which aims to regulate and even prohibit AI-based applications according to the risk they pose for the society~\cite{veale2021demystifying}.  Interestingly, these regulations emphasize the importance of transparent AI models and human oversight. Specifically, they mandate that users have the right to receive clear and understandable information of the decisions taken by automated systems, such that it allows them to challenge the model's decision~\cite{kaminski2019right, panigutti2023role}.

%%% REVIEW OF STANDARD XAI AND WHY IT IS NOT THE SOLUTION (1/2 page)
\subsection{Review of standard XAI}
To address the challenge of creating more trustworthy and transparent AI models, researchers have pursued explainable AI  methods~\cite{adadi2018peeking}. The main idea behind XAI is the attempt to shed some lights into the decision process leading a model to make a certain prediction. 
% LOCAL EXPLANATIONS
XAI methods encompass a wide spectrum of techniques. Most methods focus on a single prediction and highlight which parts of the input contributed the most to the prediction of a certain class\footnote{In case of visual input, feature importance is usually provided by means of a saliency map.}. To this aim, a wealthy research line focuses on the analysis of the internal structure and activation pathways, back-propagating the gradient loss until the input (Vanilla Gradient,~\cite{simonyan2014deep}), or reconstructing the important parts of an input image by means of deconvolutional network (DeconvNet~\cite{zeiler2014visualizing}, or also analysing the activations of the feature maps of the last convolutional layers (CAM,~\cite{zhou2016learning}, Grad-CAM~\cite{selvaraju2017grad}).  Other techniques proposed a model-agnostic approach to assess feature importance, by approximating the model's behavior in the neighborhood of the sample prediction to explain. This can be done by means of interpretable models like logistic regressions (LIME,~\cite{ribeiro2016should}), or decision trees (LORE,~\cite{guidotti2018local}), or even by scoring the importance of the input features through a game-theoretic approach (SHAP,~\cite{lundberg2017unified}).
% NODE-LEVEL EXPLANATIONS
On the other hand, some methods aim to explain network decision-process through the visualizations of intermediate layers activations and node-level explanations. In particular,~\cite{erhan2009visualizing, simonyan2014deep} proposed an optimization process over the input features maximizing the activation of a given neuron, while~\cite{nguyen2016synthesizing} employed a Generative Adversarial Network (GAN) to generate more realistic images. In~\cite{zeiler2014visualizing}, instead, authors showed that DeconvNet can be employed to create saliency maps not only of output classes, but also of hidden neurons.   
% GLOBAL EXPLANATIONS
Finally, some methods attempted to globally interpret a model behaviour. This has been done by analysing feature importance~\cite{greenwell2018simple, apley2020visualizing}, by directly using interpretable models~\cite{yang2017scalable, fisher2019all}, linear combination of non-interpretable ones~\cite{agarwal2021neural} or interpretable surrogate models~\cite{ribeiro2016should, guidotti2018local}. However, while these methods can be useful when working with tabular data, their employment is precluded in those contexts where the input features are not meaningful per se (e.g., image pixels).  


==> backups/main_acm_paper.tex <==

\section{Introduction}
%%%
% In this paper, we propose a review and categorization of Concept-based Explainability methods (see Figure~\ref{fig:cxai}) for Artificial Intelligence (AI) models. 

% DEEP LEARNING ISSUES
In recent years, the importance of Artificial Intelligence (AI) has surged due to its transformative impact on various aspects of society and industry. This success is predominantly attributed to the advancement of Deep Learning models~\cite{lecun2015deep}. However, the inherent complexity and opaque nature of Deep Neural Networks (DNN) hinders understanding the decision-making process underlying these models. This issue prevents the safe employment of these models in contexts that significantly affect users. % such as healthcare, loan approvals, and autonomous vehicles. 
Consequently, decision-making systems based on Deep learning have faced constraints and limitations from regulatory institutions~\cite{goodman2017european, maccarthy2020examination}, which increasingly demand transparency in AI models~\cite{kaminski2019right}.

% REVIEW OF STANDARD XAI
To address the challenge of creating more trustworthy and transparent AI models, researchers have pursued eXplainable AI (XAI) methods~\cite{adadi2018peeking}.  Most XAI methods focus on a single prediction, highlighting which input features contributed the most to the prediction of a certain class. This is achieved 
%\footnote{In case of visual input, feature importance is usually provided by means of a saliency map.} 
through gradient-based analysis (Vanilla Gradient~\cite{simonyan2014deep}, CAM~\cite{zhou2016learning}, Grad-CAM~\cite{selvaraju2017grad}), or local approximations with surrogate interpretable models (LIME,~\cite{ribeiro2016should}) or game-theoretic approaches (SHAP~\cite{lundberg2017unified}). Other methods, instead, focus on node-oriented explanations to enhance network transparency~\cite{erhan2009visualizing, simonyan2014deep, zeiler2014visualizing}.
Finally, a few methods attempted to globally interpret a model behaviour via global feature importance~\cite{greenwell2018simple} %apley2020visualizing}, %or by directly using interpretable models~\cite{yang2017scalable, fisher2019all}, 
linear combination of non-interpretable ones~\cite{agarwal2021neural} or global surrogate models~\cite{ribeiro2016should, guidotti2018local}. 

% LIMITS OF STANDARD XAI
However, the reliability of standard XAI methods has been contested:~\cite{adebayo2018sanity} showed that gradient-based explanations may not change even after randomly re-parametrizing the network or the data labels, while~\cite{hooker2019benchmark} showed that methods based on surrogate models are unable to identify the most important features.
Furthermore,~\cite{kindermans2019unreliability,ghorbani2019interpretation} %, slack2020fooling} 
demonstrated that feature importance methods can be misled by simple data modification, which does not affect the model's prediction. % as they operate post-hoc, these methods may also prove ineffective in detecting training-induced artifacts upon which the model relies~\cite{adebayo2021post}.
Even if these challenges were addressed through the development of more robust methods, a fundamental concern remains: standard XAI techniques provide explanations at the feature level, which may lack meaningful interpretation, especially for non-expert users~\cite{poursabzi2021manipulating}. Understanding \textit{where} the network is looking is not sufficient to explain \textit{what} the network is seeing in a given input \cite{rudin2019stop, achtibat2023attribution}. 
To really achieve this, there is a growing consensus that XAI techniques should provide explanations in terms of higher-level attributes~\cite{kim2018interpretability, achtibat2023attribution, fel2023craft}, commonly referred to as \textit{concepts}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{Images/word_cloud.png}
    \caption{Word cloud generated from the titles, abstracts, and keywords of the reviewed C-XAI papers. The trend towards human understanding and interpretability is noticeable, in contrast to standard XAI approaches.}
    \label{fig:word_cloud}
\end{figure}

Concept-based explanations offer a compelling alternative by providing a more holistic view of the model's inner workings. By explaining the model's predictions in terms of human-understandable attributes or abstractions, concept-based explanations better resemble the way humans reason and explain % than standard explanation methods
~\cite{kim2018interpretability, kim2023help}. %not only enhance the transparency and interpretability of the model, but 
 They also empower users to gain deeper insights into the underlying reasoning, helping them to detect model biases and improve the classification model~\cite{zhou2018interpretable, jain2022extending, bontempelli2023conceptlevel}. Finally, they are more stable to perturbations than standard XAI techniques~\cite{alvarez2018towards} and can create models inherently more robust to adversarial attacks~\cite{ciravegna2023logic}. 


%%% DESCRIBE WHY THIS SURVEY IS NEEDED (COMPARISON WITH OTHER EXISTING SURVEY) (1/4 page)
%%% ADD SPACE OF SURVEY (years in consideration, conferences, number of papers) 
%%% WHO ARE THE POTENTIAL READERS OF THIS SURVEY: POSSIBLY ACADEMIC, INDUSTRIAL, NON-EXPERTS USERS, LEGISLATIVE
% \paragraph{Survey methodology}
This paper proposes the first systematic review of Concept-based eXplainable Artificial Intelligence (C-XAI) methods. 
While there exists an abundant literature of surveys in the realm of explainability~\cite{guidotti2018survey, adadi2018peeking, das2020opportunities, arrieta2020explainable, dwivedi2023explainable, bodria2023benchmarking, poche2023natural}, none of them has distinctly concentrated on the concept-based domain and only few~\cite{bodria2023benchmarking, poche2023natural} identified C-XAI as a separate category.
%To date,~\cite{yeh2021human} is the only published work reviewing few of the concept-based explanation methods examined in this survey. This analysis, however, was confined to methods proposed by the same authors and only considered a line of works (i.e., post-hoc concept-based explanation methods).
%This category of methods is progressively garnering attention due to its previously described characteristics. %Remarkably, only in 2023 we witnessed the presentation of 26 concept-based explainability papers at major AI conferences such as NeurIPS, ICLR, ICML, AAAI, IJCAI, ICCV and CVPR. However,  
%Considering these factors, we believe that the opportune moment has arrived to 
% In this survey, we offer a comprehensive overview, comparison, and categorization of the diverse concept-based explanation methods proposed in the literature.  
We analyzed papers from 2017 to July 2023 appearing in the proceedings of NeurIPS, ICLR, ICML, AAAI, IJCAI, ICCV and CVPR conferences or appeared in important journals of the field such as Nature Machine Intelligence, Transaction on Machine Learning Research, Artificial Intelligence, or also cited in the related work of these papers. 
%More precisely, we selected explainability-related papers where the keywords “Concept”, “Prototypes” or “Causal” appeared either in the title or in the abstract or were defined by other papers as concept-based explainability approaches.
To gain a visual insight into the examined papers, please refer to Figure~\ref{fig:word_cloud}. This illustration showcases the 100 most frequently occurring words found in the titles, abstracts, or keywords of the papers under review. The figure already indicates a noteworthy trend in the C-XAI field, where the emphasis is shifting towards interpretable models and explanations more in line with human understanding.


% \paragraph{Concept-based Explainable AI}
% CONCEPT-BASED EXPLANATIONS vs CONCEPT-BASED MODELS -----
% In this survey, we propose first a set of definitions to clearly define the terms characterizing the C-XAI field. Then, we propose a taxonomy composed of 13 dimensions of analysis to characterize the methods.
% Also, we propose some guidelines to assess the applicability of the methods to the different contexts. 
% We then review 
%
%
%In particular, we define 13 dimensions of analysis including concept employment and annotation, concept and explanation types, explanation scope, performance loss, data type, tasks, and network employed, data and code/model availability, as well as metrics and human evaluation. 
% In general, we categorize C-XAI methods into two primary groups: \conceptexp{} and \conceptmodel{}. In the first category, we find methods delivering post-hoc explanations for a given model, but instead of dissecting input features, they operate on concepts. %They explain a prediction, an entire class, or an internal node of the network in relation to a given set of concepts. Typically, this involves projecting the samples that represent the concepts in the model's latent space and analyzing their relation to the prediction and the hidden node activations. Concepts are represented by means of attribute annotations on dedicated datasets %(e.g., the Broden dataset~\cite{bau2017network}), or by groups of similar inputs that capture the network's common areas of focus.
% On the other hand, concept-based models require the network to predict a set of concepts as an intermediate network representation. 
% We also report a categorization of the metrics and of the datasets to facilitate the development of future methods.

% In this way, %the task predictions are always influenced by the predicted concepts, and thus, they are closely tied to the provided explanations. 
% they are inherently transparent models, at least to some extent. 
% Also in this case, a variety of concepts can be used, either explicitly annotated, extracted in an unsupervised manner, or even generated by a separate model. 


To summarize, this work contributes with the following:
\begin{itemize}
    % \item We review 56 papers regarding the C-XAI literature, including papers of critics, comparisons, and applications
    \item We properly define the key terms in the concept-based explanation field, including what is a concept and a concept-based explanation.
    \item We present a taxonomy that outlines 9 different C-XAI categories based on the utilization of concepts during training, the specific type of concept used, and the required explanation.
    \item We propose guidelines for choosing a suited approach, describing each category's applicability, advantages, and disadvantages.
    \item We analyze the methods according to 13 dimensions of analysis.
    \item We provide for each method a brief outline of its main aspects and how it differs from the other methods in the same category, including papers of critics and comparisons.
    % \item We report comparisons of existing methods and critiques. %, providing the reader with a comprehensive overview of the subject.
    \item We report metrics and datasets available for assessing and developing novel C-XAI methods.
    \item We highlight first C-XAI applications and promising future directions.
\end{itemize}


% STAKEHOLDERS
We hope this paper may serve as a reference for AI researchers and practitioners seeking to enhance the reliability of explanation methods and models.
%The proposed guidelines can help domain experts adopt the explanation method/model. 
The suggested guidelines are a valuable tool for domain experts, enabling them to select the most fitting explanation method tailored to the specific type of explanation needed or the concepts at hand, for instance.
Policymakers may also find concept-based models to be sufficiently accountable and trustworthy for the deployment of neural models in safety-critical contexts, 
% Consequently, they might mandate practitioners and companies operating in such domains to employ these approaches, 
making this paper relevant to a wide spectrum of stakeholders.    

%%% STRUCTURE OF THE SURVEY (1/4 page)
% \paragraph{Paper structure}
The paper is structured as follows: in Section~\ref{sec:def_and_cat} we provide the definitions of the most important terms in the concept-based explanation field; in Section~\ref{sec:categorization}, we define a high-level categorization of C-XAI approaches and provide readers with guidelines for selecting the suitable category; in Section~\ref{sec:concept_exp} we resume the most important post-hoc concept-based explainability methods, while in Section~\ref{sec:concept_model} we review explainable-by-design concept-based models following the previously introduced categorization; 
in Section~\ref{sec:evaluation}, we report valuable tools developed in the literature to develop and assess novel methods, including metrics, human evaluations, and datasets; 
%commonly employed metrics that have been used to compare different methods in literature; 
in Section~\ref{sec:application}, we report the first applications of concept-based explainability methods;
in Section~\ref{sec:future_work}, we hypothesize some promising future directions of the concept-XAI field; 
finally, Section~\ref{sec:conclusions} concludes the paper. % by analyzing some promising future developments in the concept-XAI field. 


\section{Definitions} % 2 pages
\label{sec:def_and_cat}
In Figure~\ref{fig:vis_abstract}, we provide a common pipeline of a C-XAI method. The input is projected in the latent space of the network, where the method aims to extract or directly represent a set of concepts (normally of the same type). For some concepts, additional knowledge may be required to employ them properly. Finally, various types of explanations can be generated in addition to the model prediction. 
Due to the recent genesis of the C-XAI literature, it is challenging to establish consensus on the definitions of certain terms. Specifically, the definitions of “concept” and “explanation” are not consistently uniform, and similar studies may adopt varying interpretations.

In the following, we first propose four typologies of concepts (Section~\ref{sec:what_concept}); secondly, we identified three different concept-based explanations with different types of explainability/interpretability (Section~\ref{sec:expltype}). Further, we recall the difference between a post-hoc method and an explainable-by-design model, particularly within the C-XAI context (Section~\ref{sec:post_vs_cbm}). Finally, in Appendix~\ref{app:glossary}, we compiled a glossary of the most commonly used terms, while in Table~\ref{tab:acronyms}, we report the acronyms and abbreviations used throughout the paper.
%We hope these definitions will also serve readers as a reference source. %allowing future literature to be consistent in using the different terms. 
% For the sake of readability, we will always reintroduce these terms upon their first mention. 

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Images/visual_abstract-2.png}
    \caption{Concepts and explanations provided by C-XAI methods and models. Some concepts require additional knowledge to be implemented.}
    \label{fig:vis_abstract}
\end{figure}


\subsection{What is a Concept?}
\label{sec:what_concept}
In the concept-based explainability literature, the term \textit{concept} has been defined in very different ways. Citing~\cite{molnar2020interpretable}, “A concept can be any abstraction, such as a colour, an object, or even an idea”. 
As we resume in the top part of Table~\ref{tab:conc_exp_types}, we propose a categorization of concepts into four typologies: %of  in the reviewed papers:
\textit{Symbolic Concepts}, \textit{Unsupervised Concept Bases}, \textit{Prototypes}, and \textit{Textual Concepts}. 

\textbf{\textit{Symbolic Concepts}} are human-defined symbols~\cite{ciravegna2023logic}. They can be high-level attributes of the task under consideration or interpretable abstractions, such as the color or the shape of the predicted object~\cite{barbiero2022entropy}. Figure \ref{fig:vis_abstract} shows that \textit{beak} is a suitable symbolic concept for a bird identification task. Since these concepts are pre-defined by humans, we generally require auxiliary data equipped with concept annotation, particularly when we are dealing with non-symbolic features (e.g., image pixels vs tabular data). The representation in the network of symbolic concepts can be analyzed post-hoc or forced during training to create an explainable-by-design model.

\textbf{\textit{Unsupervised Concept Bases}} are clusters of samples the network learns. Even if they are not built to resemble human-defined concepts, these unsupervised representations may still capture abstractions that are more understandable to humans than individual features or pixels~\cite{ghorbani2019towards}. As shown in Figure~\ref{fig:vis_abstract}, a network may learn a cluster of green birds. To extract such a concept, we require the employment of a clustering algorithm either post-hoc in the latent space of the model or during training, e.g., by means of a reconstruction loss. As in the previous case, these concepts can be employed by both explainable-by-design models or post-hoc methods.

\textbf{\textit{Prototypes}} are representative examples of peculiar traits of the training samples. They can be a training sample or only a part of a training sample. As shown in Figure~\ref{fig:vis_abstract}, a part prototype of a training sample might be a \textit{beak}. The set of prototypes is, in general, representative of the whole data set~\cite{li2018deep}. We regard prototypes as concepts following recent literature~\cite{marconato2022glancenets} since they are still higher-level terms than the input features. Also, they are different from unsupervised concept bases since they explicitly encode the peculiar traits in the network weights, and consequently, they cannot be employed in post-hoc methods but only in explainable-by-design models. 

\textbf{\textit{Textual Concepts}} are textual descriptions of the main classes. As reported in Figure~\ref{fig:vis_abstract}, a textual concept might be `A bird with bright feathers' for a sample of a parrot. Textual concepts are provided at training time by means of an external generative model~\cite{oikarinen2023label}, and they are employed inside a concept-based model in the form of a numerical embedding of the text. This type of concept is gaining prominence due to the recent development of Large-Language Models (LLMs). So far, it has been only employed in explainable-by-design models.

For a more formal definition of a Concept, following category theory principles, please refer to Appendix~\ref{sec:formal_concept}.

\input{Tables/conc_exp_types}


\subsection{What is a Concept-based Explanation?}
\label{sec:expltype}
Even when considering a fixed type of concept, the definition of a concept-based explanation can be elusive. Existing literature generally agrees that concept-based explanations should explain how DNNs make particular decisions using concepts~\cite{yeh2020completeness} and adhere to specific criteria such as being meaningful, coherent, and relevant to the final class~\cite{ghorbani2019towards} and also explicit and faithful~\cite{alvarez2018towards}. %However, the concrete nature of concept-based explanations remains open to interpretation. 
As we report in the bottom part of Table~\ref{tab:conc_exp_types}, we define three distinct categories of concept-based explanations: \textit{\classconcrel}, \textit{\nodeconcass}, and \textit{\concvisual}. Each method may offer one or more explanations, serving specific purposes in different scenarios.

\textbf{\textit{\classconcrel}} explanations consider the relationship between a specific concept and an output class within the model. This relationship can be expressed either as the importance of a concept for a particular class or through the use of a logic rule that involves multiple concepts and their connection to an output class. For example, in Figure~\ref{fig:vis_abstract}, the image in input is classified as a Parrot because it is mainly related to the concept of \textit{beak}. In general, this type of explanation can be applied to all types of concepts: for instance, with prototypes, we have class-concept explanations like $parrot :=  0.8 \  prototype_1 + 0.2 \ prototype_2$. This explanation can be extracted by analyzing post-hoc the correlation of concepts and classes in the latent space of a network or with the employment of an interpretable model from the concepts to the tasks.  
% This first type of explanation is the most analogous to standard XAI explanations, as it essentially substitutes features with concepts in relation to output classes.

\textbf{\textit{\nodeconcass}} explicitly assigns a concept to an internal unit (or a filter) of a neural network. This explanation enhances the transparency of deep learning models, highlighting what internal units see in a given sample. 
It can be defined post-hoc by considering the hidden units maximally activating on input samples representing a concept. 
Otherwise, it can also be forced during training by requiring a unit to predict a concept.  
For instance, consider Figure\ref{fig:vis_abstract}: some nodes of the network can automatically learn to recognize the beak since it is a crucial part of the prediction of a bird. Otherwise, an expert can also define a set of attributes in advance and require their explicit representation in the network intermediate layers.
% predicting the level of arthritis in X-ray joint images.  
% In addition to predicting the final class, an intermediate layer of the model can be trained to predict a set of attributes related to the joint, such as bone spurs, sclerosis level, or the space between the bones. 

Finally, \textbf{\textit{\concvisual{}}} explanations highlight the input features that best represent a specific concept. When symbolic concepts are used, this explanation closely resembles the saliency map of standard XAI methods. However, when non-symbolic concepts are employed (such as unsupervised concept basis, prototypes, or even textual concepts), the focus shifts towards understanding which unsupervised attributes or prototypes the network has learned. This form of explanation is often combined with one of the previous explanations, and it enables the understanding of what are the concepts associated with a specific class or node. 
For instance, consider again Figure~\ref{fig:vis_abstract}, where we reported a model employing prototype concepts as an example of \concvisual{}. A visualization of the prototype in the input sample %and the parts of the input sample that have been found similar 
is crucial to understand which concept the network has learned. 

\subsection{C-XAI Post-hoc Methods vs Explainable-by-design Models}
\label{sec:post_vs_cbm}
In the XAI literature, the difference between \textit{post-hoc explanation methods} and \textit{explainable-by-design models} is well-defined: 
the latter are inherently designed for transparency, such as decision trees or linear models; in contrast, the former are tools applied post-training to explain complex models, such as DNNs. %, to offer insights about their decision processes. 
On the contrary, in the field of concept-based approaches, the difference becomes more subtle since C-XAI explainable-by-design models also work with DNNs but explicitly represent some concepts within the architecture. In the following, we try to clarify this difference.  %, requiring an explicit representation of concept in the network.  
% In particular, the explicit representation of concepts inside a neural network creates what have been defined explainable-by-design models.  

\textbf{\textit{Post-hoc Concept-based Explanation Methods}} operate on concepts rather than dissecting input features. They explain a prediction, an entire class, or an internal network node given a set of concepts. Typically, this involves projecting the samples representing the concepts in the model's latent space and analyzing their relation to the prediction and the hidden node activations. 
Symbolic and unsupervised concept bases have been both employed to provide all types of explanations.
% Concepts are represented by means of attribute annotations on dedicated datasets (e.g., the Broden dataset~\cite{bau2017network}), or by groups of similar inputs that capture the network's common areas of focus.

\textbf{\textit{Explainable-by-design Concept-based Model}}, on the other hand,
are neural models employing an explicit representation of a set of concepts as an intermediate layer. In this way, the predicted concepts influence the task predictions, and thus, they are closely tied to the provided explanations. Since they generally provide Node-Concept association by-design, they can be regarded as inherently transparent models, at least to some extent.
In this case, the whole spectrum of concepts can be used, either explicitly annotated, extracted in an unsupervised manner, encoding prototypes, or even generated by a separate model. 


\section{C-XAI Taxonomy} % 3 page (1/2 for the picture)
\label{sec:categorization}
To assist users in understanding the C-XAI landscape, in this section, we provide a taxonomy of concept-based methods and models together with some guidelines for selecting an appropriate method for the development constraints and the desired outcomes. 
In Section~\ref{sec:dimanalysis}, we describe the dimensions of analysis that we employed to categorize and characterize C-XAI methods,
while in Section~\ref{sec:guidelines}, we present a procedure to follow to select the desired C-XAI method for different requirements. 

\subsection{Dimensions of analysis}
\label{sec:dimanalysis}
We characterize each concept-based explainability method by 13 dimensions of analysis. %These dimensions aid in selecting the an appropriate approach for a given context. 
We categorize these dimensions into three groups: (i) concepts and explanations characteristics, (ii) the applicability of the method, and (iii) resources employed. The dimensions related to the first two groups will be analyzed in Sections~\ref{sec:concept_exp},~\ref{sec:concept_model} and reported in Tables~\ref{tab:summary:posthoc1},~\ref{tab:summary:bydesign1}, respectively analyzing methods following two different concept training (first dimension of analysis). The third group of dimensions will be analyzed vertically (per resource/evaluation) in Section~\ref{sec:evaluation}, but we also report a horizontal analysis (per method) in Section~\ref{sec:resources}, and in the Appendix in Tables~\ref{tab:summary:posthoc2} and~\ref{tab:summary:bydesign2}.  

% \subsubsection{

%\noindent
%(i) \textbf{Concept and Explanations Characteristics}

% }

\begin{enumerate}
    \item \textbf{Concept and Explanations Characteristics}.  These dimensions capture key aspects of concepts and explanations, such as how concepts are integrated into models, concept annotation strategies, concept types, the form of explanations, and their scope.
        \begin{itemize}
            \item the \textit{Concept Training}, an approach is first categorized according to whether it employs concepts only to provide explanations of an existing model (Post-hoc methods), or also while training the same model (Explainable-by-design models);
            \item the \textit{Concept Annotation}, according to whether the method employs an annotated set of concepts (Supervised), it does not (Unsup.), it employs only a few concepts (Hybrid), or it generates concept annotation (Generative);
            \item the \textit{Concept Type} (described in Section~\ref{sec:what_concept}), which can be either symbolic (Symb.),  unsupervised concept bases (Uns. Basis), prototype-based (Proto.), or textual;
            \item the \textit{Explanation Type}, (defined in Section~\ref{sec:expltype}), either Class-concept relation (C-CR), Node-concept association (N-CA), Concept Visualization (C-Viz) or a combination of these;
            \item the \textit{Explanation Scope}, according to whether the explanation is local (LO) (i.e., it explains an individual prediction), global (GL) (i.e., it provides insights into the overall model behavior), or both.
        \end{itemize}
        Regarding Concept-based Models, %the way concepts are used during the training process is also an important characteristic. Furthermore, some of these models sacrifice some performance to obtain higher interpretability. Therefore, 
        we also characterize the methods with the following:
        \begin{itemize}
            \item the \textit{Concept Employment}, how an explainable by-design supervised model employs the concepts during training, either through joint training (Joint) or concept instillation (Instil);
            %We will further describe this dimension in Section~\ref{sec:sup_concept_model};
            \item the \textit{Performance Loss}, whether %and to what extent 
            there is a performance loss (\vmark) or not (\xmark) compared to a black-box model.
        \end{itemize}

    \item \textbf{Applicability of the approach}. These dimensions describe the approach's applicability by detailing the types of data it can handle, the primary tasks it is designed for, and the specific neural architectures utilized.
        \begin{itemize}
            \item the \textit{Data}, i.e., the data type the method can handle, generally images (IMG), but also text (TXT), graph (GRA), tabular data (TAB), videos (VID) and time series (TS);
            \item the \textit{Task} the method is designed for, primarily classification (CLF) but also regression (REG) and clustering (CLU);
            \item the \textit{Network} dimension describes the type of neural network employed, including Convolutional Neural Network (CNN),  3D-CNN, Auto-Encoder (AE), Graph Neural Network (GNN), Multi-Layer Perceptron (MLP) and Transformer (TRANSF).
        \end{itemize}
    \item \textbf{Resources and Evaluation conducted}. These dimensions focus on the resources provided (data releases and code/models availability) and the conducted evaluation.
        % Dimensions that encompass the provided resources and the evaluation conducted}. 
        % For each method, we track the resources provided, and the evaluation conducted through the following dimensions}
        \begin{itemize}
            \item the \textit{Data Release} indicates whether a new dataset annotated with concepts has been made available;
            \item The \textit{Code/Models Availability} indicates whether the authors have released the code and/or the model;
            \item the \textit{New metric} dimension indicates if the paper introduces a new evaluation metric;
            \item the \textit{Human evaluation} dimension indicates whether the paper includes a user study to evaluate the method.
        \end{itemize}   
\end{enumerate}

\begin{figure}[t]
    \centering
    \resizebox{0.8\textwidth}{!}{%
    \input{Images/categorization}
    }
    % \includegraphics[width=\textwidth]{Images/Categorization - 9.pdf}
    \caption{Categorization of the C-XAI methods with guidelines for selecting a suitable approach. 
    }
    \label{fig:categorization}
\end{figure}

\subsection{Guidelines for selecting a suitable method}
\label{sec:guidelines}
We now provide some guidelines to facilitate the method selection, employing Figure~\ref{fig:categorization} as a visual reference.
In particular, let us consider a user interested in a C-XAI method. We propose a set of a maximum of three questions that he should answer to choose a category of methods. These questions regard the possibility of modifying the learning model, the availability of an annotated set of concepts, and, according to the subcategory, the desired outcome regarding explanation or concept types or the type of training set employed. We adopted a conversational approach to help the user identify a solution that is suitable for his development conditions. %and, according to the subcategory, the type of explanation and concept or the type of training dataset employed. 
As we report in the figure, this categorization will also characterize the structure of the following sections.

\textbf{\textit{Can I modify the model?}} 
This represents the first coarse-grained question a user should answer. According to the possibility of intervening in the model's development, he can choose among two macro-categories in which the C-XAI literature is divided.
He must look at \conceptexp{} (Section~\ref{sec:concept_exp}) if he needs to consider an already trained model that he cannot (or does not want to) modify. On the other hand, if he can create a model from scratch, he can employ a \conceptmodel{} (Section~\ref{sec:concept_model}), which allows an explicit representation of the concepts within the model architecture.

\textbf{\textit{Do I have annotated concepts?}} Secondly, the user should check whether he can find a dataset annotated with concepts that are related to the task at hand.  
% The following categorization depends on the availability of annotated concepts and their use. 
In case of a positive response, he should look at supervised methods; otherwise, he should consider unsupervised ones that can extract concepts from the same data automatically.
% We define a method as Supervised if it leverages annotated concepts while Unsupervised if it does not and extracts concepts automatically. 
For explainable-by-design approaches, he can pick from two more categories. He can employ a hybrid solution that leverages a few supervised concepts together with unsupervised extracted ones since, recently, he can also use a generative method that creates the concepts by means of an external model. 

For some sub-categories in Figure~\ref{fig:categorization}, we identify a third-level of fine-grained categories (and associated questions) according to whether the explanation, the concept employed, or the concept annotation varies among the methods within the subcategory. 
\textbf{\textit{To provide which Explanation?}} - If he selected a post-hoc supervised approach, these differ in the type of explanations, either class-concept relations or node-concept associations.
\textbf{\textit{On the same task Dataset?}} - Explainable-by-design supervised approaches either require concept annotation on the same dataset of the task at hand or allow them on a separate one. 
\textbf{\textit{Which kind of unsupervised concepts?}} - Finally, if he chose an unsupervised explainable-by-design approach, they differ in the representation of unsupervised concepts adopted. Instead, the methods in the remaining sub-categories share these main characteristics; hence, we have not split them further. 



% In the following, we describe the high-level characteristics of the two main categories, post-hoc (Section~\ref{sec:cat_cexp}) and explainable-by-design (Section~\ref{sec:cat_cbm}), highlighting the advantages and disadvantages and outlining their sub-categories. Finally, we specify further dimensions of analysis for the considered methods (Section~\ref{sec:dimanalysis}).

% \subsection{\Conceptexp{}} 
% \label{sec:cat_cexp}
% Concept-based Explanations methods employs a post-hoc approach, therefore providing explanations of an existing model after it has been trained. Often, these methods do not make any assumption on the explained model internal architecture: if this is the case, they are also defined as model-agnostic. They can be exploited on any given model, and they do not require changing the model's internal architecture. 

% \myparagraphbold{Advantages}
% %For these reasons, 
% Post-hoc explanation methods are the only viable option in scenarios where a pre-trained model exists or a predefined model is necessary.
% Also, Concept-based explainability methods are the preferred choice when there can be no compromise on the predictive and generalization capabilities of the model. They allow for enhanced interpretability without affecting the model's performance.  

% \myparagraphbold{Disadvantages}
% The main drawback of these methods is that they do not guarantee that the model truly comprehends or employs the adopted concepts. This is because the model was not exposed to these concepts during its training process. Concept-based explainability methods can only be regarded as a better way of explaining the network behavior by employing terms that are more comprehensible to humans than raw input features.

% \myparagraphbold{Sub-categories}
% \conceptexp{} (Section \ref{sec:concept_exp}) primarily diverge on the employment of an external dataset containing labelled concepts (Supervised) or not (Unsupervised methods). To ensure meaningful explanations, data and concepts in the external dataset must be related to the task for which the model was originally trained.

% \textit{Supervised.} Supervised concept-based explanations methods (Section \ref{sec:sup_concept_exp}) analyze network behaviour on samples representing \textit{symbolic concepts}. The underlying idea is that a network automatically learn to recognize some concept. These methods aim to assess which concept has been learnt, where, and how it influences the model. This analysis is conducted differently according to the type of explanations delivered. In particular, if a method provide Class-concepts relations (Section \ref{sec:post-sup-class}), they analyze how the current prediction or an entire class weight correlates with the projection of a concept in the latent space of the model. On the contrary, methods providing explanations in terms of Node-concept associations study the activations of single hidden nodes over the entire dataset to associate them to a concept (Section \ref{sec:post-sup-node-concept-assoc}). %and with this analysis we can shed some lights in the inner working of the model itself. 

% \textit{Unsupervised.}
% Unsupervised methods (Section \ref{sec:unsup_concept_exp}) seek to identify unsupervised clusters of samples (i.e., an \textit{unsupervised concept basis}), exerting influence on a given prediction, 
% or an entire class. Therefore, they generally provide explanations in terms of Class-concepts relations. This category bears similarities to standard XAI methods. However, they differ in that they do not select features relying solely on their saliency or internal similarity (as with superpixels) but rather for their capability to represent other input samples. Due to the limited number of unsupervised methods and since they all provide explanations in terms of \classconcrel, we do not define further subcategories in this case.  



% \subsection{\Conceptmodel}
% \label{sec:cat_cbm}
% %In contrast to \conceptexp{}, 
% \conceptmodel{} (Section \ref{sec:concept_model}) introduce a deviation from standard neural network training practices. They explicitly represent concepts within the same neural network architecture. Thereby, we define them as explainable-by-design since they all provide Node-concept associations. To achieve this goal, they typically employ a dedicated hidden layer to predict concept scores. These scores represent numerical values quantifying the relevance or presence of specific concepts in a given input sample. To learn these concepts, Concept-based Models necessitate ad-hoc network training.

% \myparagraphbold{Advantages}
% Concept-based Models offer the advantage of ensuring that the network learns a set of concepts explicitly. 
% For this reason, they generally provide explanations in terms of Node-concept associations by-design. %The predictions they provide, therefore, can always be analyzed in terms of these concepts. 
% Furthermore, %they facilitate interaction with the network through concept intervention~\cite{koh2020concept}. 
% a domain expert can modify the predicted values for specific concepts and observe how the model's output changes in response. This process is referred to as \textit{concept intervention} and it enables the generation of counterfactual explanations. For example, it allows understandings like “If the model did not consider the joint space too narrow for this patient, it would not have predicted severe arthritis”~\cite{koh2020concept}.

% \myparagraphbold{Disadvantages}
% On the other hand, these methods can only be employed when there is flexibility to train a model from scratch, possibly tailoring it to the specific task at hand.  Furthermore, in simpler solutions, the predictive accuracy of concept-based models may be lower than that of standard black-box models. 


% \myparagraphbold{Sub-categories}
% %As previously, also 
% Concept-based models primarily differ in whether they employ a dataset with annotated concepts (Supervised), without concept annotations (Unsupervised), with few concept annotations (Hybrid) or they create the supervision (Generative).

% \textit{Supervised.}
% Supervised concept models (Section \ref{sec:sup_concept_model}) mandate a consistent set of samples with Symbolic Concept annotation. This set of samples can be provided alongside the task supervisions to perform a \textit{joint-training} (Section \ref{sec:sup_joint_train}). Otherwise, they can also be embedded in the model through a separate training on an external dataset dedicated solely to concept learning, therefore performing a \textit{concept instillation} (Section \ref{sec:sup_concept_instill}).  

% \textit{Unsupervised.} Unsupervised concept models (Section \ref{sec:unsup_concept_model}), instead, modify the internal representation of a network to autonomously extract concepts without explicitly associating them with pre-defined symbols. In this case, the extracted concepts \textit{unsupervised concept basis} (Section \ref{sec:unsup_concept_basis}), i.e., a clusterized sample representation identifying groups of similar samples or generative factors. Otherwise, these model also explicitly encode \textit{prototypes-concepts} in the network architecture (Section \ref{sec:unsup_prototype}) that represent (parts of) frequently seen input samples.

% \textit{Hybrid.} Other works take a different approach, integrating in the architecture both supervised and unsupervised concepts (Section \ref{sec:sup_unsup_cbm}). The goal of this integration is generally to allow the employment of concept-based models also in those scenarios where few supervised concepts are available for the task at hand. %This allows to increase the generalization performance of standard supervised concept models as well as extracting a better concept representation.

% \textit{Generative.} Generative methods, instead, employ an external generative model to define textual concepts (i.e., textual descriptions of the main classes) (Section \ref{sec:generative}). These textual descriptions are then embedded  in the internal representation of the network in the form of numerical representation to predict the final classes. At test time, these models predict both the final class and the most suitable descriptions among those that have been learnt.  




\section{\conceptexp{}} % 8 pages
\label{sec:concept_exp}
\input{Tables/table_posthoc_1}
Concept-based explanation methods explain an existing model without modifying its internal architecture.  For this reason, they are post-hoc methods, i.e., they analyze the model only after it has finished the training process. 
% We summarize in Table~\ref{tab:summary:posthoc1} the main features of each approach based on the taxonomy outlined in Section~\ref{sec:categorization}. 

As we can observe from Table~\ref{tab:summary:posthoc1}, 
\conceptexp{} primarily diverge on the employment of a dataset containing concept annotations (Supervised, Section~\ref{sec:sup_concept_exp}) or not (Unsupervised methods, Section~\ref{sec:unsup_concept_exp}). 
While in the first case, they employ Symbolic Concepts, in the latter, they extract explanations based on unsupervised concept basis. 
Furthermore, supervised methods differ in focusing on either explaining class-concept relations (C-CR) or node-concept associations (N-CA). In both cases, they can also provide concept visualizations (C-Viz). Unsupervised methods, instead, generally focus on class-concept relations as well as on visualizing the extracted concepts. The explanation scope of most methods is global (GL), with few methods providing both local and global explanations (LO\&GL) and one only local (LO). 
All the reviewed methods have been developed to explain classification tasks (CLF), and many have been designed for CNNs and image (IMG) data types.  
A few methods have been developed for working with texts (TXT), graphs (GRAPH), or videos (VID) and employing transformers (TRANS) (both for texts and images), GNNs, and 3D-CNN architectures. 
To characterize the key aspects of post-hoc methods, here we discuss the main positive aspects versus the negative ones.

\myparagraphbold{Advantages}
Post-hoc explanation methods are the only viable option in scenarios where a pre-trained model exists or a predefined model is necessary.
Also, Concept-based explainability methods are the preferred choice when there can be no compromise on the predictive and generalization capabilities of the model. They allow for enhanced interpretability without affecting the model's performance.  

\myparagraphbold{Disadvantages}
The main drawback of these methods is that they do not guarantee that the model truly comprehends or employs the adopted concepts. This is because the model was not exposed to these concepts during its training process. Concept-based explainability methods can only be regarded as a better way of explaining the network behavior by employing terms that are more comprehensible to humans than raw input features. We will further discuss the issues and challenges post-hoc methods face at the end of this section (Section~\ref{sec:posthoc_issues}). 


% \myparagraphbold{Sub-categories}
% As we can observe from Table~\ref{tab:summary:posthoc1}, 
% To ensure meaningful explanations, data and concepts in the external dataset must be related to the task for which the model was originally trained.
% In Section~\ref{sec:sup_concept_exp}, we will analyze Supervised methods, which rely on an existing dataset set equipped with symbolic concept annotations; in Section~\ref{sec:unsup_concept_exp}, 
% %we analyze methods providing Unsupervised post-hoc explanations, therefore extracting explanations based on unsupervised concept basis. 
% we analyze unsupervised methods that extract explanations based on unsupervised concept basis. 



%\subsection{Post-hoc Supervised Concept-based explainability methods}
\subsection{Supervised Concept-based Explainability Methods}
\label{sec:sup_concept_exp}
Post-hoc supervised concept-based explanation methods analyze network behavior over samples annotated with \textit{symbolic concepts}. The underlying idea is that a network automatically learns to recognize some concepts. These methods aim to assess which concepts have been learned, where, and how they influence the model. 
This analysis is conducted differently according to the type of explanations delivered. 
In particular, to provide Class-concepts relations, some methods analyze how the current prediction or an entire class weight correlates with the projection of a concept in the latent space of the model (Section \ref{sec:post-sup-class}). On the contrary, methods extracting explanations in terms of Node-concept associations study the activations of single hidden nodes to associate them to a given concept (Section \ref{sec:post-sup-node-concept-assoc}). 
%and with this analysis we can shed some lights in the inner working of the model itself. 
% In both scenarios, post-hoc supervised methods %offer concept-based explanations 
% exploit an external dataset annotated with \textit{symbolic concepts}. 
% These annotations encompass attributes related to the tasks the model has been trained for. 
%First, we will review supervised post-hoc methods leveraging this external dataset to improve the model's interpretability and establishing connections between its outputs and the symbolic concepts, thereby providing \classconcrels. Afterwards, we will analyze methods associating these symbolic concepts to internal nodes or filters of the neural model, therefore supplying \nodeconcass{} explanations. 
% We review these methods based on the types of explanations they provide: \classconcrels\  (Section~\ref{sec:post-sup-class}) and \nodeconcass{} (Section~\ref{sec:post-sup-node-concept-assoc}).



\subsubsection{\classconcrel{} methods}
\label{sec:post-sup-class}
Supervised post-hoc methods offering explanations examine the connection between output classes and a set of symbolic concepts. As illustrated in Figure~\ref{fig:post_hoc_sup_class_conc}, 
this is generally achieved by presenting samples representing concepts to the explained network and analyzing its behaviour. In the figure, we report the case of a model trained to recognize birds (e.g., a Parrot) and tested with samples representing a related concept (e.g., the Beak). The effect of the concepts on the final class is studied by either (i) analyzing the representation of concepts in the model's latent space and its relation with the output classes (TCAV, TCAR, IBD) or (ii) exploring the causal effect of inserting or removing a concept on the prediction of a particular class (CaCE, CPM). 
The samples representing the symbolic concepts are drawn from an external dataset, which is then a requirement for this class of methods. As previously mentioned, the set of concepts must be related to the output classes to extract meaningful explanations. 


\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{Images/posthoc_sup_classconc.png}
    \includegraphics[width=.8\textwidth]{Images/posthoc_sup_classconc.png}
    \caption{Post-hoc Supervised Methods providing explanations in terms of class-concept relations. 
    These approaches provide a set of samples annotated with concepts to the explained network to determine their influence on the output class.
    %The explained network is provided with samples annotated with concepts in order to determine their influence on the output class.
    }
    \label{fig:post_hoc_sup_class_conc}
\end{figure}

\smallskip
Testing with Concept Activation Vector \textbf{(T-CAV~\cite{kim2018interpretability})} has been the first work in this category.
%providing post-hoc supervised explanations by means of class-concept relations.
It introduces the idea of employing a linear probe to assess the interpretability of a model. It consists of (i) freezing the model's internal architecture and (ii) training a linear layer in the latent space of the model to predict the concepts.
For each user-defined concept, it requires %two sets of images : 
a positive set comprising images representing the concept and a complementary one with negative samples. 
The Concept Activation Vectors (CAVs) represent the orthogonal vectors to the weights of the linear probe, separating positive examples of a given concept from negative ones. 
Then, T-CAV computes the inner product between the directional derivatives of the class and the CAVs to quantify the models' conceptual sensitivity, i.e., 
how much each concept positively influences the prediction of a given class. 
The T-CAV score is the fraction of the class's inputs with a positive conceptual sensitivity. The higher the score, the higher the influence of the concept.
As noted by the authors, CAVs require concepts to be linearly separable. However, concepts may be semantically linked and mapped to latent space portions that are close to each other. 
In this case, the authors propose to employ Relative CAVs, i.e., CAVs obtained when considering as negative samples the positive concepts of other concepts. 
The authors showed that T-CAV enables humans to identify the most important concepts for a network trained over standard and corrupted features, while several standard XAI methods do not.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Images/tcav.png}
%     \caption{Testing with Concept Activation Vectors~\cite{kim2018interpretability}. Given a user-defined set of positive and negative examples of a given concept (e.g., ‘striped’), one can analyze how these are projected in the latent space with respect to labeled training samples (e.g., representing zebras). More precisely, TCAV quantifies the extent to which a class is sensitive to a concept by means of the directional derivatives of the class with respect to the learned concept activation vector.}
%     \label{fig:tcav}
% \end{figure}


% \myparagraphbold{CAR~\cite{crabbe2022concept}}
\smallskip
Concept Activation Regions \textbf{(CAR~\cite{crabbe2022concept})} relaxes the linear separability assumption of concepts imposed by T-CAV. 
CAR only requires concept examples to be grouped in clusters in the model's latent space such that they are identifiable by a non-linear probe (e.g., a kernel-based SVM). Each concept is thus represented by a \emph{region} in the latent space and no longer by a single vector. 
To this aim, the authors define the notion of concept smoothness, i.e., the possibility to separate a \textit{positive region} in which the concept is predominantly present and a \textit{negative region} in which the concept is not present.
A concept is important for a given example if its projection lies in the cluster of concept positive representations.
Equivalently to the TCAV score, the authors propose the TCAR score, quantifying the proportion of instances belonging to a specific class whose representations fall within the positive concept region. 
% The authors show that, 
In some settings, TCAR returns high scores expressing significant associations between classes and concepts, while TCAV returns low scores. %, leading to the opposite conclusion. 
The authors claim that this is due to employing a more powerful concept classifier and, consequently, that TCAR scores reflect the relations between classes and concepts more accurately.
% However, a too-powerful model may lead to overfitting   


%%% IBD
% \myparagraphbold{IBD~\cite{zhou2018interpretable}}
\smallskip
Interpretable Basis Decomposition \textbf{(IBD~\cite{zhou2018interpretable})} 
provides class-concept relations by decomposing the evidence supporting a prediction into the most semantically related components. %Each component is represented by a symbolic concept and a ranked measure of its contribution.  
Concretely, IBD considers the classes and the concepts as vectors in the latent space of the penultimate layer of the network.
As for T-CAV, to represent the concepts, IBD trains a set of linear classifiers over the projections in the latent space. % of the network of images representing the concepts.  
IBD then performs an optimization to assess the relevance of each concept for a class. For all samples in the concept dataset, they try to reconstruct a given class's prediction using a linear regression. In this, the variables are the inner product between each concept vector and the projection of the sample in the latent space. Instead, the coefficients represent each concept's associated importance for the given class.
Interestingly, the \emph{residual} of the optimization assesses the variability in the class predictions that cannot be represented by means of the learned concepts.
% Network decisions, indeed, might rely on visual attributes that lack correspondence with any symbolic concept. 
Furthermore, each concept is accompanied by a heat map showing the features with the highest impact on the concept prediction. 
By means of human evaluation, the authors demonstrated that IBD explanations enhance standard XAI techniques (like CAM and Grad-CAM) regarding model assessment quality.

% \myparagraphbold{CaCE~\cite{goyal2019explaining}}
\smallskip
The Causal Concept Effect \textbf{(CaCE~\cite{goyal2019explaining})} investigates the causal effect made by the presence or absence of a symbolic concept on a network prediction. 
%%%What is 
% They argue that other methods might be influenced by the correlation of the concept with the explained class, which %However, the simple correlation 
% might not reflect the actual decision-making process of the model. 
To measure how much a concept can change the classifier's output, they propose operating over the original sample, removing the concept and generating a counterfactual sample.
%For simplicity, in CaCE, it is assumed that concepts are binary and correspond to the presence or absence of the concepts themselves. So, 
The CaCE measure is defined as the effect of the presence of the binary concept on the classifier's output. 
%%%How it works 
To effectively compute it, we must control the generative process of the samples annotated with concepts. % to evaluate the effect on the classifier.
To achieve this, the authors propose two approaches.
(i) Using a controlled environment, it is possible to intervene in the sample generation process, manually inserting or removing a concept and calculating the exact CaCE value for this intervention. 
(ii) Training a generative model to represent images with and without the concepts to approximate the generative process. % from concepts to samples, and requiring it to represent or remove concept. 
In the second scenario, a %conditional-
Variational Auto-Encoder (VAE) architecture can be used in two different variants, either generating images with one concept or another, or % one by means of the VAE's decoder; or by means of both the encoder and the decoder 
generating the counterfactual of an image with/without a certain concept. 
%%%Results
The authors apply their approach to four datasets, comparing CaCE with a non-causal version of CaCE and TCAV~\cite{kim2018interpretability},
showing that CaCE better understands and identifies the concept as having a causal relation with the class prediction. %, surpassing the other approaches. 

% \myparagraphbold{CPM~\cite{wu2023causal}}
\smallskip
Similarly to CaCE, the Causal Proxy Model \textbf{(CPM~\cite{wu2023causal})} provides causal concept-based explanations, this time tailored for Natural Language Processing (NLP) models.
%%%What is
CPM builds upon the CEBaB benchmark~\cite{abraham2022cebab}, a dataset %providing the controlled environment for 
studying the presence/absence of a concept on textual data and its causal effect on a model. Starting from a dataset of factual restaurant reviews, it provides counterfactual examples %of that review 
in which a concept (food, service, ambiance, etc.) has been modified. 
%%%How it works
CPM is first initialized with the weights of the black-box model to explain. For both factual and counterfactual inputs, CPM is then trained to mimic the behaviour of the black-box model. Since counterfactual examples are not provided at test time, CPM is still prompted with the factual sample and information coming from the counterfactual one for counterfactual training. %More precisely, the authors propose CPM$_{\text{IN}}$, which uses a learnable token representing the counterfactual concept values, while CPM$_{\text{HI}}$ interchange the activations of some hidden nodes of the network with the obtained when prompted with the counterfactual example~\cite{geiger2022inducing}. 
%The explanations provided by 
CPM explanations %for four models on the CEBAB dataset 
are compared with TCAV~\cite{kim2018interpretability}, the baseline of CaCE~\cite{goyal2019explaining}, %ConceptSHAP~\cite{yeh2020completeness} 
and others. The comparison is performed by measuring the distance between the ground-truth (i.e., the actual prediction variation when prompted with a counterfactual sample) and the relative importance of the concept for the predicted class provided by each explainer.  
The results show that both versions of the CPM significantly outperform previous methods in assessing the causality of a concept. 


\subsubsection{\nodeconcass{} methods}
\label{sec:post-sup-node-concept-assoc}

Supervised post-hoc methods may also aim to associate symbolic concepts with internal nodes or filters of the neural model. In this case, the idea is to understand where the model has automatically learned some concepts. This allows us to shed some light on the decision process of a given model. As shown in Figure~\ref{fig:post_hoc_sup_node}, these methods supply \nodeconcass{} explanations by checking which nodes activate the most when the network is presented with input image representing the concepts (e.g., the beak) (ND, Net2Vec) or input graphs (GNN-CI). However, this process can also be performed by human annotators analyzing a node's common activation areas (Object Detectors).   

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.4]{Images/posthoc_sup_nodeconc.png}
    \caption{Post-hoc supervised methods providing an explanation in terms of Node-Concept Associations. This class of approaches associates concepts with internal nodes or filters of the network.}
    \label{fig:post_hoc_sup_node}
\end{figure}

\smallskip
% \myparagraphbold{Object Detectors~\cite{zhou2015object}}
\textbf{Object Detectors~\cite{zhou2015object}} is a precursor to what has been termed concept-based explainability since 2017. 
% It attempts to disclose the complexities of 
It aims to shed some light on the learned representations in the hidden layers of a neural network. In particular, the study reveals that hidden neurons automatically learn to recognize some objects when training a network to classify %various categories of 
scenes. %This underlines the versatility of a unique network, demonstrating its ability to facilitate recognition across different levels of abstraction, such as edges and textures. 
More precisely, to understand and quantify the precise semantics learned from each unit, this work uses AMT workers. 
Workers have to uniquely identify the concept %that exist between the highest-scoring 
given the input activation of each unit, as well as define the unit's precision by selecting all the activations that do not correspond to the concept. According to the AMT workers, the results show that a hidden unit automatically learns to recognize a concept with a precision higher than 70\% on average across all hidden layers. 
Interestingly, they show that the types of concepts learned gradually shift from colours and textures in lower layers to objects and object parts in higher ones. 
It can be said that this is the first example of human-supervised annotation of concepts.


\smallskip
% \myparagraphbold{Network Dissection (ND)~\cite{bau2017network}}
Similarly to Object Detectors, Network Dissection \textbf{(ND~\cite{bau2017network})} %represents the first work that 
% directly aims to explain single network neurons, associating them with a unique concept.
aims to explain single network neurons by associating them with a unique concept.
Rather than employing AMT workers, they propose a new dataset, BRODEN (BROad and DENsely labeled dataset)~\cite{agrawal2014analyzing}, which includes concept labels from diverse data sources. 
To associate each node to a specific concept, the authors propose to compute the Intersection over Unions (IoU) of the bounding boxes representing the concepts and the activation maps of the node over the BRODEN dataset. The node is then associated with the concept with the highest IoU. 
In output, ND reports the units with the highest average IoU and the samples with the highest overlap for each concept.  
For each concept, we can have more than a unit in the network that is associated with it. 
It is essential to notice that Network Dissection's effectiveness relies on the quality of the underlying dataset. If a network unit corresponds to a concept understandable to humans but not present in the given dataset, it will receive a lower interpretability score IoU.
 As a result, they show that individual units may automatically learn to represent high-level semantics objects. 
concluding that the units of a deep representation may be more interpretable than expected. 

% \myparagraphbold{Net2Vec~\cite{fong2018net2vec}}
\smallskip
The work Network to Vector \textbf{(Net2Vec~\cite{fong2018net2vec})} %framework studies the association of concepts to \textit{multiple} neural network filters. The work 
argues that semantic representations of concepts might be distributed across filters. Hence, filters must be studied in conjunction, not individually, as in ND~\cite{agrawal2014analyzing}. 
Net2Vec aligns concepts to filters of a CNN via a two-step approach.
For each concept, Net2Vec first collects filter activations of the network to explain when it is probed with input samples from a dataset annotated with concepts (e.g., BRODEN~\cite{agrawal2014analyzing}).
Then, Net2Vec performs an optimization process to either classify or segment the same concept starting from these activations. The resulting weights tell us how much each node is relevant for predicting the given concept. 
The results showed that combining filters allows to identify better concepts than using a single filter in both tasks, indicating that multiple filters better represent concepts. 
Moreover, filters are not concept-specific, but they can encode multiple ones. 
As a limitation, Net2Vec models the relationship between concepts and filters as linear, potentially failing to capture more complex and non-linear concept alignments. 


% \myparagraphbold{GNN-CI~\cite{xuanyuan2023global}}
\smallskip
In Graph Neural Networks Concept-based Interpretability \textbf{(GNN-CI~\cite{xuanyuan2023global})}, the authors extend the idea of node-concept explanations to the challenging graph classification scenario. In particular, they define concepts either as properties of a node in the graph (e.g., number of connected edges > 7) or as the class of the node (being an Oxygen atom) or of the neighbors (next to an Oxygen atom). 
For each neuron, they check whether its activation resembles the presence of any concepts. The resemblance is computed as the IoU between concept presence and neuron activation. Rather than considering a single concept, they allow each neuron to be described as a short composition of concepts, e.g., $\text{number edges} > 7\land \neg \text{is Oxygen}$. 
Furthermore, they produce an explanation of the final class in terms of the concepts as a linear classifier trained only on explained nodes to mimic the original classifier.
Finally, they also propose a concept visualization in terms of a graph concept activation map, a variant of Grad-CAM applied to a graph. 
The experiments show that extracted concepts are meaningful for graph classification. For instance, they reveal the presence of functional groups which are known to be correlated with the graph class. Also, they show that interpretable neuron activations are positively correlated to correct class predictions. %On the contrary, no correlation is found be

\subsection{Unsupervised Concept-based Explainability methods}
\label{sec:unsup_concept_exp}
Relying on a given set of supervised concepts is not the only way to assess whether a network is learning higher-level semantics. %These can also be discovered through the analysis of sample representations in the latent space of the network. 
Indeed, parts of the samples may represent practical explanations of a given prediction or of a learned class. 
As shown in Figure~\ref{fig:posthoc_unsup_classconc}, input pre-processing is normally necessary for these methods.
Afterward, unsupervised methods analyze sample representation in the latent space to identify clusters composed of parts of the samples (i.e., \textit{unsupervised concept basis}). 
% Again, as shown in Figure~\ref{fig:posthoc_unsup_classconc}, 
% 
Also, they analyze how these clusters contribute to the final prediction, thereby providing explanations in terms of Class-concept relations.
How the clustering is conducted differentiates the methods: they either employ standard K-means (ACE), Non-Negative Matrix Factorization (ICE), recursion on different layers (CRAFT), subspace clustering (MCD), concept completeness maximization (Completeness-aware), or assuming concept independency, or, finally, working on voxels from videos. 
This category bears similarities to standard XAI methods. However, they differ in not selecting features relying solely on their saliency or internal similarity (as with superpixels) but rather on their capability to represent common patterns existing in other input samples. 

% \textit{Unsupervised.}
% Unsupervised methods (Section \ref{sec:unsup_concept_exp}) seek to identify unsupervised clusters of samples (i.e., an \textit{unsupervised concept basis}), exerting influence on a given prediction, 
% or an entire class. Therefore, they generally provide explanations in terms of Class-concepts relations. This category bears similarities to standard XAI methods. However, they differ in that they do not select features relying solely on their saliency or internal similarity (as with superpixels) but rather for their capability to represent other input samples. Due to the limited number of unsupervised methods and since they all provide explanations in terms of \classconcrel, we do not define further subcategories in this case.  

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Images/posthoc_unsup_classconc.png}
    \caption{Unsupervised post-hoc methods extract unsupervised concepts in terms of parts of the same input samples. In particular, these methods provide class-concept relations analyzing the representations of these parts with respect to the output class in the latent space of the network.}
    \label{fig:posthoc_unsup_classconc}
\end{figure}


% \myparagraphbold{ACE~\cite{ghorbani2019towards}}
\smallskip
The Automatic Concept-based Explanations \textbf{(ACE~\cite{ghorbani2019towards})} method explains a class within a trained classifier, employing a probing strategy that does not require human supervision.
The process involves first segmenting images belonging to a specific class at multiple resolutions, encompassing textures, object parts, and complete objects, thus capturing a diverse spectrum of concepts.
Subsequently, the projection of image segments in the latent space of the network is clustered across different data.
Outlier sample projections are filtered out since they possibly represent insignificant segments or underrepresented concepts. 
Finally, the T-CAV importance score \cite{kim2018interpretability} is calculated for each group (i.e., a concept) to estimate the average influence of a concept on class prediction. 
The final output comprises the most pertinent concepts based on their T-CAV score. %and the score itself.
As recognized by the authors, however, ACE 
might find meaningless or non-coherent concepts due to segmentation, clustering, or similarity score calculation errors. 
With a human-based evaluation, however, they tested that the samples assigned by ACE to the same concepts are very coherent and can be labeled by a human employing, in general, the same words.   


%%%Completeness-aware
% \myparagraphbold{Completeness-aware~\cite{yeh2020completeness}}
\smallskip
While ACE allows the extraction of some concepts from a learned neural network, there is no guarantee that this set of concepts is sufficient to explain a prediction. In \textbf{Completeness-aware~\cite{yeh2020completeness}}, the authors propose a method for extracting complete concept-based explanations.   
% This research addresses a fundamental question: “Can concepts alone provide a sufficient explanation for the neural networks' prediction?”. The authors argue that the concepts are considered sufficient if the scores assigned to them serve as adequate statistics to explain the prediction of the overall model.
%%%How it works
%In this analysis, the authors contribute by defining \textit{Completeness}, introducing \textit{ConceptSHAP} proposing an innovative method for concept discovery. 
%It is crucial to highlight that merely selecting a concept relevant to a specific class does not guarantee its sufficiency in explaining a prediction. 
% In this context, sufficiency aligns with completeness. 
They define a completeness score as the amount to which
%The completeness score serves as a metric for assessing how efficiently 
% concept scores operate as statistical indicators for the model. %This is grounded in the assumption that the concept scores of 
concept scores are sufficient for predicting model outcomes. To measure the concept completeness, they propose to assess the accuracy achieved by predicting the class label, given the concept scores. 
With this in mind, they propose a 
%Using the concept of completeness as a guide, the suggested 
concept discovery algorithm is optimized to unveil maximally complete concepts. %Operating under the assumption that each data point comprises constituent parts and considering the spatial interdependence in input data, 
The algorithm also promotes proximity between each concept and its closest neighbouring patches to extract meaningful concepts. %To enhance the completeness of the revealed concepts, the algorithm optimizes a surrogate loss specifically designed for the completeness term. a metric for assesing the importance of each concept for a given class. 
Furthermore, the authors propose ConceptSHAP, a metric measuring the importance of each concept for a  given class. It modifies SHAP by replacing attribute importance with concept sufficiency in representing the class. 
%within a predetermined set of concept vectors with a high completeness score. ConceptSHAP takes its inspiration from Shapley, which is modified to attribute importance to each concept. ConceptSHAP is available in two versions: one evaluates the contribution of a concept within a fixed set of concepts, while the other calculates the salience of concepts by class.
%%%Results
%The evaluation focuses on the concept discovery algorithm. 
Using a synthetic dataset with complete concepts, the authors show that the proposed method excels in discovering the complete set of concepts, outperforming compared concept discovery methods, including ACE. %and k-means. 
% The proposed method in this study excels in finding complete concepts, outperforming others. Another evaluation involves image classification using the Animals with Attributes (AwA) dataset and text classification on the IMDB dataset with movie reviews labeled as positive or negative. The proposed concept discovery algorithm performs well, although it lacks a direct comparison with other methods.
%%%Insights


%%%ICE 
% \myparagraphbold{ICE~\cite{zhang2021invertible}}
\smallskip
Invertible Concept-based Explanation \textbf{(ICE~\cite{zhang2021invertible})} builds upon ACE to improve its concept identification and importance assessment algorithm.
ICE replaces K-means with Non-Negative Matrix Factorization (NMF) for extracting concept vectors. %It then employs a classifier on top to approximate the prediction of the explained model. 
Using NMF over the feature maps uncovers a concept for each reduced dimension. This allows ICE to employ a classifier on top to approximate the model outputs and yield concept importance as the weights of the linear approximation instead of using T-CAV scores. %from the concept to the model outputs. 
The approximation error (or the completeness of the representation, as defined in \cite{yeh2020completeness}) is much lower when employing the richer NMF concept representation than when employing Principal Component Analysis (PCA) or K-Means, which can also be seen as a form of binary dimensionality reduction. 
Similarly to ACE, 
the authors perform a user study to assess the interpretability of the extracted concepts. They ask participants to assign a few-word description to a group of images belonging to the same extracted concept.
The results show that ICE concepts are more interpretable than those derived from PCA or K-Means.


%%%CRAFT 
% \myparagraphbold{CRAFT~\cite{fel2023craft}}
\smallskip
Concept Recursive Activation FacTorization for Explainability \textbf{(CRAFT~\cite{fel2023craft})} extends the techniques introduced in ACE and ICE for unsupervised concept discovery. %to provide post-hoc explanations based on unsupervised concepts as a class-concept relation. 
Also, it offers the possibility of visualizing the unsupervised concepts that contributed to the final prediction. %via \textit{concept attribution maps}. 
%In particular, CRAFT specializes in offering an explanation that reveals 'what' and 'where' the model is looking for the prediction, in contrast to standard XAI techniques, i.e., saliency maps, that only say where are located in the image, pixels critical for the prediction. 
%%%What is
% CRAFT method comprises three main pillars:
% i) a method to recursively detect concepts and decompose them in sub-concepts across layers.
% ii) a novel method to estimate concept importance.
% iii) a method to create concept visualization.
%%%How it works 
% CRAFT addresses concept discovery by using, as previously done by ICE~\cite{zhang2021invertible}, Non-negative matrix factorization (NMF). 
% Specifically, from the input images, sub-regions are chosen to identify specific concepts in a localized context. 
In contrast to ACE and ICE approaches, in CRAFT, sub-regions are identified with a random crop %data augmentation 
technique.  
The activations from an intermediate layer of a neural network are calculated for each random crop. These are then factorized using the NMF technique to obtain %two smaller matrices. The first matrix contains the coefficients of the concepts, while the second matrix is called the \textit{concept bank} and contains the 
concept representations similar to ICE. % and concept importances. 
%This approach reinterprets the embedding of random crops as a composition of human-understandable concepts, making it more accessible for interpretation. 
Selecting the right layer to analyze is critical because concepts can manifest across multiple layers. To address this, CRAFT introduces a recursive approach to identifying concepts and sub-concepts. %The calculation of activations explained above involves the selection of the layer of the neural network. This choice is critical to identify concepts that can be integrated across multiple layers (as stated by Net2Vec). To solve this problem, the authors introduce a recursive approach. 
%Indeed, repeating the previous process of factoring the concept matrix on a previous network layer effectively leads to identifying sub-concepts of the original concept.
Concept importance for the final prediction is determined using \textit{Sobol} scores derived from sensitivity analysis.
% Formally, the Sobol score measured the contribution of each concept to the model prediction, measuring the fluctuations of the model's output in response to meaningful perturbations of the concept coefficients. Unused or less important concepts will not modify the new model output. 
%Finally, the importance that a concept may have as a main effect - together with its interactions with other concepts - is calculated on the model's output by calculating the expected variance that would remain if all concepts except the one considered were fixed. Although attribution techniques like saliency maps help identify the regions that the model deems significant for the decision, they do not provide details about the precise trigger.
For concept visualization, CRAFT employs a saliency map starting from the concept representation and highlighting the most influential parts in the input image for the concept.
% Finally, in ACE and ICE, concept visualization can be performed only be checking which subparts get clustered together. In CRAFT, the visualization is performed by means of %\textit{Concept attribution maps}. These show information about concept importance extracted from the two matrices obtained with NMF. 
%Specifically, given the concept scores and the concept bank, standard XAI methods, i.e. 
% a saliency map which locates the most influential parts in the input image for a given concept 
%that drove the network's decision. 
%%%Results
% Through human evaluation, the authors assess % the practical \textit{utility} and \textit{meaningfulness} of the framework. 
%The proposed CRAFT method's evaluation primarily involves assessing, through human evaluation, its practical utility within three distinct XAI scenarios using a human-centered benchmark.
%The 3 representative real-world scenarios are: (1) identifying bias in an AI system, (2) characterizing a visual strategy too difficult for an untrained human observer, (3) understanding complex failure cases.
%Specifically, they conducted psychophysical experiments to validate the usefulness and significance of the model for human experimenters. 
% To assess 
% the \textit{utility} of CRAFT explanations, by means of an external benchmark in which they measure how well the explanations assist users in inferring the general rules that guide classifications. %, and that can be easily transferred to unseen instances. 
%At test time, the \textit{utility} measures users' accuracy in predicting model decisions on novel images, averaged over three sessions. 
% In two out of three scenarios, CRAFT outperforms the \textit{utility} scores of attribution methods (e.g. Saliency, GradCAM) and ACE.
% To evaluate the \textit{meaningfulness} of the extracted concepts, human participants engage in a two-stage survey. The initial phase involves an intruder detection experiment, followed by a second phase designed to assess the effectiveness of the recursive concept hierarchy through a binary choice between a parent concept and a sub-concept. 
% The results demonstrate a level of performance in line with the authors' expectations and underline the positive outcome of the recursive concept extraction idea. 
A Human evaluation reports CRAFT's higher utility than standard XAI methods (e.g., Saliency, GradCAM) and ACE in two out of three scenarios. To assess the meaningfulness of extracted concepts, participants were required to detect intruder concepts and identify parent concept vs sub-concept identification to evaluate the effectiveness of the recursive approach.


%%%MCD 
% \myparagraphbold{MCD~\cite{vielhaben2023multi}}
% Multi-dimensional Concept Discovery (MCD) is yet another approach for extracting unsupervised concepts. % that allows establishing the completeness of extracted concepts. %Within the MCD framework, the concepts identified possess both local and global interpretability through a clearly defined completeness decomposition.
%%%What is
%Undoubtedly, the process of uncovering concepts in neural networks is intrinsically tied to the structures present in the activations of intermediate feature layers. In light of this connection, the initial innovation brought forth by MCD focuses on methods to break down the hidden feature space into discernible and meaningful concepts. 
%%%How it works
% In MCD, the concept discovery approach shifts from constrained methods like ND~\cite{bau2017network}—identifying concepts with canonical basis vectors for each convolutional channel—to more flexible techniques such as ICE~\cite{zhang2021invertible}, %allowing orthogonality with axis rotation, and finally to 
% TCAV~\cite{kim2018interpretability} or ACE~\cite{ghorbani2019towards}.%, where concepts can take arbitrary directions.
\smallskip
Multi-dimensional Concept Discovery \textbf{(MCD~\cite{vielhaben2023multi})} introduces multidimensionality in concept extraction by allowing concepts to span on a hyperplane across different convolutional channel directions. This is obtained by means of  
%MCD Concept discovery involves two steps: 
Sparse Subspace Clustering (SSC) for feature vector clustering and a subsequent PCA for cluster basis derivation. On top, a linear layer is employed (similarly to ICE) to mimic the final classification. This allows each sample to define a concept completeness score, quantifying the fraction of the model prediction that can be collectively recovered using the extracted concepts. %During testing, new feature vectors (e.g., from a new sample) are compared with concept bases. 
The MCD framework offers two explanations: concept relevance maps, indicating a concept's importance for class predictions, and concept activation maps, for concept visualization. %highlighting strong expressions in the input space.
%MCD ensures concise model explanations by organizing reasoning with concepts that cover the feature space without fragmentation. 
 %MCD requires fewer multidimensional concepts for a specified completeness level, offering more concise explanations than more restricted methods.
%%%Results
In the experiments, the authors show that MCD with an SSC clustering strategy overcomes other concept discovery methods (ICE, ACE) regarding concept faithfulness and conciseness. These are respectively defined as the reduction of the prediction when flipping the most important concepts and as the number of concepts required to reach a certain completeness score. 
%%%Insights


%%%When are post-hoc?
% \myparagraphbold{DMA \& IMA~\cite{leemann2023are}}
\smallskip
The objective of \textbf{DMA \& IMA~\cite{leemann2023are}} %"\textit{When are post-hoc conceptual explanations identifiable?}" 
is to devise a concept discovery method characterized by \textit{identifiability}, extending the idea from PCA and Independent Component Analysis (ICA) to conceptual explanations.
%%%What is
The authors define a method as \textit{identifiable} when it can provably recover all the concepts in a context where the components generating the data are known. %ensuring the reliability of explanations. When 
%a known number of ground truth 
% the concept discovery method yields concepts that correspond to the individual ground truth components and can represent an input in the concept space.
%%%How it works
% In this paper, the authors attempt to extend the idea of identifiability from methods like PCA and ICA to conceptual explanations. However, this proves unfeasible due to the presence of mutually dependent components. 
% The authors introduce two post-hoc discovery algorithms %based on \textit{disjoint} or \textit{independent} mechanisms 
%to address this issue. 
They propose Disjoint Mechanism Analysis (DMA), which ensures identifiability in compositional data generation where distinct components control distinct pixel groups in an image. DMA guarantees the recoverability %of ground truth components 
even if ground truth components are correlated (unlike PCA or ICA). However, it requires components to affect disjoint parts of the input, which should be true as long as the explained encoder is faithful to the generative process generating input data. The second approach, Independent Mechanism Analysis (IMA), %achieves independence %in data generation through a faithful encoder, differing 
represents a less constrained version requiring concept vectors %differing from the first one in handling the matrix containing the concept vectors, requiring them 
to be only orthogonal but not disjoint.
%%%Results
The results demonstrate that %the new concept discovery methods, IMA and DMA, 
IMA and DMA yield results comparable to PCA or ICA on datasets without correlated generative components and better on the contrary. %dataset with correlated components. 
Also, discovered concepts represent ground truth concepts more often than ACE and Completeness-aware.
However, it's worth noticing that DMA and IMA do not provide any of the explanations defined in Section~\ref{sec:expltype}: they only assess which concepts can be extracted from a neural representation. %whether it is an autoencoder or a classifier. 
%Notably, the authors contribute by highlighting a strategy for selecting the appropriate concept discovery algorithm based on the components and the presence of a faithful encoder.
%%%%Insights


%%%STCE 
% \myparagraphbold{STCE~\cite{ji2023spatial}}
\smallskip
Spatial-temporal Concept-based Explanation \textbf{(STCE~\cite{ji2023spatial})} provides concept-based explanations for 3D ConvNets, a domain less explored due to the computational complexity of handling video data. % and complexity.
%%%What is
% The STCE framework provides a global explanation, extending ACE's strategy ~\cite{ghorbani2019towards} from 2D images to video without discarding the spatio-temporal dimension. It also provides \concvisual{} by means of a qualitative assessment. 
%%%How it works
%First, videos are segmented into supervoxels for each class. %Differently from previous methods that relied on time intervals, the segmentation %using 3D SLIC, is performed at three resolution levels to capture a spectrum of information from fine-grained to coarse-grained actions. 
% Then, each supervoxel is fed into a 3D ConvNet to extract features. 
% Based on the extracted features, similar supervoxels are clustered together, defining spatial-temporal concepts. 
STCE directly extends ACE's 2D image strategy to the video domain without neglecting the spatio-temporal dimension. %It offers global explanations and \concvisual{} through qualitative assessments. 
The method involves segmenting videos into supervoxels for each class, extracting features with a 3D ConvNet, and clustering similar supervoxels to define unsupervised spatial-temporal concepts.
 Concept importance is determined using T-CAV scores, considering, as negative samples, random videos from non-related datasets.
% To determine which concept the network pays more attention to, the concept importance is calculated through CAVs~\cite{kim2018interpretability}.
% Interestingly, here, to calculate CAVs, the negative samples are represented by random videos from irrelevant datasets. 
%%%Results
% The STCE framework is evaluated on two action-centric video datasets: Kinetics-700 and the KTH Action dataset.
Similarly to previous works, the quality of the STCE explanation is assessed in terms of faithfulness by measuring the reduction of accuracy of the explained model when removing concepts associated with high T-CAV scores. 
%in the quantitative analysis the classification accuracy of the model is measured by adding or removing concepts according to the importance score. The findings demonstrate that adding concepts with higher importance scores positively influences final accuracy, while their removal significantly diminishes performance. Conversely, the inverse holds true as well.
For qualitative analysis, the authors present video frames illustrating detected concepts, particularly by highlighting video frames that feature the most and least important concepts for a given classification %highlights the remarkable consistency of the proposed framework.


% \subsubsection{\nodeconcass{}}
% Recently, a few methods aimed at providing node-concept explanations in terms of unsupervised concepts.  

% \myparagraphbold{CRP~\cite{achtibat2023attribution}}
% Concept Relevance Propagation (CRP) is a simple method aiming at explaining singular nodes within a network without employing a supervised set of concepts. 
% %approach combines the effect of local and global explanation answering both the \textit{where} and \textit{what} questions for individual predictions. 
% %%%What is
% They define as unsupervised concepts the same hidden nodes whose activations are the most important for a given classification. 
% CRP builds upon Layer-wise Relevance Propagation (LRP), a method that backpropagate the relevance of a decision until the input features. 
% In contrast, CRP define the relevance streams conditioned to the concepts.
% % CRP allows, by selecting a neuron (i.e., a concept), to reveal how relevance flows through the chosen network unit to lower-level concepts, offering insights into the importance of underlying building blocks for a given decision and a given concept.
% % For example, in the classification of the \textit{bee-eater} bird, the relevant concept \textit{animal on the branch } depends on previous concepts describing the branch, such as \textit{wood}, %and for the colorful plumage, such as \textit{colorful threads},
% % %learned through conditioned back-propagation. 
% % illustrating the composition of the final concept.
% It provides for concept visualization by means of relevance maps for a given node as well as concept atlas, i.e., input regions such as superpixels associated to the highest relevance for a given node (concept). %revealing their presence in an image and contribution to predictions. 
% %However, channel relevance and conditional concept maps of CRP do not identify the specific concept encoded by a channel. To solve this problem, 
% % The authors also introduce , 
% %ActMax: Method that searches for input images that result in the highest activation value of a specific network unit. with the aim of maximising concept relevance for the selection of representative samples of latent model features.
% To show which latent features the concept represents, the authors also RelMax, a method for finding the samples associated to the highest concept relevance.
% %%%How it works
% %CRP provides visualisation of concepts through the Concept Atlas. This tool effectively illustrates the most relevant concepts in specific regions of the input images. By selecting super-pixels as regions of interest, the method aggregates channel conditional relevance for each super-pixel, allowing for the derivation of regional relevance scores.
% %%%Results
% %To evaluate the practicality of CRP and RelMax, the authors conducted a human evaluation study. Participants had to judge whether the prediction of a model was affected by specific artefacts in the data, such as a thick black border around an image. Compared to four standard XAI methods (IG, SHAP, Grad-CAM, LRP), CRP and RelMax performed significantly better, allowing participants to reliably detect such influences. However, in a second assessment of participants' confidence in their assessments, CRP and RelMax produced lower confidence and clarity. The authors attribute this result to the complexity of the methods.
% To assess CRP and RelMax, the authors conducted a human study where participants judged the impact of data artifacts on model predictions. Compared to standard XAI methods (IG, SHAP, Grad-CAM, LRP), CRP and RelMax performed better in detecting influences. However, in a second assessment of participant confidence, CRP and RelMax yielded lower confidence and clarity, possibly due to method complexity.



% \subsection{Challenges of \conceptexp{}}
\subsection{Discussion}
\label{sec:posthoc_issues}
In the following, we report the critics that have been moved to the concept-based methods reviewed in this section and how, in particular, they affect their performance.  

\myparagraphbold{Do standard networks learn concepts?}
Several works in literature have disputed it \cite{koh2020concept, chen2020concept}
whether standard models actually learn symbolic concepts when trained to accomplish a different task. In particular, \cite{koh2020concept} tested the concept accuracy of a linear probe. We remember that a linear probe is a linear layer trained to predict the concepts in the latent space of an already trained model, as proposed in \cite{kim2018interpretability}. They found that linear probes achieve a lower concept accuracy with respect to a model trained to predict the concepts (91\% vs 97\% on the CUB dataset~\cite{} and 0.68 vs. 0.53 error on the OAI dataset). 
This result confirms that post-hoc concept-based explainability methods cannot ensure that the model actually learns symbolic concepts, as introduced at the beginning of this section. On the other side, they help to understand what the network is learning: the still high accuracy of linear probes implies that the model learned many concepts. 

%CW: they assume that the latent space places members of each concept in one easy-to-classify portion of latent space. Since the latent space was not explicitly constructed to have this property, there is no reason to believe it holds.


\myparagraphbold{Different probe datasets provide different explanations}
In \cite{ramaswamy2023overlooked}, the authors tested the importance of the dataset choice in extracting the explanations.  
They have shown that different probe datasets lead to different explanations even when explaining the same model using the same interpretability method. This issue arises for methods explaining both node-concept associations and class-concept relations. As an example of the first type, they show that ND label neurons differently according to the dataset employed (ADE20k or Pascal): while in some cases, the concepts are still similar (e.g., \textit{plant} vs \textit{potted-plant}, \textit{computer} vs \textit{tv}), in other cases are profoundly different (e.g., \textit{chair} vs \textit{horse}, \textit{tent} vs \textit{bus}).
As an example of the second type, they show that the T-CAV concept activation vectors extracted from different datasets are projected in different directions. To numerically assess this, they compute the cosine similarity between the vectors representing the same concept but extracted from ADE20k and Pascal, and they show that while for same concepts the similarity score is quite high (\textit{ceiling} 0.27), for others it is very low (\textit{bag} 0.01, \textit{rock} -0.02), with a cosine similarity of common concept vector lower than 0.1 on average.
As we also highlighted in Section \ref{sec:categorization}, they suggest that the probe dataset should be chosen carefully and specifically recommend probe datasets that closely resemble the data distribution of the dataset on which the model was originally trained.


\myparagraphbold{Post-hoc concept-based explanation methods are vulnerable to adversarial attack}
In \cite{brown2023making}, Concept-based post-hoc explainability methods, much like their standard XAI counterparts \cite{kindermans2019unreliability,ghorbani2019interpretation, slack2020fooling,adebayo2021post}, are susceptible to adversarial perturbations. 
This study focuses primarily on supervised methods that explain class-concept relationships using linear probes, such as TCAV. The underlying idea is that a sample can be crafted to change the interpretation while maintaining the same classification. In particular, they show that an attack can induce a positive interpretation with respect to a concept, such as making a \textit{Corgis} important for the classification of a \textit{Honeycomb}. At the same time, they also provide examples of negative interpretation, such as making \textit{Stripes} not important for classifying a \textit{Zebra}. Notably, the authors also demonstrate that these attacks maintain some level of effectiveness even in black-box scenarios, i.e., when the adversarial samples are created for a different model to the one they are tested on, which is a more realistic scenario.   

\section{\conceptmodel{}} % 12 pages
\label{sec:concept_model}

\conceptmodel{} introduces a deviation from standard neural network training practices. They explicitly represent concepts within the same neural network architecture. We define them as explainable-by-design since they inherently provide Node-concept associations (N-CA) (except for some cases). 
They typically employ a dedicated hidden layer to predict concept scores to this aim. These scores represent numerical values quantifying the relevance or presence of specific concepts in a given input sample and condition the model's output. The same concept scores can also be studied in relation to the output classes to define Class-Concept Relations (C-CR) and can be visualized through Concept-Visualization (C-Viz).  
 %, and it inherently shapes the nature of the explanations the model can offer. 

How the intermediate representation is defined varies according to the concept annotations and, consequently, the concept types. As shown in Table~\ref{tab:summary:bydesign1}, %the main features of each approach based on the categorization outlined in Section~\ref{sec:categorization}.
% As we can see from Table~\ref{tab:summary:bydesign1}, 
% Concept-based models primarily differ in whether 
Concept-based models either employ a dataset with annotated concepts (Supervised, Section~\ref{sec:sup_concept_model}), without concept annotations (Unsupervised, Section~\ref{sec:unsup_concept_model}), with annotations for few concepts only (Hybrid, Section~\ref{sec:sup_unsup_cbm}) or they generate the supervision by means of an external model (Generative, Section~\ref{sec:generative}). 
Furthermore, if they employ annotated symbolic concepts (Symb.), they differ according to whether they employ them during training (Joint) or afterward to instill them in a trained network (Instil). If they automatically extract concepts, they differ for the type of concepts extracted, either clusters (Uns. Basis) or prototypes (Proto.). If they adopt a hybrid approach, they generally employ both symbolic and unsupervised basis concepts. Finally, if they generate concept annotations, these are normally Textual concepts.   
Concept-based models have been mostly developed to solve classification tasks (CLF), with one also performing regression (REG) and another clustering (CLU). Similar to the post-hoc method, in this case, the network's backbone is mostly a CNN working on images (IMG), possibly reconstructing the data with an auto-encoder (AE). Some works employ a fully-connected network working on tabular data (TAB), GNN on graphs, and transformer (TRANS) working on both images and texts (TXT).
To summarize the key aspects of concept-based models, we now discuss their main advantages and disadvantages compared to post-hoc methods.

\input{Tables/table_by_design_1}

% Concept-based Models are explainable-by-design models that incorporate an explicit representation of the concepts inside the network architecture. Therefore, all these methods intrinsically provide \nodeconcass. The model's output is always based on this intermediate representation. 
% % The way in which this representation is defined varies according to the concepts employed, and it inherently shapes the nature of the explanations the model can offer. 
% In the upcoming subsections, we will explore four distinct approaches, each utilizing a different type of concept annotations: \textit{Supervised} (Section \ref{sec:sup_concept_model}), \textit{Unsupervised} (Section \ref{sec:unsup_concept_model}), \textit{Supervised and Unsupervised} (Section \ref{sec:sup_unsup_cbm}), and \textit{Generated} (Section \ref{sec:generative}).


\myparagraphbold{Advantages}
Concept-based Models offer the advantage of ensuring that the network learns a set of concepts explicitly. 
% For this reason, they generally provide explanations in terms of Node-concept associations by-design. 
%The predictions they provide, therefore, can always be analyzed in terms of these concepts. 
Furthermore, %they facilitate interaction with the network through concept intervention~\cite{koh2020concept}. 
a domain expert can modify the predicted values for specific concepts and observe how the model's output changes in response. This process is referred to as \textit{concept intervention}, and it enables the generation of counterfactual explanations. %For example, it allows understandings like “If the model did not consider the joint space too narrow for this patient, it would not have predicted severe arthritis”~\cite{koh2020concept}.

\myparagraphbold{Disadvantages}
On the other hand, these methods can only be employed when there is flexibility to train a model from scratch, possibly tailoring it to the specific task at hand.  Furthermore, in simpler solutions, the predictive accuracy of concept-based models may be lower than that of standard black-box models. Further issues and challenges of concept-based models will be analyzed at the end of the section (Section \ref{sec:cbm_issues}).


% \myparagraphbold{Sub-categories}


\subsection{Supervised Concept-based Models}
\label{sec:sup_concept_model}
Supervised Concept-based Models employ a dataset annotated with symbolic concepts (like attributes of the output classes) to supervise an intermediate layer explicitly representing the concepts. 
% The symbolic concepts must be supplied through additional annotations during training to achieve this. 
% We categorize the approaches based on when the concept information is employed: during the training as a \textit{joint-training} (Section~\ref{sec:sup_joint_train}) or via post-hoc tuning of the intermediate representations in \textit{post-hoc concept tuning} strategy (Section~\ref{sec:sup_concept_instill}). 
%the concepts can still be integrated into the network architecture through a \textit{post-hoc concept tuning} approach.  
% \textit{Supervised.}
When these annotations are readily available within the same training dataset, a \textit{joint concept training} strategy can be employed (Section \ref{sec:sup_joint_train}). 
Otherwise, they can also be embedded in the model through separate training on an external dataset dedicated solely to concept learning to perform a \textit{concept instillation} (Section \ref{sec:sup_concept_instill}). 


\subsubsection{Joint concept training} \label{sec:sup_joint_train}
 As shown in Figure~\ref{fig:cbm_sup_jt}, supervised concept-based models employ concept annotations to supervise an intermediate representation and increase the transparency of the model. %Historically, these annotations have been used in multi-label classification scenarios to supervise further classes.
 Unlike methods performing concept instillation, the training is performed \textit{jointly} for the target task (e.g., image classification) and for concept representation.
 This requires employing a training dataset that includes annotations about both the main classes (e.g., Parrot) and the related attributes (e.g., Feather, Beak, Foot, Muzzle).  
 Concepts can be represented by means of a single neuron (CBM, LEN) or through an embedding (CEM, ProbCBM, DCR), which avoids performance loss with respect to a black-box model. As shown in the picture, these methods can also analyze the relations between concepts and classes through concept importance (CBM, ProbCBM) or logic relations (LEN, DCR).    

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{Images/cbm_sup_jt.png}
    \caption{Supervised Concept-based Models jointly training output classes and concept representation on a dataset where both class and concept annotation is provided.}
    \label{fig:cbm_sup_jt}
\end{figure}


%\myparagraphbold{CBM~\cite{koh2020concept}}
\smallskip
The first work proposing a joint task-concept training strategy is attributed to
%for supervised explainable-by-design concept-based models is attributed 
Concept-Bottleneck Model \textbf{(CBM~\cite{koh2020concept})}, where %, as illustrated in Figure~\ref{fig:cbm}. 
the authors modify the typical end-to-end neural architecture mapping from an input to a target by introducing an intermediate \textit{concept bottleneck} layer. 
This layer has neurons dedicated to learning and predicting a set of human-specified concepts from input features. A task function then predicts the final target, relying only on concept prediction (concept scores). 
Specifically, %during the training phase, a CBM is trained on samples in which the input is labelled with both the concepts and the target.
a double loss is optimized, penalizing wrong predictions in both the output and concept bottleneck layers. %creating a mapping function $f: X \rightarrow C \rightarrow Y$. 
% During the testing phase, the CBM takes an input $x$, predicts concepts $\hat{c}$, and employs these predicted concepts to predict the target variable $\hat{y}$. 
% For example, in Figure~\ref{fig:cbm}, the model uses clinical concepts to predict the severity of osteoarthritis.
%In this particular case, the authors used bird attributes as concepts in the first scenario, which involved fine-grained bird classification. In the second scenario, which focused on evaluating osteoarthritis, they employed joint conditions as the concepts. 
CBM design enhances the model's transparency and enables interaction with the model itself. 
A domain expert may intervene in the predicted concepts, allowing potential adjustments to the model's predictions. 
This process is referred to as \textit{concept intervention}. 
Concept interventions also facilitate the extraction of counterfactual explanations by manipulating the concept predictions and observing the model's response on the counterfactual concept representation. 
% For example, we can investigate scenarios such as, “If the model did not perceive the joint space as too narrow for this patient, it would not have predicted severe arthritis.”\cite{chen2020concept}. 
CBMs, however, are affected by two main limitations. 
i) CBMs provide class-concept relations only when employing a single layer to model the task function. In this case, the importance of a concept corresponds to the weight connecting the concept to the final class, as shown in Figure \ref{fig:cbm_sup_jt}. %However, the readability of concept importance scores has been disputed in~\cite{jain2022extending}, particularly when employing many concepts.  
ii) The generalization capability of CBM is lower than standard end-to-end models. This is mainly due to the bottleneck layer where each concept is represented by a single neuron~\cite{mahinpei2021promises}. This limit becomes more severe in contexts with few concepts available and when employing a shallow task function.
% Moreover, a limitation shared among the supervised joint training approaches is that they necessitate annotated concepts during training, which may not always be readily accessible. 
% Nonetheless, the authors suggest that working with a smaller yet robust set of concepts can still attain the desired accuracy. 
%This implies that gathering a smaller number of high-quality samples is feasible while achieving the desired accuracy. 
%This proves particularly beneficial in medical contexts where acquiring new training samples might entail invasive procedures for the patient.


%\myparagraphbold{LEN~\cite{ciravegna2023logic}}
\smallskip
In a series of works, the authors address the first issue by means of a framework named Logic Explained Networks \textbf{(LENs ~\cite{barbiero2022entropy, ciravegna2023logic})}. 
LENs improve the explainability of CBMs. These models, indeed, are trained to provide explanations in terms of First-Order-Logic (FOL) formulas associating task functions with the concept having the highest influence on it. To achieve this goal, they impose architectural constraints enforcing sparsity in the weights of the task function. As an example, on a bird classification task, a LEN may provide explanations of the type $\text{billShapeHooked} \land \text{mediumSize} \land \neg \text{throatColorWhite} \Leftrightarrow \text{blackFootedAlbatross}$. 
While most of the other works focus on vision tasks, LENs can be applied to tabular data and textual data \cite{jain2022extending} without a concept extractor, i.e., without requiring a module explicitly mapping the non-interpretable input data to a concept space. LEN can consider the same input data as concepts when they are associated with human-understandable symbols. 
%Another distinct factor compared to other works is that 
Furthermore, LEN can solve clustering tasks %starting from concepts the LEN can be employed to  
% In this context, a LEN assigns data points to specific clusters and
and provide logic explanations about cluster assignment in terms of frequent concept relations~\cite{ciravegna2023logic}.
Finally, logic explanations can be used to defend a LEN from an adversarial attack by checking the consistency of the test-time predictions with the explanations extracted at training time.
% The accuracy of LENs, however, is still lower than the one provided by black-box networks since they are still based on a concept-bottleneck architecture. 
% Limitations?


%\myparagraphbold{CEM~\cite{zarlenga2022concept}}
Concept Embedding Models \textbf{(CEM~\cite{zarlenga2022concept})} improve CBM performance by using an entire set of neurons to represent a concept (concept embedding). CEM obtains the same classification accuracy of black-box neural networks while retaining the possibility to employ and interact with a concept-based model. Unlike CBM, CEM performance does not decrease when the number of employed concepts decreases, showing a very high concept efficiency.
A naive solution to the performance loss issue of CBM is adding a separate set of unsupervised neurons \cite{mahinpei2021promises}, encoding information about the task function. % and bridging the performance gap.
However, as shown in CEM, this hybrid solution loses the possibility of interacting with the network. % since intervening on the concepts does not affect the task functions. 
According to CEM authors, in the hybrid configuration, the task functions only rely on unsupervised neurons, nullifying the effects of concept interventions on the task function. 
%, i.e., they allow the employment of a concept-based architecture even when very few annotated concepts are available.
% A naive solution to the performance loss issue of CBM is adding a separate set of unsupervised neurons \cite{mahinpei2021promises}, encoding information about the task function and bridging the performance gap. %These can encode more information regarding the task function and thus bridge the performance gap of CBM. 
% However, as shown in~\cite{zarlenga2022concept}, this hybrid solution loses the possibility to interact with the network since intervening on the concepts does not affect the task functions anymore. According to the authors, this behaviour is due to the fact that the task functions mainly rely on unsupervised neurons in the hybrid configuration.  
%In~\cite{zarlenga2022concept}, the authors proposed Concept Embedding Models (CEM) which overcomes 
% Concept Embedding Models (CEM)~\cite{zarlenga2022concept}, instead, overcome this limitation by using an entire set of neurons to represent a concept (concept embedding). This allows to retain the same classification accuracy of neural networks trained without concepts, while retaining the possibility to interact with the network. Unlike CBM, CEM performance does not decrease when decreasing the number of employed concepts, showing a very high concept efficiency. %, i.e., they allow the employment of a concept-based architecture even when very few annotated concepts are available. 
In CEM, the authors also introduce the Concept Alignment Score to measure the quality of a concept representation in describing a set of concepts. More precisely, it measures the entropy reduction in the concept space when a concept representation is provided. %(more details in Section \ref{sec:metrics}). 
They show that CEM concept alignment to the real concept distribution is close to the one provided by CBM and much higher than the hybrid solution.

%\myparagraphbold{ProbCBM~\cite{kim2023probabilistic}}
\smallskip
When concepts used to make the final predictions are not visible in the input sample, a deterministic prediction of the concepts may damage %the reliability of 
both the final task prediction and the explanation based on the concepts. 
To solve this problem, the Probabilistic Concept Bottleneck Model \textbf{(ProbCBM~\cite{kim2023probabilistic})} employs probabilistic concepts to estimate uncertainty in both concept and class predictions. %This innovative model offers interpretability through explanations based on the concepts and their associated uncertainties. Furthermore,
% ProbCBM also provides the uncertainty of the class prediction, which can be derived directly from the uncertainties of the concepts. 
%%%What is
% Ambiguity problems exist when the concepts that are used by the model to make the final prediction are not always visible in the input sample, and therefore, the model cannot predict their presence or absence. In such cases,
%%%How it works
Similarly to CEM, ProbCBM also employs concept embedding. However, given an input, ProbCBM outputs mean, and variance vectors %makes probabilistic concept embedding 
for each predicted concept. Concepts are then represented as multivariate normal distributions. The probability of % the existence (or absence) of the 
each concept is calculated via Monte-Carlo estimation by sampling from the distribution and computing the mean distance from the true and false concept vectors. Class predictions are similarly computed, generating a class embedding from the concept embeddings. %The concept and class predictor are trained separately. 
The uncertainty quantification in ProbCBM is done by calculating the determinant of the covariance matrix, which represents the volume of the probabilistic distribution. 
%%%Results
% ProbCBM was evaluated on a synthetic dataset proposed by the authors and on two real-worlds, CUB and AwA.
% In the first scenario, by inducing training ambiguity with a clipping augmentation method, ProbCBM achieves an accuracy of 99.8\% in both concept and class prediction. The results also confirm that high uncertainty of the estimated concept corresponds to ambiguity in the prediction of the relevant concept, resulting in increased uncertainty in the final classification. In the second scenario, 
ProbCBM's performance is compared with CBM~\cite{koh2020concept} and CEM~\cite{zarlenga2022concept}. ProbCBM outperforms CBM in classification accuracy but falls short of CEM. Regarding concept prediction accuracy, it is on par with CBM and better than CEM, demonstrating that integrating uncertainty through probabilistic embedding doesn't compromise performance. %Additionally, it slightly surpasses CEM, despite having fewer parameters
%%%Insights



%\myparagraphbold{DCR~\cite{barbiero2023interpretable}}
\smallskip
Even though CEM and Prob-CBM enhance the performance of standard CBMs, %it is important to note that 
they worsen the underlying explainability. When employing embedded concepts, even with the use of a shallow network, the interpretability of the task function is compromised since the dimensions within a conceptual embedding lack a direct association with a symbolic meaning. %and we cannot assess the concept importance looking at the weights of the task function.
% The trade-off between model interpretability and capacity can potentially lead to a decrease in human trust when working with such models. 
In response to this challenge, Deep Concept Reasoner \textbf{(DCR~\cite{barbiero2023interpretable})} is introduced  %, representing the first 
as an interpretable concept embedding model. 
Starting from concept embeddings, DCR %incorporates differentiable and learnable modules that, 
learn differentiable modules which output for each class and each sample a different fuzzy rule. These rules are then executed, taking into account the concept activations. %Differently from the concept embeddings, the concept activations are semantically meaningful. 
As a result, the model outputs an interpretable prediction regarding the concepts, even though only locally. %Since the rule is built on the concept embedding, indeed, the network may provide a different prediction even with the same concept activations. 
DCR achieves task accuracies on par with CEM and higher than CBM. The authors also show that in contexts where ground truths rule are available, DCR can recover them. %logic rules that align with ground truths. %, even when training concept supervision is unavailable. 
Compared with LIME and LEN, DCR facilitates the generation of counterfactual examples, and extracted explanations are less sensitive to input perturbations. %: on average, it is sufficient to change the prediction of a few concepts to get the model providing a different prediction. , the authors show that is easier to extract counterfactual explanations and that DCR explanations are less sensitive to input perturbation. %enhancing its utility and interpretability. 
Finally, they showcase that DCR can also work on graphs employing GNN as a backbone. In this case, they extract concepts post-hoc from a trained GNN by means of a Graph-Concept Explainer~\cite{magister2021gcexplainer}, a variant of ACE for graph structure. %, where each concept corresponds to a cluster of graph nodes in the embedding space. The authors then train a GNN to map these extracted concepts in a supervised way and provide with DCR the final predictions by means of a logic relations in terms of these concepts.




\subsubsection{Concept Instillation} \label{sec:sup_concept_instill}
This class of approaches considers the case where concept information is not available in the training set, but it is available from an external data source, such as a separate supervised dataset (CW, CT), a semi-supervised one (CME), or a knowledge graph (PCBM).  
As shown in Figure~\ref{fig:cbm_sup_ci}, the process is composed of two steps: 1) a black-box network is standardly trained end-to-end; 2) through \textit{Concept Instillation}, a given layer of the network is modified to represent concepts. At test time, this process still allows the employment of a concept-based model. Similarly to jointly trained models, concepts can be represented by means of single nodes (CW, CME, PCBM) or through concept embeddings (CT). They also provide class-concept relations if they replace the classifier head with an interpretable task predictor (CME, PCBM, CT).
%The introduced concepts are separated from the labels of the primary classification problem and can be sourced from a supplementary dataset where these concepts are annotated.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/cbm_sup_ci-2.png}
    \caption{Supervised Concept-based Models instilling concept in the network after a first end-to-end network training. Concept representation is either extracted from the network itself with post-hoc C-XAI techniques or from an external source (e.g., a knowledge graph).}
    \label{fig:cbm_sup_ci}
\end{figure}

%\myparagraphbold{CW~\cite{chen2020concept}}
% The first method proposing to create a post-hoc concept instillation is 
\smallskip
Concept Whitening \textbf{(CW~\cite{chen2020concept})} modifies a hidden layer of a neural network after it has been trained in such a way that it also predicts a given set of concepts. 
%It aims at enhancing the ability to comprehend the interpretability of the computation inside a neural layer and leading up to that particular layer. 
Usually, CW can be used to replace the Batch Normalization (BN) layer in a CNN because it combines batch whitening (decorrelating and normalizing each dimension) with an extra step involving a rotation matrix to align the concepts with the axes. %When integrated into a CNN, the CW module ensures that the latent space aligns with a specific set of concepts the user provides. 
%Rather than assuming that the latent space naturally supports disentanglement as done by \conceptexp{} extracting \classconcrels, CW proactively shapes through training the latent space (i.e. the output of a hidden layer) to represent the concepts. 
The underlying idea is that axes of the latent space should align with concepts, allowing each point within the space to correspond to and be interpreted through known concepts. 
Further training on the standard classes is required to avoid loss in the final task performance.
%The concept alignment step may be performed either during training time or by means of post-hoc tuning after standard training.
% In CW, the concept alignment step is performed as a post-hoc tuning after standard training. 
% While the primary classification dataset can have concepts annotations, it is not a requirement. %Similarly, the primary classification labels are unnecessary for the auxiliary dataset used for concept identification. 
An interesting aspect of CW is its capability to determine how a network captures a concept across different layers, as it can be applied after any layer.  
The authors show that a network produces more abstract and fundamental representations in the lower layers. 
%The authors point to an example of an airplane image. This representation is rather vague in the early stages of the network, marked by white or grey shapes against a blue background. The network can only recognize the “airplane” in the subsequent, more sophisticated layers. 
The authors compute the concept purity as the 1-vs-all AUC score on the test concept predictions to evaluate interpretability. 
A comparative analysis against concept-based post-hoc methods (TCAV, IBD) % in terms of concept purity. %, and filters in standard CNNs. 
% For TCAV and IBD, the AUC score was computed based on sample projections onto the concept vectors. %provided by the two methods. 
%The findings 
indicate that the concepts acquired with CW exhibit higher purity. % than those obtained via the other methods. %We claim that this is due which do not fine-tune the previous layer to represent the concepts. 
% Motivation of why
This result is attributed to the inherent orthogonality of CW conceptual representations and the impact of the entire model fine-tuning process.
% These results underscoree the significance of concept purity, as pure axes allow for the concentration of a concept's signal solely along its axis, in contrast to standard CNNs, where the concept may be dispersed throughout the latent space. %than those from alternative methods.

% Concept importance




%\myparagraphbold{CME~\cite{kazhdan2020now}}
\smallskip
Similarly to CW, the Concept-based Model Extraction \textbf{(CME~\cite{kazhdan2020now}) }also proposes to derive an interpretable model from a black-box.  
% This work introduces the Concept-based Model Extraction (CME) framework that unifies two XAI approaches, the concept-based and the model extraction. Model extraction methods are defined as those that approximate black-box models with simpler models to provide explanations.
%%%What is
% The CME framework deviates from the conventional concept-based models (CBM~\cite{koh2020concept}) because it leverages existing DNN models for extracting concepts and explaining predictions.
%While models like CBM~\cite{koh2020concept} propose methodologies for constructing concept-based DNN models, CME adopts a distinctive approach by leveraging existing DNN models for comprehensive analysis.  
% Moreover, CME can use partially-labelled data in a semi-supervised fashion and can efficiently use knowledge from pretrained DNNs to learn which concepts are (or are not) required for a given task.
%%%How it works
CME trains a concept extractor starting from the hidden representation of a given DNN.
To reduce the concept annotation effort, CME employs only a small annotated dataset and trains the concept extractors in a semi-supervised fashion. Interestingly, the authors repeat the extraction process of each concept for different hidden layers, retaining the one providing the higher concept accuracy. 
The predicted concept scores are employed as input for an interpretable task predictor, which is trained to mimic the task prediction of the original model.  
% In this study, the authors characterize a DNN as concept-decomposable when it can be accurately represented by the interplay of two functions \textit{p} and \textit{q}: one mapping inputs to concepts and another mapping concepts to outputs, mirroring the CBM approach. However, CME explores the possibility of a DNN being concept-decomposable by evaluating its approximation with an \emph{extracted model}.
% The function \textit{p} is generated by aggregating the predictions of the concept labels in the various layers of the DNN model. As CME utilizes both labeled and unlabelled concepts, it exploits Semi-Supervised Multi-Task Learning (SSMTL) to predict concept labels from the hidden space of each layer. This function \textit{p} encapsulates the concept information contained in a given DNN model, enabling the analysis of information representation and the prediction of concept values for new inputs. 
% In the end, through function \textit{p}, a labeled dataset with concept labels and classification outputs is obtained. This dataset is then employed to train \textit{q} in a supervised setting. Through \textit{q}, classification output labels are predicted based on the concepts predicted by \textit{p}.
% As extracted models, for the function \textit{q},
For the task function, the authors employ Decision Trees and Logistic Regression. 
Since they directly work on concepts, they both allow concept intervention at test time.
%Overall, the \textit{q} can be used to analyze how a DNN uses concept information to make predictions. 
%%%Results
% CME evaluation occurs on two datasets: dSprites, with full knowledge of essential concepts for maximum accuracy, and Caltech-UCSD birds, where this knowledge is lacking. The assessment involves the functions \textit{p} and \textit{q}, and 
CME's performance is compared with Net2Vec~\cite{fong2018net2vec} and CBM~\cite{koh2020concept} frameworks. CME significantly outperforms Net2Vec in task accuracy while remaining comparable to CBM.
%%%Insights
% In the CME framework, 
The authors also introduce a new metric, the MisPrediction Overlap (MPO), %This metric assess how concept mispredictions are distributed across test samples, especially in scenarios with numerous concepts. 
%The MPO calculates the fraction of test samples with at least \textit{m} mispredicted relevant concepts. 
to compute the portion of samples with at least \textit{m} concepts inaccurately predicted. 
% The results reveal that, 
Based on MPO, CME performs similarly to Net2Vec but falls behind CBM. 


%\myparagraphbold{PCBM~\cite{yuksekgonul2022posthoc}}
\smallskip
%Given the intensive nature of the annotation process, concept annotations are not always readily accessible.
%When this happens, it is possible to use Post-hoc Concept Bottleneck Models (PCBM)~\cite{yuksekgonul2022posthoc}. 
Post-hoc Concept Bottleneck Models \textbf{(PCBM~\cite{yuksekgonul2022posthoc})} implement two modalities to extract concepts: (i) from other datasets, similarly to CW~\cite{chen2020concept}, and (ii) from a knowledge graph and then encoded in the network by means of a textual encoder. 
In the first scenario, Concept Activation Vectors (CAVs) are employed to learn the concept representations in the latent space of a model pretrained on the final task. 
%The concept annotations employed can either be predefined by domain specialists or autonomously derived from data, similar to the ACE approach. %\todo{lo mostrano poi questo?}. 
% Crucially, it is worth highlighting that,
%Similarly to CW~\cite{chen2020concept} and in contrast to joint-training strategies (e.g., CBM~\cite{koh2020concept}), the samples might differ from the data used to train the backbone model. % encompasses both positive and negative instances of concepts. 
In the latter scenario, the authors employ an open-access 
knowledge graph (e.g., ConceptNet~\cite{speer2017conceptnet}), to gather concepts in relation %(i.e., hasA, isA, partOf, HasProperty, MadeOf) 
with the queried classes. %(e.g., "stripes", "horse" concepts for the "Zebra" class). 
They then obtain a vectorial representation of the concepts by means of a text encoder. 
% As shown in Figure~\ref{fig:post-cbm}, 
In both scenarios, the concepts are projected in the latent space of a pretrained model. The projections then train an interpretable task predictor, providing class-concept importance. %The usage of interpretable prediction is an essential property of the PCBM framework %This feature is desirable and invaluable, 
%as it sheds light on the concepts the model leans on for decision-making. 
% Similarly to concept intervention, a domain expert can detect an anomaly or counterintuitive behavior within the predictor and correct it to enhance the overall model. 
In addition to concept intervention, PCBMs also allow for \emph{global model edits}, %, being more efficient than previous works that involved only local interventions (e.g., CBM~\cite{speer2017conceptnet}). 
% The model can undergo
global modifications, which enables the model %based on feedback informed by learned concepts, enabling it 
to adapt its behaviour to novel scenarios, including shifts in data distributions. 
%Unlike other model intervention techniques, like in CBM, this one does not require data from the training or target domains, which is especially useful when data is scarce or inaccessible. 
%With a trained PCBM, global intervention can be made to the conceptual bottleneck by manipulating the concept weights. The authors outline three distinct global intervention strategies and an editing experiment under human guidance. All of these approaches enhance the final accuracy. 
Similarly to~\cite{mahinpei2021promises}, the authors propose to employ an unsupervised set of neurons to improve network scaling. % (bottom branch of Figure~\ref{fig:pcbm}). 
This time, however, they propose to employ a residual fitting, such that the hybrid prediction still has to rely on the interpretable one.
% They indicate this approach as capable to improve concept bottlenecks' usability and expressiveness. 
With respect to the original model, PCBM performances are slightly worse, but still comparable. % (CLIP-ResNet50, ResNet18, Inception, etc.).


%\myparagraphbold{CT~\cite{rigotti2022attentionbased}}
\smallskip
% ConceptTransformer (CT)~\cite{rigotti2022attentionbased} is an explanatory module designed to provide output class predictions as well as explanations in terms of symbolic concepts.  
% These \classconcrel{} are provided in terms of the attention scores between the output class and a set of user-defined high-level concepts. 
% A key feature of the attention module is its ability to reveal the underlying logic of the provided result.
% Within CT, the authors introduce an abstraction from the conventional role of attention, moving from low-level input characteristics to high-level concepts.
ConceptTransformer \textbf{(CT~\cite{rigotti2022attentionbased})} substitutes the task classifier of a DNN % head in any deep learning architecture 
with an attention module enriched with concept embeddings. Instead of being extracted from a knowledge base as in PCBM, concept embeddings in CT come from a transformer model trained on a dataset annotated with user-defined symbolic concepts.
The output of the attention module represents concept scores. A linear layer is employed on top to predict the final classes. 
CT provides \classconcrel{} in terms of the attention scores between the output class and the concepts embeddings. 
% The resultant model can be trained end-to-end %with no extra training pipeline overhead, except for 
% introducing an explanation loss that ensure the coherence of the explanation.
However, CT does not provide \nodeconcass{} since it does not explicitly represent concepts by means of a set of nodes but only with concept embeddings. % within the network . In CT, indeed, concepts are only represented in terms of concept embeddings.
% The authors claim that CT explanations are inherently \textit{Faithful} \cite{lakkaraju2019faithful} and \textit{Plausible} \cite{guidotti2018survey}. In this context, \textit{Faithfulness} measures 
% the degree to which an explanation locally mirrors the model's decision. %, ensuring an understanding of the model's functionality. 
% \textit{Plausibility} evaluate how convincing the explanation is to humans.
% how much the explanation is aligned with human reasoning
%focuses on the power of the interpretation to persuade human observers. 
% More precisely, they claim that \textit{faithfulness by design} is rooted on the linear relationship between the transformer value vectors representing concepts and their influence on the classification log probabilities.
The authors claim that their model is faithful by-design since it employs a linear layer from concepts to classes, similar to CBM. 
% \textit{Plausibility} is accomplished by construction through explicit guidance of the attention heads. %, directing them to attend to input concepts known as informative a priori. 
To obtain more plausible explanations, they also propose supervising attention scores so that concept-output relationships align with domain knowledge. 
% This construction is achieved by supervising the cross-attention mechanism's attention heads to adhere to input-concepts-output relationships derived from domain knowledge. 
%Performance comparison is made only for the CUB-200-2011 dataset. In the end, CT surpasses all state-of-the-art approaches whose performance values were identified by \textit{Li et al.} \cite{li2018deep}.
CT classification performance matches end-to-end black box models. %the state-of-the-art techniques therefore, it does not decrease the model's performance. 
Leveraging the concepts with CT seems to even boost the performance in contexts where the set of concepts is well-defined, and the relationships with the final classes are known (as in the case of CUB-200-2011 dataset \cite{welinder2010caltech}). 
%Moreover, the paper results on the CUB-200-2011 dataset \cite{welinder2010caltech} show that leveraging the concepts to train the CT significantly boosts the classification performance.



\subsection{Unsupervised Concept-based Models}
\label{sec:unsup_concept_model}
%It remains to be seen if tasks on a larger scale, like ImageNet, can be addressed by human-crafted conceptual representations. For this reason, 
Unsupervised concept models (Section \ref{sec:unsup_concept_model}), modify the internal representation of a network to autonomously extract concepts without explicitly associating them with pre-defined symbols. 
In some cases, these models jointly train an intermediate layer with an unsupervised learning technique to extract an \textit{unsupervised concept basis}, i.e., a clusterized representation identifying groups of similar samples (Section \ref{sec:unsup_concept_basis}). 
Otherwise, they explicitly require the network to represent in the layer weights \textit{prototypes-concepts},  (parts of) frequently seen input samples (Section \ref{sec:unsup_prototype}).
% A separate line of research focuses on automatically extracting Unsupervised Concept-based Models. 
% As anticipated in Section~\ref{sec:cat_cbm}, this category mainly follows two approaches according to the type of unsupervised concept employed either \textit{unsupervised concept basis} (Section \ref{sec:unsup_concept_basis}) or \textit{prototype-based concepts} (Section \ref{sec:unsup_prototype}).

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.8\linewidth]{Images/senn.png}
%     \caption{SENN~\cite{alvarez2018towards}}
%     \label{fig:senn}
% \end{figure}

\subsubsection{Unsupervised Concept Basis}
\label{sec:unsup_concept_basis}
The idea behind these approaches is to learn unsupervised disentangled representations in the latent space of a model. These representations must group samples with some characteristics, such as a generative factor. This class of approaches takes inspiration and shares ideas with the disentangled representation learning field~\cite{bengio2013representation}.
To extract unsupervised concepts, these models are jointly trained to reconstruct the input by means of a decoder branch (SENN, BotCL, and reported in Figure~\ref{fig:cbm_unsup_basis}) to maximize the mutual information (Interpretable CNN) or via self-supervised loss over textual data (SelfExplain). When these models employ an interpretable task predictor over the concepts, they also provide class-concept relations (SENN, BotCL). 


\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{Images/cbm_unsup_basis-2.png}
    \caption{Unsupervised concept-based model extracting unsupervised concept basis. How the concepts are extracted varies between the models. Here, we report the case in which a decoder branch is employed over the concept to reconstruct the input and extract meaningful concepts (SENN, BotCL).}
    \label{fig:cbm_unsup_basis}
\end{figure}


%%%Interpretable CNN
%\myparagraphbold{Interpretable CNN~\cite{zhang2018interpretable}}
% This study presents a technique to enhance traditional CNNs, transforming them into pseudo-interpretable models. 
% Interpretable CNN has been the first method proposing an unsupervised approach to create an explainable-by-design network. 
\smallskip
In \textbf{Interpretable CNN~\cite{zhang2018interpretable}}, convolutional filters act as unsupervised concepts and are required to represent different object parts. The assignment occurs during the learning process without employing any concept annotation.
%%%What is
% This work builds upon Network Dissection~\cite{bau2017network}, adopting its IoU evaluation metric. The authors intend to improve the existing CNNs by orienting the representation of each filter towards a distinct part of the object, ultimately making the networks more interpretable.
%%%How it works
% Given a high convolutional layer of a CNN, the authors implement a loss to direct each filter toward representing a specific part of the object within a category. 
%During this phase, the expectation is that, for a given input image, the CNN will activate at the target part's location using a designated template. 
The authors devise an unsupervised loss function to achieve this, maximizing the mutual information between the image and the filter activations. 
Also, the loss promotes low entropy in both the inter-category activations and the spatial distributions of neural activations.
The idea is that filters should create a clusterized representation of the concepts. Each filter should encode a distinct concept associated with a single object category, possibly not repeated in different image regions. %ensuring activation by a specific object part appearing only once in the image. 
%This ensures that the filter is only activated for that part while it remains inactive for images of other categories. 
 %Consequently, each filter only encodes a distinct object part associated with a single object category, 
% ensuring activation by a specific object part rather than appearing repetitively in different regions. 
%In the forward propagation stage, for each input image, the CNN strategically chooses a specific template from a set to serve as a mask for filtering out unwanted activations. This mask operation is crucial for supporting the subsequent gradient back-propagation phase.
%During this phase, the expectation is that, for a given input image, the CNN will activate at the target part's location using a designated template. To achieve this, the authors devise a loss function that measures the mutual information between the image and the selected template.
%%%Results
% Interpretable CNN %is applied to four CNN architectures (i.e., VGG-M, VGG-S, VGG-16, AlexNet) and 
% is tested on three datasets, each with ground-truth bounding boxes of objects, to evaluate the capability to identify human-annotated objects without employing them while training. 
% It is worth noticing that, in this study, the term 'concept' is absent. 
In the evaluation, the authors measure the IoU score with ground-truth object bounding boxes, similar to ND. % adopting, however, a higher threshold (justified by the intervention during training).
% The evaluation uses two metrics: \textit{part interpretability} and \textit{position stability}. The former, derived from ND, measures the Intersection Over Union (IoU) scores. A key distinction is adopting a higher threshold, justified by the higher-level semantics (object parts) compared to ND's colors or textures. 
They also measure the part location stability, 
% The second metric assesses part location stability, 
assessing the consistency in how a filter represents the same object part across various objects. 
%This entails minimal distance variation between the inferred part location and specific object landmarks across different objects.
The experimental findings show that Interpretable CNNs exhibit superior interpretability and location stability compared to standard CNNs. Regarding classification accuracy, Interpretable CNNs are on par with simple CNNs. %simple CNNs outperform in single-classification scenarios, while Interpretable CNNs excel in multi-classification scenarios.
%%%Insights



%%% SENN
%\myparagraphbold{SENN~\cite{alvarez2018towards}}
\smallskip
Self-explanatory neural network \textbf{(SENN~\cite{alvarez2018towards})}, similarly to Interpretable CNN, also employs an unsupervised approach to create an explainable-by-design network, this time based on an auto-encoder architecture. %is the first method proposing an unsupervised approach to create an %self-explainable 
% explainable-by-design model based on concepts.  
 % are models with built-in interpretability characteristics. 
% The authors motivate the self-explainability ability of SENN  since it can be seen as a generalization of a linear (and interpretable) regression model without compromising performance. 
%The goal is to refine the linear model, making it intricate yet retaining the clarity and comprehensibility typical of linear models.
% A SENN model has two main components. %(see Figure~\ref{fig:senn}). 
% The former is a concept encoder, 
SENN first employs a concept encoder to derive a clusterized representation of its features from the input. 
% For example, given a digit image as input, the basis concepts may be stroke width, global orientation, position, roundness, and the like. 
Second, it employs an input-dependent parametrizer that generates class-concept relevance scores. %which can be interpreted as the contribution of each basis concept 
% which represent the relevance of each extracted concept for a given output class.
The output is given by the linear combination of these basis concepts and their relevance scores. %via the aggregator component.
The degree of interpretability of SENN is intrinsically tied to the interpretability of the underlying concepts. %So, to learn interpretable concepts, the SENN
% To this aim, the authors introduce three minimal desiderata and how SENN achieves them: % that these concepts should have.
% i) Fidelity: The input representation of concepts should keep relevant input information. This is obtained by learning basis concepts in the latent encoding of an encoder.
SENN promotes concept diversity to this aim: inputs should be representable using a few non-overlapping concepts. This is achieved by making the concept encoder sparse. %However, while this forces input to be representable with few concepts, it does not guarantee that they should be non-overlapping.
% iii) Grounding: Concepts should be immediately interpretable and understandable to humans. Even though this is a more subjective criterion, SENN addresses this by providing interpretations for the concepts through the concept relevance scores and prototyping. %; however, this did not work. 
Also, to visualize the identified concepts, SENN %shows its relevance score and 
provides a small set of training examples that maximally activate it.
The authors show that SENN explanations compared to standard XAI techniques (i.e., LIME \cite{ribeiro2016should}, SHAP\cite{lundberg2017unified}) result in more:
i) explicit, SENN explanations are more immediate and understandable;
ii) faithful, SENN importance scores are assigned to features indicative of ground-truth importance;
iii) stable, since similar examples yield similar explanations for SENN. 
SENN classification accuracy is slightly lower or on par with standard CNN according to the experimented scenarios. 
% The authors demonstrate that SENN models are able to produce robust explanations.
%\todo{do they compare with a black box network? do they lose in accuracy?}



%%%BotCL
%\myparagraphbold{BotCL~\cite{wang2023learning}}
% \textit{Bottleneck Concept Learner} (BotCL) discover concepts in a self-supervised manner while simultaneously tackling classification tasks. %BotCL encodes images based on the presence or absence of learned concepts.
%\textit{Bottleneck Concept Learner} (BotCL) is a concept-based explainable by-design model that can simultaneously discover concepts in a self-supervised manner and solve the classification task. It represents an image solely by the presence or absence of concepts that are learned through training over the target task. 
%
%%%What is and How it works 
% Similarly to SENN, also 
\smallskip
Bottleneck Concept Learner \textbf{(BotCL~\cite{wang2023learning}) }is based upon and improves the idea of SENN for extracting an unsupervised concept basis. % and provides for the task prediction by means of a linear classifier. %The importance of the concepts, however, is not computed from the input but directly with a linear layer.
% The way in which concept are extracted and trained, however, get refined. 
% The BotCL framework includes as key components a Concept Extractor, a Classifier, Regularizers, and a self-supervision mechanism.
% BotCL processes input images using a CNN backbone to generate feature maps, which are then fed into the Concept Extractor. 
In BotCL, the features extracted from the convolutional encoder are fed into a slot attention-based mechanism~\cite{li2021scouter} predicting for concept scores. A set of vectors learnt by backpropagation represent the concept embeddings and are used as keys of the attention mechanism. 
% without supervision. 
% The attention mechanism employs \textit{conceptual prototypes}, acquired through the training process, to determine the presence of a given concept within each input image.
% The results from the attention are summarized into concept bottleneck activations. % that the classifier will use to make the final classification. In this case, 
%Concept activations are expressed by continuous values and optimized to be between 0 and 1 by means of a quantization loss. 
%
A linear layer working over concept scores is employed as a task classifier, and it captures class-concept relationships. %Specifically, a positive weight value indicates that a particular class within the dataset is associated with a specific concept and that these two elements tend to occur together.
%
%The absence of concept labels motivated the incorporation of self-supervision in BotCL. 
BotCL employs the reconstruction loss of SENN or a contrastive loss to learn meaningful concepts.
% Self-supervision is integrated by introducing two loss terms: reconstruction and contrastive loss.
% The former SENN~\cite{alvarez2018towards}, uses a decoder to reconstruct the original image from the concept activations. 
The latter enforces similarity among concept activations belonging to the same class and dissimilarity otherwise. %It is shown to 
%Given the compositional nature of images, where different elements can usually be arranged arbitrarily, the reconstruction loss alone may be ineffective. Inspired by contrastive learning, BotCL also incorporates a contrastive loss. In particular, if a pair of concept activations belongs to the same class, it must be similar, as a set of similar concepts must be present in the corresponding images and otherwise dissimilar. 
%
%BotCL uses Concept Regularizers to facilitate training and constrain the \textit{concept prototypes}. 
Also, BotCL employs two regularizations to facilitate training and ensure consistency in the learned concepts.
%For better interpretability, each learned concept should have no large variations. 
The first is a consistency loss, enforcing similarity between the concept features that activate the concept in different images. The second is a mutual distinctiveness loss, requiring different concepts to cover different visual characteristics.
%Utilizing cosine similarity, the authors establish a consistency loss that guarantees the similarity of conceptual attributes between two images, in relation to a specific concept, when their conceptual activation approaches a value close to 1.
%Another aspect that is regularized is mutual distinctiveness. That is, to capture different aspects of images, different concepts must cover different visual characteristics. 
%This means that the average image features of a concept within a mini-batch of data should be different from any other features.
%%%Results
BotCL task performance, on average, is higher than SENN, ProtoPNet, and Completeness-aware, particularly when employing the contrastive loss. %, while it shows suboptimal results when employing reconstruction loss.
%BotCL is evaluated both quantitatively and qualitatively.
% The BotCL's quantitative performance is assessed across four datasets, including one synthetic dataset. 
% The benchmarking process involves 
BotCL extracted concepts, instead, are compared against ACE and Completeness-aware on a synthetic dataset annotated with concepts. They result in being good in terms of concept purity and efficiency and reconstruction error, particularly when employing many concepts. %, both interpretable models while employing k-means and PCA for non-interpretable models. Notably, BotCL demonstrated strong performance when utilizing contrastive loss, surpassing other methods in most cases, except for one instance. However, when employing reconstruction loss, BotCL consistently exhibited suboptimal results.
%For the qualitative analysis, 
% To evaluate the extracted concepts the
% authors conduct a user study to evaluate %human understanding. Participants are asked to observe images and select predefined phrases that describe the concepts.
% % BotCl yields good results in terms of 
% concept discovery (i.e., identification of consistent visual elements), concept consistency (i.e., consistent selection of a description for a concept), and mutual distinctiveness (i.e., number of concepts associated to the same elements, the lower, the better). 
% %
%
%
%They can also answer \textit{None of them} if they think they are inconsistent. 
%In this qualitative evaluation, the authors establish three key metrics:
%i) Concept Discovery Rate: This metric gauges the participants' ability to identify consistent visual elements.
%ii) Concept Consistency: This metric quantifies the extent to which multiple participants select the same descriptive phrase for a given concept.
%iii) Mutual Information between Concepts: This metric assesses the degree to which various concepts are associated with the same visual elements. 
%BotCl yields good scores for all the metrics described above, showing that the learned concepts are interpretable for humans, consistent, and mutually distinct. 




%%% SelfExplain
%\myparagraphbold{SelfExplain~\cite{rajagopal2021selfexplain}}
\smallskip
\textbf{SelfExplain~\cite{rajagopal2021selfexplain} }is a self-explaining model, providing local explanations within text classifiers as \classconcrel{}. It extracts concepts in an unsupervised way directly from the input text. In particular, the concepts are here represented as the non-terminal leaves of the semantic tree parsing the text. %during the training. 
%%%What is
SelfExplain incorporates two different layers into a neural text classifier to explain the predictions. %The introduction of these layers facilitates interpretability while maintaining the task performance. 
%%%How it works
Specifically, the Locally Interpretable Layer (LIL) %is introduced. This layer aims to 
compute the relevance score for all input concepts extracted from the input sample. 
%On the other hand, t
%To provide global explanation, 
The Globally Interpretable Layer (GIL), instead, %is used. In this case, the aim is to 
interpret sample predictions by means of the concepts extracted from all the training data. The GIL layer brings the advantage of studying 
how concepts from the training set influenced the classifier's decision. %, providing more granularity to the explanation.
The concept scores of both layers are employed to re-predict the final class, but they are not employed for the standard prediction. 
% The definition of concepts in NLP settings is different because it goes beyond individual words. In this work, phrases are considered as concepts. 
%%%Results
% The SelfExplain framework undergoes evaluation across five datasets designed for text classification, including two specifically tailored for sentiment analysis. 
As a baseline, RoBERTa and XLNet transformer encoders are used. GIL and LIL layers are incorporated into the transformers to make a comparison. The results reveal that incorporating GIL and LIL layers % into the transformers within the SelfExplain framework 
consistently leads to better classification across all evaluated datasets, probably due to the multitask loss employed.
% To gauge the efficacy of the explanations, the authors employ the following criteria as key measures: (i) Sufficiency; (ii) Plausibility; (iii) Trustability.
To gauge the efficacy of the explanations, the authors conducted a human evaluation, where explanations provided by SelfExplain are consistently acknowledged as more understandable, trustworthy, and adequately justifying model prediction than standard XAI techniques.



\subsubsection{Prototype-based Concepts}
\label{sec:unsup_prototype}
Within the domain of unsupervised concept-based models, another possibility is to require the network to explicitly encode \textit{prototype-based concepts}, which represent specific (parts of) train examples. As shown in Figure~\ref{fig:cbm_unsup_proto}, the prototypes are  
compared to input samples, and their similarities are employed as sufficient statistics to provide the final prediction.   
How the prototypes are extracted is different among the methods, either by means of an autoencoder (Prototype DL), or per class by means of the same convolutional filters (ProtoPNets), sharing them among the classes (ProtoPShare, ProtoPool) with a hierarchy of prototypes (HPNet), with deformable filters (Deformable ProtoPNets) or through an interactive process with human experts (ProtoPDebug). 
In most cases, a linear layer is employed on top of the prototypes to classify the final class and provide an interpretable class-concept relation. All the methods provide different systems to visualize the concepts since prototype concepts particularly require a visualization.    

%%% Deep Learning for case-based reasoning
% \myparagraphbold{Deep Learning for case-based reasoning~\cite{li2018deep}}
%\myparagraphbold{Prototype DL~\cite{li2018deep}}
%The work of \textit{Li et al.}~\cite{li2018deep}
\smallskip
\textbf{Prototype DL~\cite{li2018deep}} introduces the use of prototypes in concept-based explainability. 
%Their proposed model employs a case-based reasoning (i.e., local) approach.
The proposed model explains predictions based on similarity to prototypical observations within the dataset. % instead of highlighting input segments or identifying unsupervised concept basis. 
Its architecture comprises an autoencoder and a prototype-based classification network.
The autoencoder aims to reduce input dimensionality and learn predictive features. 
The autoencoder's encoder facilitates comparisons within the latent space, while the decoder enables the visualization of learned prototypes. 
Given the encoded input, the prototype classification network generates a probability distribution across K classes. This network includes a prototype layer where each (prototype) unit stores a weight (prototype) vector mirroring an encoded training input.
%The training objective has four terms. Other than the standard cross-entropy and the reconstruction loss for the autoencoder, a term requires each prototype vector to be as close as possible to at least one of the training examples in the latent space, while the last term encourages every encoded input to be close to at least one prototype vectors.
For model prediction interpretation, we can visualize the learned prototype by feeding prototype vectors into the decoder. Then, from the learned weights of the prototype layer, we can identify which prototypes are more representative of a class. 
The experimental results show that the proposed interpretable architecture does not compromise predictive ability compared to traditional and non-interpretable architecture.
%,  demonstrating that we do have to necessarily sacrifice interpretability for accuracy.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{Images/cbm_unsup_proto-2.png}
    \caption{Unsupervised concept-based models employing prototype concepts.
    The network explicitly encodes prototype concepts representing (part of) training examples. The explanations are typically provided as class-concept relation and/or concept visualization.}
    \label{fig:cbm_unsup_proto}
\end{figure}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Images/propnets.png}
%     \caption{ProtoPNets~\cite{chen2019looks}.}
%     \label{fig:protopnets}
% \end{figure}

%%% ProtoPNets
%\myparagraphbold{ProtoPNets~\cite{chen2019looks}}
\smallskip
Prototype Parts Network \textbf{(ProtoPNet~\cite{chen2019looks})} identifies different parts of the input image that look like some learned prototypical parts.
Similarly to \textit{Li et al.}~\cite{li2018deep}, ProtoPNet incorporates a prototype layer but employs convolutional layers for the prototype extraction process.
Thus, ProtoPNet extracts prototypes based on segmented image parts rather than the whole images. Specifically, the convolutional layers extract a set of features for each image patch. ProtoPNet then computes the similarity between each prototype unit and all the image patches.
This process yields a similarity score activation map (similar to a saliency map), where each value indicates the presence of a prototypical component for each part of the image.
These similarity maps generated by individual prototype units are then condensed into a single similarity score for each prototype. % through maximum global pooling.
% This unified score quantifies the presence of a prototypical component in a specific segment of the input image.
The final prediction is based on a weighted combination of similarity scores according to the importance of a prototype for a given class. %between image parts and the learned prototypes.
The resulting model provides explanations in three forms: \classconcrel{} according to the weight connecting each prototype to a class, \nodeconcass{} since each prototype represents a unit of the network, and \concvisual{} through the similarity activation map. 
%Despite its interpretability, 
ProtoPNet achieves a slightly lower accuracy (up to $3.5\%$) than non-interpretable baselines. % (e.g., VGG16, ResNet34, and Dense121).


%%%HPNet
%\myparagraphbold{HPnet~\cite{hase2019interpretable}}
\smallskip
The Hierarchical Prototype network \textbf{(HPnet~\cite{hase2019interpretable})} builds upon ProtoPNet but supports a hierarchical organization of prototypes.
The model supports hierarchical classification, i.e., a classification based on a taxonomy at multiple granularities. The approach learns a set of prototypes for each taxonomy class, from coarser ones (e.g., animal) to finer ones (e.g., cat).
HPnet architecture, after the convolution layers as in~\cite{rymarczyk2021protopshare}, includes a prototype layer for each parent node of the taxonomy. Each layer includes and classifies the prototypes of the finer classes of the corresponding parent one. The design of the prototype layer is close to that of ProtoPNet and provides for the computation of the similarity scores of the learned prototype and patches of the input image.
The approach can provide \concvisual{} via a heat map showing localized portions of the input image that strongly activate the prototype at multiple levels of the hierarchy. Hence, it enables the understanding of the prediction at multiple granularities.
Thanks to its ability to handle hierarchical classification, HPNet addresses the novel class detection problem by classifying data from previously unseen classes at the appropriate level in the taxonomy. 
The experiments show that HPnet experiences a slight drop in fine-grained accuracy with respect to a black-box model. % (VGG-16 network). 

%%% ProtoPShare
%\myparagraphbold{ProtoPShare~\cite{rymarczyk2021protopshare}}
\smallskip
Prototypical Part Shared network \textbf{(ProtoPShare~\cite{rymarczyk2021protopshare})} is an extension of ProtoPNet that introduces the idea of sharing prototypes between classes to reduce the number of prototypes. A reduced number of prototypes, which are, as in ProtoPnet, representations of prototypical parts, improves the interpretability of predictions.
% It can provide all of the previously identified explanation types, such as \classconcrel{}, \nodeconcass{}, and \concvisual{}.
ProtoPshare addresses two issues of ProtoPNet. First, ProtoPNet derives many prototypes since each is assigned to only one class. Second, two prototype representations of two distinct classes with similar semantics can be far apart in latent space, making the final predictions unstable.  
ProtoPShare addresses these issues by introducing prototype sharing between the classes via prototype pruning.
ProtoPShare has two phases: i) initial training and ii) prototype pruning. The initial training phase follows the one of ProtoPNet. The second phase consists of the \textit{data-dependent merge-pruning}.
Given the set of prototypes after initial training,  this step merges a fixed percentage of most similar prototypes. Specifically, the work introduces a data-dependent similarity function to identify prototypes with different semantics, even if they are apart in the latent space. The pruning process proceeds by computing the similarity of pairs of prototypes. If a pair is among a given percent of most similar pairs, one prototype of the pair is removed. 
Even with fewer prototypes, ProtoPShare outperforms ProtoPNet in terms of accuracy.
%The paper qualitatively shows that prototype sharing enables the discover of similarities between classes based on the prototypes they share.
% A user study assesses that prototypes selected with the proposed similarity rather than similarity in the representation space induce more consistent prototypes.


%%% ProtoPool
%\myparagraphbold{ProtoPool~\cite{rymarczyk2022interpretable}}
\smallskip
\textbf{ProtoPool~\cite{rymarczyk2022interpretable}}, inspired by ProtoPNet~\cite{chen2019looks}, tackles some of its limitations and those of subsequent works. One limitation it addresses is the assumption of separate prototypes for each class in ProtoPNet. Like ProtoPShare~\cite{rymarczyk2021protopshare}, ProtoPool reduces the number of prototypes by sharing them across different data classes.
However, ProtoPShare's merge-pruning step leads to increased training time. ProtoPool avoids the pruning by adopting a soft assignment of prototype represented by a distribution and automatic, fully differentiable prototype assignment, thus simplifying the training process.
Furthermore, ProtoPool introduces a focal similarity function that generates saliency maps more focused on salient features compared to using ProtoPnet similarity.
Additionally, ProtoPool introduces \concvisual{} via prototype projection. This involves replacing the abstract prototype learned by the model with the representation of the nearest training patch.
Compared to ProtoPNet and ProtoPShare, % and TesNet,
ProtoPool achieves the highest accuracy on one dataset using fewer prototypes and comparable but lower accuracy results on another one. A user study rated ProtoPool's visualization as more interpretable than other compared methods.
%%%How it works
%The model architecture of ProtoPool closely resembles that of ProtoPNet, but it implements two key modifications in the prototype layer. Specifically, the prototype layer consists of a pool of trainable prototypes with a predetermined number of slots allocated for each class. Each slot is conceptualized as a distribution of prototypes drawn from the pool, where the values within the distribution indicate the probability of assigning a specific prototype to that slot. The assignment of prototypes is carried out through a differentiable function.


%%% Deformable ProtoPNet
%\myparagraphbold{Deformable ProtoPNet~\cite{donnelly2022deformable}}
\smallskip
Also \textbf{Deformable ProtoPNet~\cite{donnelly2022deformable}} builds upon ProtoPNet~\cite{chen2019looks}. The work addresses the limitation of ProtoPNet and its subsequent works of using spatially rigid prototypes, which cannot explicitly consider geometric transformations or pose variations of objects.
Deformable ProtoPNet uses spatially flexible deformable prototypes.
Each prototype consists of adaptive prototypical parts that dynamically adjust their spatial positions based on the input image. 
The work builds upon previous work modeling object deformations and geometric transformations to deform prototypes, specifically on Deformable Convolutional Network~\cite{dai2017deformable}.
%%%How it works
%In Deformable ProtoPNet, a prototypical part is a 1x1 patch within a deformable prototype. Each part can move independently, representing a distinct, spatially decoupled semantic concept. The framework adopts an offset to enable prototype deformation, granting each part the ability to move within the prototype's application. This facilitates evaluating the similarity between prototypical parts at deformed positions. Offset calculation for deformable prototypes involves an offset prediction function that maps fixed-length input features to an offset field with identical spatial dimensions, accommodating both integer and fractional offset values.
The experimental results show that Deformable ProtoPNet achieves state-of-the-art accuracy.
%%%Results
%The Deformable ProtoPNet framework is evaluated on the CUB dataset across various configurations of deformable prototype sizes, with a performance comparison against ProtoPNet. The results indicate that Deformable ProtoPNet consistently achieves competitive accuracy across different backbone architectures.

%%% ProtoPDebug
%\myparagraphbold{ProtoPDebug~\cite{bontempelli2023conceptlevel}}
\smallskip
ProtoPNets~\cite{chen2019looks} may provide confounder factors as part-prototype explanations (e.g., textual metadata in image X-rays or background parts), limiting the model's predictive performance and generalizability.
\textbf{ProtoPDebug~\cite{bontempelli2023conceptlevel}} addresses this issue by proposing a human-in-the-loop concept-level debugger for ProtoPNets architectures. 
Human experts identify which part-prototypes are confounders by examining ProtoPNets' explanations. This information is provided as a feedback to the model and it is fine-tuned to align with the user supervision.
%ProtoPDebug adopts cost-effective concept-level supervision, offering informative annotations. 
ProtoPDebug assesses all learned part-prototypes during each iteration, retrieves maximally activated training samples, and prompts user judgment on confounding. Confirmed confounders are added to the \textit{forbidden concepts} set. %, specifying if their impact is on specific or all classes. 
Conversely, high-quality part-prototypes are incorporated into the \textit{valid concepts} set. For the fine-tuning step, ProtoPDebug proposes two losses for the fine-tuning step. 
The \textit{forgetting loss} penalizes forbidden concepts while the \textit{remembering} loss encourages remembering valid ones. 
%Specifically, the \textit{forgetting loss} minimizes how much the part-prototypes of each class activate on the most activated concept to be forgotten for that class. The \textit{remembering} loss maximizes how much the part-prototypes activate on the least activated concept to be remembered for that class.
%%%Results
ProtoPDebug outperforms a predecessor debugger %, IAIA-BL,
and ProtoPNet, enhancing test classification accuracy.


% A strategy for debugging ProtoPNet with confounded part-prototypes is to delete the problematic ones and fine-tune the remaining ones. However, there is no guarantee that the network will reacquire the same confounder using one of the remaining part-prototypes. This problem inspired the creation of the only debugger for ProtoPNet to date, IAIA-BL~\cite{barnett2021case}, with which ProtoPDebug directly competes. ProtoPDebug highlights a notable limitation in its predecessor; specifically, the method is restricted solely to pixel-level supervision.


% \textit{Hybrid.} Other works take a different approach, integrating in the architecture both supervised and unsupervised concepts (Section \ref{sec:sup_unsup_cbm}). The goal of this integration is generally to allow the employment of concept-based models also in those scenarios where few supervised concepts are available for the task at hand. %This allows to increase the generalization performance of standard supervised concept models as well as extracting a better concept representation.

% \textit{Generative.} Generative methods, instead, employ an external generative model to define textual concepts (i.e., textual descriptions of the main classes) (Section \ref{sec:generative}). These textual descriptions are then embedded  in the internal representation of the network in the form of numerical representation to predict the final classes. At test time, these models predict both the final class and the most suitable descriptions among those that have been learnt.  

\subsection{Hybrid Concept-based Models}
\label{sec:sup_unsup_cbm}
Hybrid concept-based models propose the joint employment of both supervised and unsupervised concepts, as shown in Figure~\ref{fig:cbm_hybrid}. The strategy normally involves the employment of an unsupervised learning strategy, either reconstructing the input image with an AE (Ante-hoc, and reported in Figure\ref{fig:cbm_hybrid}) or a VAE (GlanceNet) or maximizing the mutual information (CBM-AUC), together with some supervision over some concepts. 
The goal of this integration is generally to allow the employment of concept-based models also in those scenarios where few supervised concepts are available for the task at hand.
This approach has been adopted to improve the performance of standard CBM (CBM-AUC, Ante-hoc Explainable Model) and its capability to represent concepts (GlanceNet).

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/cbm_hybrid.png}
    \caption{Hybrid concept-based model employing both supervised and unsupervised concepts. This approach normally involves employing an unsupervised learning strategy (such as reconstructing the input image) to learn an unsupervised concept basis and a few supervisions over some neurons representing symbolic concepts.}
    \label{fig:cbm_hybrid}
\end{figure}


%%%CBM-AUC
%\myparagraphbold{CBM-AUC~\cite{sawada2022concept}}
\smallskip
Concept Bottleneck Model with Additional Unsupervised Concepts \textbf{(CBM-AUC~\cite{sawada2022concept})} is the first approach designed to merge CBM~\cite{koh2020concept} with SENN~\cite{alvarez2018towards}, employing supervised and unsupervised concepts at the same time. %Also, they provide visualization of the concepts
%
%%%What is
CBM-AUC addresses the issue of CBM's restricted concept efficiency. %, as the number of available concepts can be limited in several real-world scenarios. 
To address this, the authors suggest enabling the model to leverage the representation capability associated with unsupervised concepts. %extracted with SENN.
% Furthermore, as SENN cannot work on large image datasets, integrating CBM and SENN alone would be unsuccessful.
%
%%%How it works
The first contribution is the introduction of M-SENN, a variant of SENN reducing the computational complexity and improving the scalability of SENN. 
First, it replaces the decoder of the AE architecture employed by SENN with a discriminator. This module now optimizes
% effectively solves a limitation of SENN, i.e., its inability to handle a substantial volume of images due to the demand for many parameters.
% The first modification involves substituting the decoder with a discriminator to optimize
the mutual information between the input and the unsupervised concepts. %latent space, which, in this context, correspond to the concepts. 
Second, M-SENN parametrizer now 
% relates to the structural modification of SENN's encoder and parametrizer. In M-SENN These components 
shares the intermediate network with the encoder, reducing the computational complexity. 
For integrating CBM into SENN, they add supervision on some concept basis, which then comprises unsupervised and supervised neurons.
% while allowing for incorporating a more intricate network such as Inception-v3. The selection of the intermediate network has to respect the desiderata of SENN about inputs.  
%%%Results
% The evaluation of CBM-AUC comprises two datasets, including %BDD-OIA, 
% a video dataset. Specifically, only the final frame of each video is extracted from this dataset, consistent with the approach outlined in the original article, and used as input. 
The results show that the modifications made to join SENN with CBM are effective. %In particular, they succeeded in significantly reducing the number of parameters. %Significant are the results obtained by CBM-AUC on the CUB dataset.  Specifically, 
CBM-AUC outperforms the task accuracy of both SENN and CBM. 
% In particular, by overcoming the bottleneck of CBM, CBM-AUC achieves good task performance even when employing very few supervised concepts.  
% However, the best results are obtained by CBM-AUC on the video dataset. 
%%%Insights 
Also, they analyze both supervised and unsupervised concepts by visualizing their activation through saliency maps. They show that both types of concepts look at semantically meaningful areas of the input images. %, facilitating the model to take the right the final decision.% for the prediction. 


%\myparagraphbold{Ante-hoc~\cite{sarkar2022framework}}
\smallskip
Similarly to CBM-AUC, also Learning \textbf{Ante-hoc Explainable Models via Concepts~\cite{sarkar2022framework}} %presents a novel approach to learning concept-based explanations based on an 
integrated supervised and unsupervised concepts %  and self-supervised concepts, 
starting from SENN and CBM. 
%The method proposed entails integrating an explanation generation module onto any network and simultaneously training the entire module to both achieve high predictive performance and generate explanations.
%
%%%What is
% The proposed module offers several distinct features:
% i) It can be seamlessly integrated into existing networks with minimal additional parameters.
% ii) It can provide explanations for both individual input data and groups of images.
% iii) It exhibits the flexibility to incorporate varying levels of supervision. Indeed, the authors introduce a model that is adaptable to unsupervised, supervised, or self-supervised conditions to enhance explanation extraction.
%%%How it works
% Similarly to CBM-AUC, 
% The proposed framework starts from the architecture of SENN, %can merge seamlessly with any neural network, 
%incorporates a base encoder for input feature extraction, a concept encoder and a base classifier for the classification task. 
Differently from CBM-AUC, however, it %In addition, it incorporates a concept encoder anemploys
still employs SENN concept decoder to learn unsupervised concepts. %, as shown in Figure \ref{fig:ante_hoc}.
% Similarly to SENN, %the concept encoder is responsible for acquiring concepts from the input features extracted by the base encoder, 
% the concept decoder, with its associated reconstruction loss, is introduced to encourage the model to acquire semantically relevant concepts.
However, the most important difference between both models is that the classifier is added on top of the base encoder and not the concepts. This entails that the final classification is not based on the concepts. %, and we argue that concept interventions (as defined in CBM) should have no effect.
To minimize this issue, they add a classifier to the concept encoder and minimize predictions' divergence via a fidelity loss. %the measure whether the predictions obtained from the concepts alone are as informative as those obtained from the base classifier.
As presented, the model is designed to operate in unsupervised concept learning mode. A loss function is employed to align the learned concepts with the available annotations to allow the model to learn supervised concepts. %in the dataset for the respective instances. 
% If supervision is unavailable, the model tries to learn interpretable concepts by exploiting the underlying structure of the data.
Otherwise, self-supervision can also be integrated as an auxiliary task, such as predicting the rotation of the input images starting from the encoded concepts. %Unlike conventional methods where the auxiliary task utilizes the output from the feature extractor, in this approach it relies on the conceptual encoder instead.
%%%Results
The proposed framework demonstrates competitive performance across both annotated and not annotated datasets, %, encompassing two annotated (AwA2 and CUB) and two unannotated ones (CIFAR10 and ImageNet). 
% When evaluating the unannotated datasets, the comparison exclusively involves SENN and the unsupervised version of the proposed framework. For the annotated datasets, the comparison encompasses SENN, CBM, and both versions of the proposed framework.
% In both scenarios, the proposed approach %outperforms the respective competitor, therefore 
improving the task accuracy of CBM and SENN, respectively. 
% We argue, however, that this improvement comes at the cost of a reduction of the interpretability of the network, since the final prediction is not based on the concepts, which are rather seen as an auxiliary task.   
% Overall, the proposed framework represents a significant advancement in this context.
%%%Insights 
% Other metrics used in the evaluation are faithfulness, fidelity, explanation error, and intervention on concepts. The proposed framework is competitive in all of them.

%%% GlanceNets
%\myparagraphbold{GlanceNet~\cite{marconato2022glancenets}}
\smallskip
% GlanceNets~\cite{marconato2022glancenets}, propose another variant of hybrid concept-based models. 
Unlike previous work, \textbf{GlanceNets~\cite{marconato2022glancenets}} aims to improve the concept representations of SENN and CBM rather than the performance. It improves the interpretability of SENN %and the concept representation of CBM by exploiting techniques from disentangled representation learning and open-set recognition. 
by employing a VAE instead of a standard AE to learn disentangled concepts. %GlanceNets can seamlessly integrate with various VAE-based architectures designed to acquire separate representations. 
% Also this paper addresses two challenges of CBMs and proposes a solution. 
% Given the need for more agreement on the definition of interpretability, GlanceNets' authors present a new definition stating that interpretability relies on the alignment between acquired and ground truth concepts.
% The proposed definition combines the notion of disentanglement with an extra monotonicity constraint. 
% \textit{Disentanglement} can be defined as how a learned concept r
Due to the variational approach, learned concepts can better represent sample generative factors and respond to their alterations. %a generative factor undergoes an alteration. 
When supervised concepts are available, they force a mapping with the learned concepts to preserve known semantics. 
They also improve the representations of CBM by identifying a solution to %also contribute to a novel perspective on 
the concept leakage issue (see Section~\ref{sec:cbm_issues} for a description). They claim it is a deficiency in the out-of-distribution generalization of concept-based models. 
% They show that information leaks into the learned concepts from intendant ground truth, and it is faced when unintended concepts vary due to a shift in the distribution. 
% To counteract concept leakage, the authors develop a strategy that,
Therefore, GlanceNets employs an open-set recognition technique at inference time to detect instances that do not belong to the training distribution. They show this solution substantially improves the concept alignment with respect to CBM. 
% An inherent limitation inherited from VAEs is the assumption that interpretable generative factors are disentangled from one another, which may not always reflect human-defined attributes.
% Possibly also for this reason, 
Task performances are on par with CBM and SENN. 
%\todo{do they compare with a black box network? do they lose in accuracy?}


\subsection{Generative Concept-based Models}
\label{sec:generative}
% Very recently, some approaches have chosen a different path to create explainable-by-design concept-based models. 
Rather than employing a set of symbolic supervised concepts or extracting an unsupervised concept basis, generative concept-based models have recently shown that they can directly create concept representations. % with a generative model. 
As shown in Figure~\ref{fig:cbm_gen}, this is generally performed by employing a Large Language Model (LLM) producing \textit{Textual Concepts}, short textual descriptions of the final class. The embeddings representing the textual concepts are aligned to the latent input representation to output concept scores. These scores are then employed to provide for the final classification, possibly with an interpretable classifier providing class-concept relations. 
% Different kinds of blending can be imagined following the same idea, a concept generator creating representations (not necessarily textual) that can be employed in an external model (not necessarily visual). 
At test time, these models predict both the final class and the most suitable descriptions among those that have been learned.  
In the following, we outline two methods (LaBO~\cite{yang2023language} and Label-free CBM~\cite{oikarinen2023label}) of this recent line of work. The two methods are similar in their main components since they both employ an LLM in combination with a vision-language one and provide class-concept relation explanations.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Images/labo.png}
%     \caption{Language in a Bottle~\cite{yang2023language}.}
%     \label{fig:labo}
% \end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/cbm_gen-2.png}
    \caption{Generative concept-based models employ an external LLM to generate textual concepts, i.e., short descriptions of the final classes without requiring a concept annotation. The embeddings representing the textual concepts are aligned with the input latent representation. The alignment produces the concept scores, which are used to provide the final classification.}
    \label{fig:cbm_gen}
\end{figure}


%%% Language in a bottle
%\myparagraphbold{LaBO~\cite{yang2023language}}
\smallskip
Language-guided Bottlenecks \textbf{(LaBO~\cite{yang2023language})} is the first model proposing this idea. It exploits the Generative Pre-trained Transformer 3 (GPT-3) language model \cite{brown2020language} to generate factual sentences to derive concepts. This approach circumvents the requirement for costly manual annotation of concepts.
In the LaBO framework, the process initiates by prompting the GPT-3 model with queries designed to generate a collection of \emph{candidate concepts} for each class. An example of a prompt is: \textit{"Describe what the <class\_name> looks like."} 
Subsequently, the approach applies a submodular optimization technique to select a subset of the generated sentences to maximize the discriminability and diversity of the concepts.
The generated textual concepts are then aligned to images using a pretrained alignment model to form a bottleneck layer. 
Specifically, LaBO uses CLIP~\cite{radford2021learning} to derive embeddings of concepts in textual form and images. 
%CLIP aligns the textual concepts with the visual content of images, ensuring meaningful association between the two modalities.
%Then, the similarity score between concepts and images is computed through the dot product.
Subsequently, a linear layer is applied to the similarity scores of concepts and images to learn a weight matrix whose values represent the importance of the concepts in the classification task.
The effectiveness of LaBo is intrinsically linked to the representation of the classes and concepts within the adopted LLM. 
%LaBo introduces two user-evaluated metrics: factuality (precision of concepts in describing classes) and groundability (consistency of the vision-language alignment model in aligning concepts with images). 
LaBo retains accuracy in limited training data scenarios, but as data volume grows, its performance slightly decreases while remaining competitive compared to black-box models.
Compared to PCBM~\cite{yuksekgonul2022posthoc} as an interpretable baseline, LaBo exhibits a substantial performance improvement. 

%%% Label-free
%\myparagraphbold{Label-free CBM~\cite{oikarinen2023label}}
\smallskip
Label-free Concept Bottleneck Model \textbf{(LabelFree-CBM~\cite{oikarinen2023label})} is a framework close to LaBo~\cite{yang2023language}. 
As LaBO, LF-CBM can convert a neural network into an interpretable CBM without requiring annotating concepts but by generating them using a language model. 
%
Its main steps also resemble LaBO ones.
It generates the concepts using GPT-3~\cite{brown2020language} and filters them to enhance the quality and reduce the concept set's size.
Then, it computes embeddings from the network backbone of input data and the concept matrix. 
The concept matrix is derived using a visual-text alignment model (CLIP-Dissect~\cite{oikarinen2022clip}). 
Each element of the matrix is the product between the CLIP encoding of the images of the training set and the concepts.
%
The framework then involves learning the concept weights to create the Concept Bottleneck Layer. 
Lastly, the final predictor is learned by training a fully connected sparse layer.
%%% Results 
The authors assessed the interpretability of the model with a user study.
Regarding performance, LF-CBM demonstrates only a small loss in task accuracy compared to the original neural network backbones while it outperforms the interpretable PCBM~\cite{yuksekgonul2022posthoc}.
%The authors assessed the model interpretability from the global and local perspectives.  From the global one, they used the Sankey diagram visualization of the final layer weights and showed, in some case examples, that the learned decision rules in the final layer align well with human intuition. For example, concepts like "citrus" are highly correlated with both "Orange" and "Lemon," while the concept of "Yellow" only activates "Lemon". From the local one, the model allows for understanding the reasoning behind individual predictions since the final predictions are linear functions of interpretable features.
%
%In Label-free CBM, both the accuracy and interpretability are evaluated.
%As far as accuracy is concerned, the proposed Label-free CBM, compared to the used backbones, has a small loss on all five datasets. On the other hand, this seems to exceed the performance achieved by PCBM. 
%To assess the global interpretability, they first use a visualization diagram, the Sankey diagram. This shows that in the final layer of Label-free CBM, the learned decision rules largely align with the "human" intuition. In Imagenet, for example, the concept of "citrus" is highly correlated with both "Orange" and "Lemon", while the concept of "Yellow" only activates the last of the above. 
%Besides the global understanding, the model also allows us to understand the reasoning behind the individual prediction. Since the final predictions are linear functions of interpretable features, these can be easily explained. As we previously outlined, the matrix of weights in the last layer is sparse, and since many contributions will be 0,  contributions of important concepts to the final prediction can be easily visualized. 
%
%%%Insight
%The case study carried out on manually improving the model on ImageNet is interesting. The authors identify four precise categories of errors that the model makes, more or less serious. Of these, fixing the incorrect final layer weight is the one that is resolved. This is done by changing the magnitude of a weight relative to the incorrect concept by slightly more than it takes to change the final prediction. Interesting as a first large-scale model intervention approach.  
%
%The authors assessed the faithfulness and plausibility of the model.
%From the first evaluation, they evaluated if the neurons learned in the concept bottleneck layer indeed correspond to their target concepts by showing highly activating images for a given neuron and asking how they match the concept.
%From the plausibility perspective,  they evaluate how much users find the concepts that contribute the most to a decision reasonable.


\subsection{Discussion}
\label{sec:cbm_issues}
%\cite{zarlenga2022concept}

In the following, we analyze critical aspects of explainable-by-design models.
We focus on three perspectives: (i) performance loss, (ii) information leakage in concept representation, and (iii) pitfalls of concept intervention.
% saliency

\myparagraphbold{Performance loss}
Concept-based models explicitly represent a set of concepts within the model architecture and rely on these concepts for the final task predictions.
On the other side, the higher transparency of these architectures comes at the cost of a performance loss compared to traditional, black-box architectures.
We analyze this aspect in Table~\ref{tab:summary:bydesign1}. 
Still, we note that several approaches (that we report with \xmark) match the performance of complex black-box prediction models, with the advantage of enabling decision explanations through concepts. 

\myparagraphbold{Information leakage in supervised concept representation}
% Supervised concept-based models learn to map inputs to symbolic concepts and then map those concepts to predictions. 
% We can use the intermediate concept scores (i.e., the predictions of the symbolic concepts) to explain the model decisions. 
Recent works revealed that supervised concept-based models encode additional information in the concept space other than the concept information itself~\cite{havasi2022addressing, DBLP:journals/corr/abs-2105-04289, mahinpei2021promises}. 
% Concept representations may encode additional information than the concept information itself. 
Concept representations may include representations of the task labels when trained jointly with the downstream task. 
% Hence, the model uses the concept representation %not only in their intended manner but 
% also as proxies to incorporate target information.
%, affecting both interpretability and intervenability. 
This phenomenon is denoted as \textit{information leakage in concept representation}, and compromises the model's interpretability and intervenability (i.e., the possibility to perform concept intervention) ~\cite{havasi2022addressing, DBLP:journals/corr/abs-2105-04289, mahinpei2021promises}.
From the interpretability perspective, we cannot directly interpret the association between the concept representations and the model decision since the outcomes may depend on other encoded information. 
From the intervenability one, interventions %(e.g., by setting to 1 a concept probability) 
may remove the extra information encoded and can decrease the final model performance.
% Margeloiu et al.~\cite{DBLP:journals/corr/abs-2105-04289} shows that concept representations of CBMs~\cite{koh2020concept} encode additional information %about the task label 
% when trained jointly with the downstream task. 
% %The joint training encourages the encoding of task-relevant information.
Mahinpei et al.~\cite{mahinpei2021promises} argue this issue is shared among concept-based models that use soft or fuzzy representations to represent concepts and experimentally demonstrate it for CBM~\cite{koh2020concept} andCW~\cite{chen2020concept}).
% Recall that 
% In soft representations, each concept is encoded as a real value in $[0,1]$, representing the confidence in the presence of the concept. Soft representations are used in most current work since they achieve better task performance than hard representations, which represent concepts with $\{0,1\}$ values.
Mahinpei et al.~\cite{mahinpei2021promises} also show that information leakage is not avoided even when applying mitigation strategies, including (i) training concept representations and the concept-to-task sequentially (rather than jointly), (ii) adding unsupervised concept dimensions to account for additional task-relevant information, or (iii) via concept whitening~\cite{chen2020concept} which explicitly decorrelate concept representations during training~\cite{mahinpei2021promises}.
Hence, they conclude that soft representations encode concept information and data distribution.
%
Recent works specifically address leakage issues in concept-based models, such as~\cite{havasi2022addressing} for CBMs and GlanceNets~\cite{marconato2022glancenets}. 


\myparagraphbold{Pitfalls of concept intervention}
Concept-based models enable human experts to intervene in the concept representation and modify them at test time. 
Concept intervention improves final task performance when intervening on mispredicted concepts and generating counterfactual explanations.
However, concept intervention techniques might be affected by major pitfalls. 
Shin et al. identify two major issues~\cite{shin2023closer} on CBMs~\cite{koh2020concept}.
First, intervention could increase the task error, compromising the reliability of intervention techniques. 
This decrease in performance could happen when users nullify void concepts by setting unsure concepts to zero. 
The authors justify this phenomenon, noting that the absence of a concept in a specific image does not entail the concept is not associated with its class. 
We argue this is also linked to the soft representation of concepts and leakage issues.  %My take :)
The second issue arises from the practice of using majority voting to associate concept values to classes to improve task performance (e.g., in \cite{koh2020concept, zarlenga2022concept, havasi2022addressing}). 
Majority voting affects a fair representation of minority samples and makes task outcomes biased toward the majority. 
The authors argue that intervention can exacerbate this unfair treatment since it would increase minority performance only when changing the concept value to the majority one.

%%%% GABRI: add that concept interventions does not work when employing supervised + unsupervised methods


\section{Evaluation} % 2 pages
\label{sec:evaluation}
This section overviews the quantitative and qualitative metrics, the datasets, and the resources mainly used in the literature to assess the performance of C-XAI methods. 
In Section~\ref{sec:metrics}, we delve into the quantitative metrics employed to evaluate the methodologies. This includes measures of the effect of concepts on task predictions and performance, and the quality of concepts. Conversely, Section~\ref{sec:human_eval} elaborates on the qualitative evaluations which leverage human assessments. Section~\ref{sec:datasets} provides an overview of the datasets utilized to assess the effectiveness of C-XAI methods. Finally, in Section~\ref{sec:resources}, we provide details about the resources accessible for each method.


\subsection{Quantitative evaluation} \label{sec:metrics}
We categorize the quantitative metrics used and proposed in the reviewed papers into two categories according to their final purpose and what they measure.
%While classifying the metrics, we maintain the name defined by the proposing method, even though different methods assign the same name to different metrics. Nonetheless, when two metrics measured the same quantity, we considered them under a single definition.  
The metrics of the first category assess how well concepts contribute to class predictions and task performance. The second category focuses on the intrinsic quality of concepts. For a more detailed explanation of each single metric, please refer to Appendix\ref{app:metrics}.
%, studying their inherent properties, how they relate to internal network representations, and their impact on prediction errors. 


\myparagraphbold{Concept effect on class prediction and task performance}
These metrics assess how concepts contribute to (i) the final class prediction or (ii) the task performance.

\textit{(i) Concept effect on class prediction.}
This set of metrics assesses the effect of the concepts on the final class prediction. Concept-based methods often naturally provide the concept relevance (importance) by means of the concept weight connecting the concept to the final classes. Hence, these metrics have been mostly employed for post-hoc explanation methods providing \classconcrel\ to study the impact of the identified concepts on task prediction. 
Among these metrics we find the T-CAV score \cite{kim2018interpretability, ghorbani2019towards}, CaCE~\cite{goyal2019explaining,wu2023causal},  ConceptSHAP~\cite{yeh2020completeness}, Smallest Sufficient Concepts (SSC)~\cite{ghorbani2019towards}, Smallest Destroying Concepts (SDC)~\cite{ghorbani2019towards, vielhaben2023multi}, STCE Concept Importance~\cite{ji2023spatial}, T-CAR score~\cite{crabbe2022concept}, Sobol score~\cite{fel2023craft}, Concept Weight~\cite{yuksekgonul2022posthoc, yang2023language}, Concept Relevance~\cite{alvarez2018towards,rigotti2022attentionbased, barbiero2023interpretable}. 

    % \begin{itemize}
    %             \item T-CAV score: it is the fraction of the class’s inputs with a positive conceptual sensitivity~\cite{kim2018interpretability, ghorbani2019towards}, where the conceptual sensitivity is how much each concept influences the prediction of a given class. So, it measures how many samples have concepts whose effects lie positively on the final prediction. 
    %             %Proposed by: ~\cite{kim2018interpretability}. Used in: ~\cite{ghorbani2019towards}
    %             \item CaCE: it measures the causal effect of the presence of concepts on the final class prediction~\cite{goyal2019explaining,wu2023causal}. 
    %             %Proposed by: ~\cite{goyal2019explaining}. Used in ~\cite{wu2023causal}.
    %             \item ConceptSHAP: it assesses the effect of a concept on the final completeness score~\cite{yeh2020completeness}. The completeness is defined as the amount to which concept scores are sufficient for predicting model outcomes. %So, also ConceptSHAP measures the effect of concepts on the final class prediction. 
    %             %Proposed by: ~\cite{yeh2020completeness}.     
    %             \item Smallest Sufficient Concepts (SSC):
    %             it computes the class accuracy when employing only a subset of the concepts, looking for the smallest set of concepts~\cite{ghorbani2019towards}. 
    %             % it looks for the smallest set of concepts enough to predict the target class. 
    %             %Used in: ~\cite{ghorbani2019towards}
    %             \item Smallest Destroying Concepts (SDC): it looks for the smallest set of concepts deleting, which causes prediction accuracy to fall the most~\cite{ghorbani2019towards, vielhaben2023multi}. 
    %             %Used in: ~\cite{ghorbani2019towards}, ~\cite{vielhaben2023multi}.
    %             \item STCE Concept Importance: it computes the importance rank of each concept for a given class~\cite{ji2023spatial}. %If the score is greater than zero, it indicates that this concept positively affects the prediction for the video. 
    %             %Proposed by: ~\cite{ji2023spatial}.
    %             \item T-CAR score: it quantifies the proportion of instances belonging to a specific class whose representations fall within the positive concept region~\cite{crabbe2022concept}. %If a concept falls within the positive concept region positively impacts the final prediction. 
    %             %Proposed by: ~\cite{crabbe2022concept}
    %             \item Sobol score: %Sobol indices give a quantification of the importance of any subset of concepts with respect to the model decision. 
    %             it measures the contribution of a concept and its interactions of any order with any other concepts to the model output variance~\cite{fel2023craft}. 
    %             %Used in: ~\cite{fel2023craft}.
    %             \item Concept Weight: in concept-based models employing a linear layer from concept to task, the same weight represents the importance of a concept for a given class~\cite{yuksekgonul2022posthoc, yang2023language}. 
    %             %Used in~\cite{yuksekgonul2022posthoc},~\cite{yang2023language}.
    %             \item Concept Relevance: the predicted importance of a concept for a final class in a concept-based model, determined differently for each sample~\cite{alvarez2018towards,rigotti2022attentionbased, barbiero2023interpretable}. 
    %             %Proposed by: ~\cite{alvarez2018towards}; used in:~\cite{rigotti2022attentionbased, barbiero2023interpretable}.  
    %         \end{itemize}

\textit{(ii) Concept effect on task performance.}
 These metrics assess how well concepts contribute to the predictive capacity of the model. 
 They are employed in post-hoc methods, to assess the quality of the extracted concept for predicting the final class; at the same time, they are also studied in concept-based models, to assess how well concepts contribute to the predictive capacity within the given model.
 % Post-hoc methods use them to evaluate the predictive capacity of extracted concepts for approximating the model outcomes. Explainable-by-design models, instead, employ them to assess the concept representations and its capability to predict the task labels. 
 Among these metrics we find the Completeness Score~\cite{yeh2020completeness}, Fidelity~\cite{zhang2021invertible, sarkar2022framework, fel2023craft}, Concept Efficiency~\cite{zarlenga2022concept}, Conciseness~\cite{vielhaben2023multi}.
            % \begin{itemize}
            %     \item Completeness score: it measures the amount to which concept scores are sufficient for predicting model outcomes~\cite{yeh2020completeness}. This is based on the assumption that the concept scores of \textit{complete} concepts are sufficient statistics of the model prediction. 
            %     %Proposed by: ~\cite{yeh2020completeness}.
            %     \item Fidelity: it counts the number of times in which the original and approximate model predictions are equal over the total number of images~\cite{zhang2021invertible, sarkar2022framework, fel2023craft}. 
            %     %Used in: ~\cite{zhang2021invertible}, ~\cite{sarkar2022framework}, ~\cite{fel2023craft}.
            %     \item Faithfulness: this measures the predictive capacity of the generated concepts~\cite{sarkar2022framework}. It represents the capability of the overall concept vector to predict the ground truth task label. 
            %     %Used in: ~\cite{sarkar2022framework}
            %     \item Concept Efficiency: in concept-based models, the concept capacity to predict the task depends on the number of concepts employed~\cite{zarlenga2022concept}. Richer concept representations mitigate this problem. 
            %     %Proposed in~\cite{zarlenga2022concept}. 
            %     \item Conciseness: similar to the concept efficiency but for post-hoc methods, it represents the number of concepts required to reach a certain grade of completeness and so a desired level of final accuracy~\cite{vielhaben2023multi}. 
            %     %Used in: ~\cite{vielhaben2023multi}.
            % \end{itemize}


\myparagraphbold{Quality of concepts}
This second category focuses on the quality of concepts, studying (i) their inherent properties, (ii) how they relate to internal network representations, and (iii) their impact on prediction errors. In the following, we review these metrics with respect to these three targets of focus.


\textit{(i) Concepts properties.}
This group of metrics centres on the intrinsic characteristics of concepts themselves
% not on their relation to the final classes or the network representation.
They evaluate the retained information, distinctiveness, completeness, and purity of concepts, providing insights into the information content and coverage of concepts. Among these metrics we find the Mutual Information~\cite{zarlenga2022concept}, Concept Distinctiveness~\cite{wang2023learning}, %Concept Completeness~\cite{wang2023learning}, 
Concept Purity~\cite{wang2023learning}. 
  
            % \begin{itemize}
            %     \item Mutual Information: it quantifies the amount of information retained in a concept representation with respect to the input data~\cite{zarlenga2022concept}. 
            %     %Proposed by:~\cite{zarlenga2022concept}.
            %     \item Distinctiveness: it quantifies the distinction between different concepts by considering the extent of their coverage~\cite{wang2023learning}. 
            %     %Proposed by: ~\cite{wang2023learning}.
            %     \item Completeness: Different from the previous definition of completeness given in~\cite{yeh2020completeness}, it measures how well a concept covers a specific associated class in the dataset~\cite{wang2023learning}. %Proposed by: ~\cite{wang2023learning}.
            %     \item Purity: it quantifies the ability to discover concepts covering only a single class~\cite{wang2023learning}. %Used in: ~\cite{wang2023learning}. 
            % \end{itemize}

\textit{(ii) Relation of Concepts with internal network representation.}
This group of metrics quantifies the relationship between a node (or filter) of the model and the concept it represents. These metrics are adopted for methods that provide explanations as \nodeconcass{}. They assess the spatial overlap (IoU) and location stability of concepts within activation maps. Among these metrics we find Intersection over Union \cite{bau2017network, fong2018net2vec, xuanyuan2023global} (and adopted~\cite{zhang2018interpretable} with the name of \textit{Part Interpretability}), Location stability~\cite{zhang2018interpretable}.

            % \begin{itemize}
            %     \item Intersection over Union (IoU): it measures the degree of overlapping of the bounding boxes representing the concepts and the activation maps of the single node~\cite{bau2017network, fong2018net2vec, xuanyuan2023global} (and adopted~\cite{zhang2018interpretable} with the name of \textit{Part Interpretability}).  
            %     %Proposed by: ~\cite{bau2017network}. 
            %     %Used in: ~\cite{fong2018net2vec}, ~\cite{xuanyuan2023global} and in ~\cite{zhang2018interpretable} with the name of \textit{Part Interpretability}.  
            %     \item Location stability: it assesses the consistency in how a filter represents the same object part across various objects~\cite{zhang2018interpretable}. %It computes the distance deviation between the inferred position and a specific ground-truth landmark among different images and uses the average deviation w.r.t. various landmarks to evaluate the location stability. A smaller deviation indicates a higher location stability. 
            %     %Used in: \cite{zhang2018interpretable}.
            % \end{itemize}


\textit{(iii) Concept prediction error.}
This group of metrics measures the alignment between learned concepts and concept ground truth. Hence, they are applicable when concept labels are available. These metrics evaluate and quantify mispredictions and the purity of concepts. Among these metrics we find the Concept Error~\cite{koh2020concept} (and used in~\cite{sarkar2022framework} with the name Explanation Error), AUC score~\cite{chen2020concept}, Misprediction-overlap metric (MPO)~\cite{kazhdan2020now}.

%This group focuses on the concepts, particularly on assessing the quality of the concepts learned concerning the prediction of the concepts themselves. The main objective is to examine potential errors that may occur during the prediction process.
%%Similarly to the previous group, this group focuses on concepts and particularly assesses the quality of the representation with respect to the ground truth.             
            % \begin{itemize}
            %     \item Concept Error: %when ground truth concepts are available, 
            %     it measures how close the concepts learned are to the concept ground truth~\cite{koh2020concept} (and used in~\cite{sarkar2022framework} with the name Explanation Error). It involves computing the L2 distance between the concepts learned and the ground truth concepts to measure the alignment. 
            %     %Proposed by:~\cite{koh2020concept}, used in~\cite{sarkar2022framework} with the name Explanation Error.
            %     \item AUC score: this score measures whether the samples belonging to a concept are ranked higher than others~\cite{chen2020concept}. That is, the AUC score indicates the purity of the concepts. 
            %     %Used in: ~\cite{chen2020concept}.
            %     \item  Misprediction-overlap metric (MPO): it computes the sample fraction in the test set with at least \textit{m} relevant concepts predicted incorrectly~\cite{kazhdan2020now}. A larger MPO score implies a bigger proportion of incorrectly predicted concepts. 
            %     %Proposed by: ~\cite{kazhdan2020now}.
            % \end{itemize}



\subsection{Qualitative evaluation}\label{sec:human_eval}
As common in XAI assessment~\cite{bodria2023benchmarking}, several C-XAI works perform human evaluations to assess their method through human feedback.
% Qualitative assessments via human evaluation provide insights into the effectiveness of explanations based on concepts, and it does so from a user-centric perspective to ensure that explanations align with user understanding. 
% The human evaluation during testing is one of the 13 dimensions we utilized for method categorization. 
We report which methods perform human evaluations in the ``Human evaluation'' column of Tables \ref{tab:summary:posthoc2} (post-hoc methods) and \ref{tab:summary:bydesign2} (by-design approaches). Half of the post-hoc approaches conduct qualitative assessments, while only a quarter of explainable-by-design ones perform them.
In the following, we overview the assessment based on the nature of the aspect under study: understandability, coherence, and utility of concept explanations.


\myparagraphbold{Understandability of explanations} 
When evaluating explanations, the predominant focus involves assessing how understandable and reasonable the explanations are to humans.
Various measures and evaluation settings have been introduced to capture specific nuances within this context. One relevant property of explanation is their \textit{plausibility}, denoting the extent to which explanations align with human reasoning.
One direct setting for evaluating the explanation plausibility consists of asking users to determine if the explanation is justifiable and understandable based on their expectation~\cite{rajagopal2021selfexplain, bau2017network}.  %For example, a set of images with highlighted patches showing the most highly activating regions for each unit in the network are shown to human users, and they decide whether a given phrase describes most of the image patches or not~\cite{bau2017network}.
%In ProtoPool~\cite{rymarczyk2022interpretable}, users rank the feature salience on . 
To evaluate \textit{human understanding} of concepts, another evaluation approach requires users to label the identified concepts by selecting some phrases from a predefined vocabulary that best describes the concept~\cite{wang2023learning}. This method provides a structured measure for summarizing users' comprehension of identified concepts. Other approaches as~\cite{zhang2021invertible} measure the interpretability of a concept by asking users to provide free-text labels for concepts and identify, among a set, the candidate explanations matching the concept and measure their accuracy as the percentage of correctly identified concept explanations. Close to this setting,~\cite{zhou2015object} focus on quantifying the semantics learned by each network unit and evaluating the accuracy of human-assigned text annotations to concepts.
The \textit{trustability} of explanations is another critical aspect, where users provide feedback on their level of trust in the explanation~\cite{rajagopal2021selfexplain}.
The \textit{reasonability} of explanations evaluates the effectiveness of conveying meaningful information through explanations.
A way to evaluate it is by investigating what information saliency maps can communicate to humans. %The results of T-CAV~\cite{kim2018interpretability} show that saliency maps are ineffective in over half of the cases.
Another setting consists of providing different explanations for the same prediction and asking human raters to indicate which is more reasonable, as adopted by IBD~\cite{zhou2018interpretable}.
\textit{Factuality} assesses the accuracy of concepts by having annotators judge their alignment with ground truth images~\cite{yang2023language}.


\myparagraphbold{Coherence of concepts} Another aspect to evaluate is the coherence of concepts as perceived by humans.  This involves scrutinizing and evaluating the characteristics of the discovered concepts. 
An adopted evaluation method for measuring concept coherence is the intruder detection experiment. In this setup, for example, users are asked to identify an image among a set that is conceptually different from the rest~\cite{ghorbani2019towards, fel2023craft}. Another setting involves examining the nearest neighbor images associated with each discovered concept vector and selecting the most prevalent and cohesive concept~\cite{yeh2020completeness}.
The work in~\cite{yang2023language} defines the \textit{groundability} to measure the consistency of the vision-language model adopted in LaBO~\cite{yang2023language} to ground concepts to images in a manner that aligns with human interpretations.




\myparagraphbold{Utility of explanations }
The \textit{utility} of an explanation refers to its practical usefulness and effectiveness in providing insights or guidance to users, typically in the context of the specific task.
It is often measured by its ability to assist users in predicting, performing a task, or making informed decisions in a given context.
For example, in~\cite{jain2022extending}, users evaluate the utility of explanations in improving classifier generalization through feature engineering. They identify problematic features using global explanations and evaluate the ease of use of the explanations for this task. In addition, users select the most general classifier based solely on the global explanations of various methods.
Other user study settings, such as in~\cite{fel2023craft}, measure how well the explanations assist users in inferring the insights guiding classifications. The utility is evaluated by measuring users' accuracy in predicting model decisions on novel images given the explanations.

%\myparagraphbold{Human Annotation Verification}:  %coherence between the expected human annotation and 
   % this entails evaluating the accuracy of human-assigned \textit{tags} to concepts, as demonstrated in Obj. Det~\cite{zhou2015object}.

%\myparagraphbold{Similarity Function efficacy}:
%Some approaches  for prototype approaches, it might be important to assess with humans the effectiveness of the similarity function used to calculate the maximum similarity between the prototypes and the image activation map. 

  %  \item \textbf{Explanation Quality: Plausibility, Trustability, and Utility}: this category includes methods that assess the quality of explanations through human evaluation. In SelfExplain~\cite{rajagopal2021selfexplain}, the assessment is conducted based on two metrics: (i) \textit{Plausibility}, where users determine if the explanation is justifiable and understandable to humans, and (ii) \textit{Trustability}, where users indicate their level of trust in the explanation. In~\cite{jain2022extending}, users assess \textit{Utility} of explanations for enhancing classifier generalization via feature engineering. Users identify problematic features using various global explanations and evaluate the ease of use of the explanations for this task. In addition, users select the most general classifier based solely on the global explanations of various methods.
  %  \item \textbf{Concept Soundness: Factuality, Groundability, and Understanding}:  this category includes methods that assess the validity of concepts through human evaluation. In LaBO~\cite{yang2023language}, two metrics are applied: (i) \textit{Factuality}, assessing concept accuracy by having annotators judge their alignment with ground truth images, and (ii) \textit{Groundability}, measuring the consistency of the vision-language model grounding of the concepts to images with human interpretations. by requiring annotators to judge their applicability on the top-10 images ranked by CLIP alignment scores. In BotCL~\cite{wang2023learning}, the human understanding of concepts is evaluated by asking users to label the identified concepts by selecting some phrases from a predefined vocabulary that best describes the concept. %Then three metrics summarize the users' understanding of concepts. 


% \input{Tables/table_datasets}

\subsection{Datasets}\label{sec:datasets}
We now analyze the most interesting datasets employed in the literature. Among the datasets experimented by the method reviewed in this survey, we report in Table~\ref{tab:datasets} only those where the authors either explicitly describe the concept annotations or the procedure followed to extract them (Extracted).
%We present here the datasets employed by the reviewed methods. From the entirety of collected datasets, we focus on showcasing datasets for which the authors of the methods that use them explicitly describe the concepts or procedures followed to extract them. 
We classified them based on the data type: images (IMG), text (TXT), videos (VID), tabular (TAB), time series (TS), and graph data (Graph).

On top of Table~\ref{tab:datasets}, we report the image datasets.
% Table \ref{tab:IMG_datasets} shows the image datasets used, all of which are suitable for classification tasks, including one suitable for a regression task. 
We observe that the CUB dataset is the predominant choice in the C-XAI literature. This dataset is very suitable for such methodologies due to its extensive annotation of concepts, representing the visual attributes inherent to different bird species. 
We also note that the BRODEN dataset~\cite{bau2017network} was introduced explicitly for concept-based XAI. This dataset encompasses over 63,000 images and 1,197 concepts distributed across six categories (i.e., textures, colors, materials, parts, objects, and scenes).
Finally, OAI is the only dataset that is suitable for regression tasks and not only for classification (the level of osteoarthritis may be both considered as a class or as a continuous level).
%
% Table \ref{tab:TXT_datasets}
In the second part, we find the text datasets. These datasets predominantly revolve around binary or multi-class sentiment classifications. In most datasets, the concepts are not already present but are extracted from the input texts using various techniques. For example, in~\cite{rajagopal2021selfexplain}, concepts are represented by non-terminal phrases of the parsing tree.
%
%Table \ref{tab:VID_datasets} shows datasets of videos. 
Within the third part of the table reporting videos dataset, BDD-OIA is the only dataset with pre-established concepts, while in the other two cases, concepts are extracted through specific processes.
%
% Finally, we include in Table \ref{tab:MISC_datasets} datasets of different natures, including tabular and graphs. 
In tabular data sets, data attributes are used concepts. Finally, in graph datasets, concepts are always extracted by the method.


% \input{Tables/table_VID_dataset}
% \input{Tables/table_MISC_dataset}

\subsection{Resources}\label{sec:resources}
We now report information and insights regarding the resources associated with the reviewed methods. %The resources of these methods are delineated within the dimensions of the analysis outlined in Section \ref{sec:dimanalysis}. 
Specifically, when we refer to \textit{resources}, we are addressing whether the authors of the respective papers have made the code, models utilized in their research publicly accessible or have released a new dataset. 
Among all methods discussed, nearly all but four have made their code publicly available on GitHub, two post-hoc methods (CaCE, Object Detection) and two concept-based models (SENN, CBM-AUC).
Overall, there is a common trend of releasing code on public platforms (e.g., GitHub), which benefits the community by providing a starting point for testing and development.  
Concerning data release, four methods released novel datasets, equally distributed between post-hoc methods (ND, DMA \& IMA) and concept-based models (CME, Glance-Nets).
The release of new datasets is infrequent due to the resource-intensive nature of creating concept annotated datasets. It may require $C\times N$ extra annotations where $C$ represents the number of concepts and $N$ the number of samples. In other cases, a class-level annotation of the concept is preferred to decrease this effort. It consists in employing the same concept annotation for all the samples belonging to the same class, therefore reducing the number of annotations to $N\times Y$, where $Y$ represents the number of final classes.
%In the case of concept datasets, annotating these is still an effort-intensive additional step. Therefore, we find the low tendency to release datasets in revised methods reasonable.
For additional information on the works with shared code, models, or datasets released, please consult Appendix \ref{app:resources}.


% \section{First Applications and Promising Directions}
% \label{sec:app_and_future}
% In this section we briefly review the first applications of concept-based approaches (Section~\ref{sec:application}). Also, we will discuss some promising future work within the C-XAI field (Section~\ref{sec:future_work}).

\section{Applications}
\label{sec:application}
The recent emergence of C-XAI methods has %already 
led to some interesting applications. We report first novel algorithms based on concepts in the field within the AI area (outside explainability), followed by real-world applications.

\myparagraphbold{Support to AI algorithm's development}
The first application of concept-based methods within AI came out in the image generation field. In VAEL~\cite{misino2022vael}, the authors proposed to condition the generation of images by means of a neuro-symbolic program working over concepts. %More precisely, they require the generated images to solve a given query. 
For example, given two pairs of digits from MNIST, they train the concepts to represent the digits and the logic program to predict the addition of the digits. When decoding, they require instead that the generated images correspond to samples solving the given query (e.g., digits whose sum is 13). Interestingly, they show that their method also generalizes to queries unseen in training (e.g., they generate the samples whose difference or factorization is provided). 
% In \textbf{VICE}~\cite{muttenthaler2022vice}, NON E' CONCEPT EXPLANATION

Other concept-based algorithms appeared in the out-of-distribution sample detection field. In particular, the author of~\cite{madeira2023zebra} proposed a concept-based approach to characterize outliers. They propose first mapping the sample into an interpretable feature space comprising human-defined concepts like textures, colors, and geometry. In this space, they analyze the rarity of the features to detect outliers and explain the rarest concepts identified in the sample.
The author of~\cite{choi2023concept}, instead, employs an unsupervised approach to extract concepts that can sufficiently characterize the decisions of an out-of-distribution detector. Furthermore, they require extracted concepts to separate in-distribution and out-of-distribution samples. Interestingly, they show that extracting concepts to explain the classifier is insufficient to explain the out-of-distribution detector's prediction.

\myparagraphbold{Real-world applications}
Outside the AI world, the medical sector is where we find most applications of C-XAI already in the reviewed papers (CAR, CBM, PCBM, ProtoPDebug, LaBO). Another example is~\cite{lucieri2020interpretability}, where the authors employ a post-hoc concept-based method in the Computer-Aided Diagnosis (CAD) systems in skin cancer diagnosis. %The main concern in adopting CAD systems is the lack of insight into the reasoning that the model is doing to make the predictions. For this reason, 
The authors want to elucidate the basic principles that guide the model's predictions, discerning whether the model operates on similar concepts to those used by dermatologists to describe and diagnose the disease. Specifically, using TCAV~\cite{kim2018interpretability} method, they show a strong correlation between DNN's learned representation of concepts and those routinely used by dermatologists. Hence, listing the concepts that positively influenced the final outcome may be sufficient for trusting the predictions of a CAD system. %when justifying their predictions. %is widely applicable in this field although the usage of a more fine-grained labelling of data can benefit the method's performance. 

In the field of education, we identify RIPPLE ~\cite{asadi2023ripple} as a first application. This work introduces a pipeline to make predictions from raw time series data about students' success that is also interpretable. Specifically, they use a combination of a graph-based neural network approach for classifying raw time series of student interactions and an adaptation of concept activation vectors TCAV~\cite{kim2018interpretability} for interpreting NN internal state in terms of human-interpretable concepts. In this case, concepts are represented by six learning dimensions from educational scenarios defined a-priori. 


\section{Promising Directions}
\label{sec:future_work}
The analysis of the C-XAI field literature allows highlighting  several promising directions existing for both researchers and practitioners. Addressing these frontiers is important not only for enhancing the interpretability of artificial intelligence systems but also for fostering their responsible and effective deployment across diverse domains. Herein, we outline key directions that we believe merit focused explorations, encompassing both methodological advancements and improvements from an evaluation and application point of view.

From a methodological point of view, we believe that generative approaches could also be explored for post-hoc concept-based methods. On one side, Generative models could be harnessed to create concepts akin to their role in concept-based models. On the other, LLMs could also be employed to enhance supervised post-hoc methods in assessing model causality when prompted with specific concepts.
Still considering the post-hoc methods, the analysis of Table~\ref{tab:summary:posthoc1} reveals a gap in exploring node-concept association explanations for unsupervised methods. Even though it may be difficult to associate nodes to extract concepts, it represents a valuable avenue for exploration.

Concerning concept-based models, extending concept representations to accommodate multi-modal data, such as text, images, and audio, could greatly enhance the versatility of C-XAI across different domains.
Also, the novel generative approach seems open to several extensions. Moreover, the new generative approach seems to be open to different types of fusion following the same approach: a concept generator that creates representations (not necessarily textual) that can be used in an external (not necessarily visual) model. 

%Exploring both post-hoc methods and concept-based models capable of dynamic and contextual explanations is another intriguing avenue. Understanding how concepts and their importance evolve over time or under different contexts could enhance the adaptability and relevance of explanations.

On the evaluation front, the field currently lacks benchmark datasets and standardized metrics, hindering systematic comparisons. Developing these resources would facilitate fair assessments of different methods. %Moreover, human-centric evaluation could be improved through more extensive and diverse experiments. This should include several methods and user users with varying levels of expertise in the domain.

From an application point of view, it would be important to develop scalable concept-based methods and models that can handle and be integrated into large-scale models and applied to large-scale datasets. 
Finally, properly integrating concept-based models is crucial to creating accountable AI-powered decision-making systems, particularly in critical domains like healthcare, finance, and autonomous systems. 


\section{Conclusion} % 1 page
\label{sec:conclusions}
% ADD something on future directions?

In conclusion, our comprehensive review of Concept-based explainable Artificial Intelligence highlights the growing interest in concept-based explanations in addressing the demand for transparent and interpretable AI models. The ongoing debate regarding the limitations of raw feature-based explanations has led to a substantial body of work on concept-based explanations. 
By defining the various types of concepts and concept-based explanations and introducing a systematic categorization framework, we hope to have facilitated a more structured understanding of the C-XAI landscape. Our analysis of C-XAI papers, which we reviewed and categorized with the proposed taxonomy into nine categories, may provide valuable insights into the strengths and challenges of different categories. 
Furthermore, by highlighting key resources within the C-XAI literature, such as datasets and metrics, we aspire to catalyze future research and facilitate comparisons between different methodologies. % we hope to propel future research and method comparisons by reporting the pivotal resources within the C-XAI literature, including datasets and metrics. %Moreover, this review has shed light on the early applications of C-XAI methods and laid the foundation for intriguing avenues of exploration in the realm of interpretable and trustworthy AI models.



% \begin{acks}
% Figures \labelcref{fig:cxai,fig:xai_problem,fig:tcav,fig:net_dissect,fig:ace,fig:len,fig:pcbm,fig:senn,fig:protopnets,fig:ante_hoc,fig:labo} have been extracted from the referenced paper or source. The copyright for these figures is held by the respective authors of the original paper.
% \end{acks}

\bibliographystyle{acm}
\bibliography{main}

